Coverability, Termination, and Finiteness in Recursive Petri Nets

In the early two-thousands, Recursive Petri nets have been introduced in order to model distributed planning of multi-agent systems for which counters and recursivity were necessary. Although Recursive Petri nets strictly extend Petri nets and context-free grammars, most of the usual problems (reachability, coverability, finiteness, boundedness and termination) were known to be solvable by using non-primitive recursive algorithms. For almost all other extended Petri nets models containing a stack, the complexity of coverability and termination are unknown or strictly larger than EXPSPACE. In contrast, we establish here that for Recursive Petri nets, the coverability, termination, boundedness and finiteness problems are EXPSPACE-complete as for Petri nets. From an expressiveness point of view, we show that coverability languages of Recursive Petri nets strictly include the union of coverability languages of Petri nets and context-free languages. Thus we get a more powerful model than Petri net for free.

==> algo_abstra.tex <==
% !TEX root = main.tex
\begin{algorithm2e}[h]
	\LinesNumbered
	\DontPrintSemicolon
	\SetKwFunction{Remove}{Remove}
	\SetKwFunction{Select}{Select}
	\SetKwFunction{Pick}{Pick}
	\SetKwFunction{Delete}{Delete}
	\SetKwFunction{NewAcceleration}{NewAcceleration}
	\SetKwFunction{Push}{Push}
	\SetKwFunction{Pop}{Pop}
	\SetKwFunction{Parent}{Parent}
%	\igor{change everything to $ \N_{el} $}
	
	Abstract\_Graph$(\N,s)$\;
	\KwIn{ $(\N,s)$ a marked RPN}
	\KwData
	{
		The vertices of the abstract graph $V_a$ , its edges $ E_a  $, and its marking $ M_a:V_a\rightarrow \nat^P$
		
	}
	\KwOut{$G_{\N,s}=(V_a,E_a,M_a)$}
%	\ForEach{ $v\in V_s$}{ $M_a(v)=M_{s_{ini}}(v)$}
	
	
	$V_a \leftarrow V_{s}$; $ E_a \leftarrow \emptyset $\; 

	\lForEach{$ v\in V_s $}{$ M_a(v) =M_{s}(v) $}\label{line: init end}
%	\igor{change to acc. to edges}\;
	\ForEach(\tcp*[h]{Gratest depth first}){$ e=(u,v)\in E_s$ \label{line: beg first loop}}
		{
			\If{ $ \exists m\in\mathcal{F} \text{ and }\sigma$ s.t. $ M_a(v)\xrightarrow{\sigma} m'\geq m $ in $\widehat{\N}_{el}$  \label{line:checking marking}}
			{
				$ M_a(u)\leftarrow M_a(u) + W^+(\Lambda_{s}(e)) $ \label{line: add tokens to parent}
			}
				
		}
	\label{line: end first loop}
	$ Front \leftarrow V_{s} $ \;
	\While{$ Front \neq \emptyset $ \label{line: beg second loop}}
	{
		$ u = \Pop(Front) $\;
		\ForEach{$ t\in T_{ab} $}
		{
			\If{ $ \exists \sigma $ s.t. $ M_a(u)\xrightarrow{\sigma} m\geq W^-(t)$ in $\widehat{\N}_{el}$ \label{line:checking abs tran fire}}
			{
				\lIf{$v_t\notin V$} 
				{
					$V\leftarrow V\cup \{v_t \}$; $M'(v_t)=\Omega(t)$; $ \Push(Front,v_t) $
				}
				$E\leftarrow E\cup \{(u,v_t)\}$
			}
		}
		
	}\label{line: end second loop}
	\Return $(V,E,M_a)$\;
	
	\caption{Computing the abstract graph} 
	\label{algo:abstract graph}
	
\end{algorithm2e}


==> conclusion.tex <==
% !TEX root =main.tex
\section{Conclusion}
\label{sec:conclusion}

%\alain{can we limit the order to a Rackoff constant such that it don't contain infinite antichains and then becomes a wqo ?}

%
%\alain{coverability set sometimes better than Rackoff.KM ? emptyness known but complexity of the word membership problem ? with a reduction to another RPN ?}
We have proven that RPN is a strict generalisation of both Petri nets 
and context-free grammars without increasing the complexity of coverability, termination, boundedness and finiteness problems. 
%Let us put the emphasis on the fact that Rackoff techniques work well while the ordering is not a wqo. 
It remains several open problems about languages of RPN and decidability/complexity 
of checking properties. Here is a partial list of open problems:
\begin{itemize}
%\item Is the family of coverability languages of RPN included
%in the family of reachability languages of RPN?
\item  How to decide whether a word belongs 
to a coverability or reachability language of a RP?
%\item define the Recursive VASS ?
%\item study RPN with one and two bounded places?
%	avec une place as a natural extension of 1-VASS and context-free languages ?
%\item May be reachability is PSPACE for 2-RPN (2-Recursive VASS) as for 2-VASS ?
%\end{itemize}
%Decidability and complexity
%\begin{itemize}
%
\item Since the quasi-order possesses an infinite antichain, but there exist short witnesses for coverability, 
does there exist an effective finite representation 
of the downward closure of the reachability set?
\item Does there exist a relevant fragment of LTL decidable for RPN?
\end{itemize}
%\item In this case, is it possible to make a Karp-Miller algorithm (like for BVASS) for computing the coverability set ?

{\noindent \bf Acknowledgment.} We thank the reviewers very much for their deep, detailed and insightful reviews, which helped us a lot in order to simplify and clarify this paper.


==> coverability-3.tex <==
% !TEX root =main.tex
\section{Coverability  is \EXPSPACE -Complete}
\label{sec:coverability}

The section is devoted to establishing that the coverability problem
is $\EXPSPACE$-complete. The
$\EXPSPACE$-hardness follows immediately
from the $\EXPSPACE$-hardness of the coverability problem for Petri nets~\cite{Lipton76}.

Observe that the coverability problem is equivalent to the emptiness problem of the coverability language of an RPN.
In Section \ref{sec:expressiveness} we have shown that the families of coverability languages and cut languages for RPN are equal and that the transformation from one to another is performed in polynomial time (proposition \ref{prop:reach-inc-cov} and \ref{prop:cov-inc-reach}). Therefore we will establish the complexity result for the cut problem getting as a corollary the same result for the coverability problem.
%So to solve the coverability problem on Petri nets,
%one guesses a sequence of length at most  $2^{2^{cn\log n}}$,
%checking at the same time whether it is a covering sequence in exponential space.
%Which shows that the coverability problem belongs to $\NEXPSPACE=\EXPSPACE$
%by Savitch's theorem.
%For this end we will show that if there exists some $\sigma$ such that
%$
%s_0\xrightarrow{\sigma}\emptyset
%$
%in an RPN $\N$, then there exists a `short' sequence $\sigma'$.
%\noindent{\bf Notation:} we denote by $\eta$ the input of the cut problem, i.e. the accumulated size of the RPN and the initial state
%	In the sequel .
%\begin{proposition}\label{prop:bound_on_cut_length}
%	Let $ \N $ be an RPN, and $s_0\xrightarrow{\sigma}\emptyset$. Then there exists a firing sequence of length shorter than $2^{2^{e\eta\log \eta}}$.
%\end{proposition}
\begin{theorem}\label{thm:cut_problem}
	The cut problem is \EXPSPACE-complete.
\end{theorem}

\begin{proof}
	\noindent Let $(\N,s_0)$ be a marked RPN and $\eta$ the accumulated size of the RPN and the initial state. 
	By Proposition~\ref{col:rooted} we can assume that $V_{s_0}$ is a singleton $\{r\}$.
	
	\noindent Assume there exists a firing sequence $s_{0}\xrightarrow{\sigma}_{\N}\emptyset$.  Using Proposition~\ref{prop:omniciant} one gets an omniscient sequence $ s_0\xrightarrow{\widehat{\sigma}}_{\widehat{\N}}\emptyset$ such that
	$\widehat{\sigma}=(r,\sigma_{1})(r,t)$ for some $t\in T_{\tau}$.
	
	\noindent The (omniscient) sequence $(r, \sigma_1)$  contains only elementary transitions.
	Thus $m_0 \xrightarrow{\sigma_1}_{\widehat{\N}_{el}} m$ with $m\geq W^-(t)$.
	By Theorem~\ref{thm:Rackoff covering path}, there exists  $ \sigma_1' $ with
	$ |\sigma_1'|\leq 2^{2^{c\eta\log \eta}}$ covering $W^-(t)$.	
	Using Corollary \ref{col:bound_on_translation_of_N-hat_to_N} there $s\xrightarrow{\sigma'}_{\N}\emptyset$ with $|\sigma'|\leq ^{2^{e\eta\log \eta}} $ for some constant $ e $.
	
	\noindent Therefore if there is a cut sequence
	then there is one with length at most $2^{2^{e\eta\log \eta}}$. Hence
	one guesses a sequence with at most this length and
	simultaneously checks  whether it is a cut sequence in exponential space.
	This shows that the cut problem belongs to $\NEXPSPACE$ which is equivalent to $\EXPSPACE$
	by Savitch's theorem. 
	
	\noindent The \EXPSPACE\ hardness of the coverability problem in Petri nets entails \EXPSPACE\ hardness of the coverability problem in RPNs
	which in turn entails the \EXPSPACE\ hardness of the cut problem in RPNs.
	
\end{proof}
The next theorem is an immediate corollary of the previous one.
\begin{theorem}\label{thm:Coverabilty for RPN in EXPSPACE}
	The coverability problem for RPNs is $\EXPSPACE$-complete.
\end{theorem}




















==> expressiveness.tex <==
% !TEX root =main.tex
\section{Expressiveness}
\label{sec:expressiveness}



The expressiveness of a formalism may be defined by the family
of languages that it can generate. In~\cite{HP-icatpn99}, the expressiveness
of RPNs was studied using reachability languages. However, using reachability languages as specification languages has an
inconvenient since the emptiness problem for these languages is not elementary \cite{DBLP:conf/stoc/CzerwinskiLLLM19} for Petri nets, 
so it is also not elementary, at least, for RPN. We propose to characterize the expressive
power of RPN by studying the family of coverability languages
which is sufficient to express most of the usual reachability properties since many of them reduce to check that no reachable state 
may cover a bad marking in a thread.


%
%Thus we now study the coverability languages.
%	\alain{It is true that this argumentation is weak. New argumentation pour etudier les langages couvrants .}

The characterization of the expressive power by means of covering languages has been done for Petri nets (studied in the book of Peterson  \cite{nla.cat-vn2956435}), and more recently, for Well Structured Transition Systems (WSTS) \cite{DBLP:journals/acta/GeeraertsRB07} and for monotonic extensions of Petri nets like reset-transfer Petri nets, $\nu$-Petri nets, unordered Petri nets \cite{BFHR-icomp13,DBLP:journals/tcs/DelzannoR13}. 
More properties are decidable for VASS covering languages than for VASS reachability languages.
For instance, universality for reachability languages is undecidable for 1-VASS \cite{DBLP:journals/jcss/ValkV81} and then co-finiteness is also undecidable but these two properties are both decidable for VASS covering languages \cite{figueira:hal-02193089}; moreover, it is Ackermann-complete for 1-VASSs \cite{DBLP:conf/rp/HofmanT14}. Generally, the universality of both reachability and coverability of WSTS languages is undecidable \cite{DBLP:journals/acta/GeeraertsRB07}.
%
%and this is equivalent to test the emptiness of an associated covering language). 
%\alain{find another argument to manipulate covering languages}
%
%Moreover, for VASS, the class $L_C(VASS)$ has an avantage compared with the class $L_R(VASS)$ of reachability languages:
%\begin{enumerate}
%\item The algorithms for languages in $L_C(VASS)$ often have a better complexity than those in $L_R(VASS)$.
%For instance, the emptyness question for languages in $L_R(VASS)$ is decidable but it is not elementary \cite{DBLP:conf/stoc/CzerwinskiLLLM19} while it is "only" $ \EXPSPACE$ for languages in $L \in L_C(VASS)$.
%\item More properties are decidable in $L_C(VASS)$ than in $L_R(VASS)$.
%For instance, universality for languages in $L_R(VASS)$ is undecidable for 1-VASS \cite{DBLP:journals/jcss/ValkV81} and then co-finitess is also undecidable but these two properties are both decidable for covering languages in $L_C(VASS)$ \cite{figueira:hal-02193089}; moreover, it is Ackermann-complete for 1-VASSs \cite{DBLP:conf/rp/HofmanT14}. Universality of both reachability and covering WSTS languages is undecidable \cite{DBLP:journals/acta/GeeraertsRB07}.
%\end{enumerate}
%
%We will prove in Section XXX that 
%\begin{enumerate}
%\item  Does universality decidable for languages in $L_C$(RPN)  ? Does universality decidable for languages in $L_C$(1-RPN)  ? Peut-on generaliser \cite{figueira:hal-02193089} qui utilise le fait que les sequences bad ont une longueur bornee ? Not sure since we have not a wqo.
%
%
%\item Coverability is $ \EXPSPACE$ for RPN, hence emptyness of covering languages is also $ \EXPSPACE$. 
%\end{enumerate}
%
%In the next section, we are going to establish
%that the coverability problem for RPNs has a lower complexity than the one of the reachability problem for RPNs.

%\alain{We complete l’etude des reachability languages des RPN (Haddad ).}

%Many questions: $L_C(RPN)$ is it closed under concatenation ? cartesian product ? complement ? and under Kleen star $*$ ? inclusion of a covering language into a regular one ?

%Que peut-on encore decider pour les langages couvrants ?



So we equip any transition $t$ with a \emph{label} $\lambda(t)\in \Sigma \cup \{\varepsilon\}$
where $\Sigma$ is a finite alphabet and $\varepsilon$ is the empty word.
The labelling is extended to transition sequences in the usual way.
Thus given a labelled marked RPN $(\N,s_0)$ and a finite subset of states $S_f$, 
the (coverability) language
$\mathcal L_C(\N,s_0,S_f)$ is defined by:
$$\mathcal L_C(\N,s_0,S_f)=\{\lambda(\sigma) \mid \exists\ s_0 \xrightarrow{\sigma} s\succeq s_f\wedge s_f \in S_f\}$$
i.e. the set of labellings for sequences covering some state of $S_f$ in $\N$.



%The next lemma simplifies the proof that coverability languages of RPN are closed by union.
%\begin{lemma}
%	\label{lem:singlethread}
%	Let $\mathcal L(\N,s_0,S_f)$ be an RPN language. 
%	Then there exists a  marked
%	RPN $(\N',s[r',m'_0])$
%	for some $m'_0\in \nat^P$and a finite subset of states
%	$S'_f$ such that $\mathcal L(\N',s[r',m'_0],S'_f)=\mathcal L(\N,s_0,S_f)$.
%\end{lemma}
%\begin{proof}
%	$\N'$
%	is built from $\N$ by adding a subset of places $\{p_v \mid v\in V_s\setminus \{r_s\}\}$ and
%	a subset of abstract transitions $\{t_v \mid v\in  V_s\setminus \{r_s\}\}$
%	all labelled by $\varepsilon$. Let $u\xrightarrow{m}_s v$.
%	Then $W^-(t_v)=p_v$, $W^+(t_v)=m$ and $\Omega(t_v)=M(v)+\sum_{v\xrightarrow{m'}_s v'} p_{v'}$.
%	$S'_f$ is obtained from $S_f$ by extending the markings occurring in the states of $S_f$ to be null
%	on the subset  $\{p_v \mid  v\in V_s\setminus \{r_s\}\}$. Finally
%	$m'_0=M(r_s)+\sum_{r_s\xrightarrow{m'}_s v'} p_{v'}$.
%	
%	\smallskip \noindent
%	Let us prove that $\mathcal L(\N,s_0,S_f) \subseteq \mathcal L(\N',s[r',m'_0],S'_f)$.
%	Consider a coverability sequence $\sigma$ for $(\N,s_0,S_f)$.
%	One starts to fire all transitions of $\{t_v \mid  v\in V_s\setminus \{r_s\}\}$ in a top-down way
%	to get a state $s'_1$ such that (when omitting places $\{p_e\}$) 
%	both $s_0\simeq s'_1$ and
%	so that we identify the corresponding threads. Let us denote $\sigma_0$
%	this sequence. Then $\sigma_0\sigma$ is a coverability sequence for $(\N',s[r',m'_0],S'_f)$
%	with $\lambda(\sigma_0\sigma)=\lambda(\sigma)$.
%	
%	\smallskip \noindent
%	Let us prove that  $\mathcal L(\N',s[r',m'_0],S'_f) \subseteq \mathcal L(\N,s_0,S_f)$.
%	In $(\N',s[r',m'_0],S'_f)$, consider a coverability sequence $\sigma$.
%	By construction of $\N'$, all  occurrences of transitions of $\{t_v \mid v\in V_s\setminus \{r_s\}\}$
%	can be pushed at the beginning of the sequence leading to a covering
%	sequence $\sigma'=\sigma_1\sigma_2$ where $\sigma_1$
%	consists of such occurrences. Then $\sigma_1$ can be completed 
%	by the missing occurrences
%	still in a top-down way producing $\sigma'_1$ and 
%	yielding a coverability sequence $\sigma''=\sigma'_1\sigma_2$.
%	Moreover the state $s_1$ (when omitting places $\{p_v\}$) reached from $\sigma'_1$
%	is equivalent to $s_0$. Thus $\sigma_2$ is a coverability sequence for $(\N,s_0,S_f)$
%	with $\lambda(\sigma_2)=\lambda(\sigma)$. 	
%\end{proof}
We now study the family of RPN coverability languages both from the point of view of expressiveness and closure under multiple operations.

\begin{restatable}{proposition}{closedbyunion}
	%\begin{proposition}
	\label{prop:closedunion}
	The family of coverability languages of RPNs is closed under union.
	%\end{proposition}
\end{restatable}
\begin{proof}
	We closely follow the classic proof that the family of Petri net languages is closed under union, i.e. adding a place and two extra transitions that have to be fired in the beginning of the firing sequence in order to decide in which of the Petri net one fires. Due to the correspondence between firing sequences of $(\N,s_0)$ and those of $(\rooted{\N},\sr)$,
	established in the previous section,
	one can assume w.l.o.g. that the initial markings of the RPNs have a single vertex.
	Consider two labelled marked RPNs with final states
	$(\N,s[r,m_0],S_f)$ and $(\N',s[r',m'_0],S'_f)$.
	Let us define $\widetilde{\N}$ as follows.
	Its set of places is the disjoint union of $P$ and $P'$
	with three additional places $p_0$, $p$ and $p'$.
	Its set of transitions is the disjoint union of $T$ and $T'$
	with four additional elementary transitions $t_b$, $t_c$, $t'_b$ and $t'_c$.
	
	\smallskip\noindent
	$\bullet$ For all $t\in T$, $\widetilde{W}^-(t)=W^-(t)+p$ and when $t\notin T_{\tau}$
	$\widetilde{W}^+(t)=W^+(t)$\\
	$\bullet$ For all $t\in T'$, $\widetilde{W}^-(t)=W'^-(t)+
	p'$ and when $t\notin T'_{\tau}$ $\widetilde{W}^+(t)=W'^+(t)$\\
	$\bullet$ For all $t\in T_{ab}$, $\widetilde{\Omega}(t)=\Omega(t)+ p$\\
	$\bullet$ For all $t\in T'_{ab}$, $\widetilde{\Omega}(t)=\Omega'(t)+ p'$\\
	$\bullet$ $\widetilde{W}^-(t_b)=\widetilde{W}^-(t'_b)= p_0$,
	$\widetilde{W}^+(t_b)=m_0+ p$, $\widetilde{W}^+(t'_b)=m_0'+ p'$\\
	$\bullet$ $\widetilde{W}^-(t_c)=p$, $\widetilde{W}^+(t_c)=2 p$,
	$\widetilde{W}^-(t'_c)= p'$, $\widetilde{W}^+(t'_c)=2 p'$\\
	$\bullet$ $\widetilde{S}_f$ is obtained from the union 
	$S_f\cup S'_f$ by adding a token in place
	$p$ (resp. $p'$)\\
	\hspace*{0.3cm}of all markings of states of $S_f$ (respectively $S'_f$).\\
	$\bullet$ For all $t\in T$, $\widetilde{\lambda}(t)=\lambda(t)$ and
	for all $t\in T'$, $\widetilde{\lambda}(t)=\lambda'(t)$\\
	$\bullet$ For all $t\in \{t_b,t_c,t'_b,t'_c\}$, 
	$\widetilde{\lambda}(t)=\varepsilon$.\\
	$\bullet$ The initial state of $\widetilde{\N}$ is $s[\tilde{r},p_0]$.
	
	\smallskip\noindent
	Let us prove that $\mathcal L(\N,s[r,m_0],S_f) \cup \mathcal L(\N',s[r',m'_0],S'_f)
	\subseteq \mathcal L(\widetilde{\N},s[\tilde{r},p_0],\widetilde{S}_f)$.
	Let $\sigma$ be a coverability sequence of $(\N,s[r,m_0],S_f)$.
	The corresponding coverability sequence $\widetilde{\sigma}$
	of $L(\widetilde{\N},s[\tilde{r},p_0],\widetilde{S}_f)$ is built as follows. 
	Initially,
	one fires $(\tilde{r},t_b)(\tilde{r},t_c)^{\ell_r}$ where $\ell_r$ is the number of abstract transition firings
	occurring in $\sigma$ triggered by $r$. Then after the creation
	of a thread $v$, one inserts $(v,t_c)^{\ell_v}$ firings where $\ell_v$ 
	is the number of abstract transition firings
	occurring in $\sigma$ triggered by $v$. It is routine to check that
	$\widetilde{\sigma}$ is coverability sequence. The proof for
	$\mathcal L(\N',s[r',m'_0],S'_f)$ is similar.
	
	
	
	\smallskip\noindent
	Let us prove that $\mathcal L(\widetilde{\N},s[r,p_0],\widetilde{S}_f)
	\subseteq \mathcal L(\N,s[\tilde{r},m_0],S_f) \cup \mathcal L(\N',s[r',m'_0],S'_f)$.
	Observe that any firing sequence must start
	by a firing of $t_b$ or $t'_b$.
	Let $t_b\widetilde{\sigma}$ be a coverability sequence of
	$(\widetilde{\N},s[\tilde{r},p_0],\widetilde{S}_f)$. Consider the sequence $\sigma$
	obtained by deleting all the firings of $t_c$ in $\tilde{\sigma}$.
	It is routine to check that
	$\sigma$ is a coverability sequence for $(\N,s[r,m_0],S_f)$.
	The case of a coverability sequence starting by $t'_b$ is similar. 
	
\end{proof}
The next theorem has two interesting consequences: the family of RPN coverability languages
is not closed under intersection with the family of regular languages. But the family obtained by this intersection
is \emph{quite close} to the family of recursively enumerable languages.
The result was already stated in Proposition~9 of~\cite{HaddadP99}
for the family of RPN reachability languages but the proof was only sketched. 
\begin{theorem}
	\label{theo:re}
	Let $\mathcal L$ be a recursively enumerable language. Then there
	exist an RPN language $\mathcal L'$, a regular language
	$\mathcal R$ and a homomorphism $h$ such that
	$\mathcal L=h(\mathcal L'\cap\mathcal R)$.
\end{theorem}
\begin{proof}
	Let $\mathcal M=(\Sigma,L,\delta)$ be a Turing machine with it set of states $L$ 
	including $\ell_0$ (resp. $\ell_f$) the initial (resp. final) state and its transition function
	$\delta$ from $L\times \Sigma \cup \{\flat\}$ to $L\times \Sigma \times \{\leftarrow,\rightarrow\}$
	where $\flat$ is the blank character.
	
	Let us define a labeled marked RPN $\N$ and an automaton $\mathcal A$.
	Their common alphabet is the set of transitions of $\N$
	and the labeling of the transitions of the RPN is the identity mapping. 
	The intersection of their languages is thus the language of the synchronized product of the two devices.
	The single final state of $\N$ (to be covered) is the empty tree.
	
	The automaton $\mathcal A$ is depicted below (with $\Sigma=\{a,b\}$). In $q_0$ it allows $\N$ 
	to generate the representation of any word $w\in \Sigma^*$, input of $\mathcal M$. 
	However, this intermediate representation is not suitable for mimicking $\mathcal M$.
	Thus in $q_1$, the intermediate representation is translated into an appropriate one.
	Once this representation is obtained, it mimics any transition of $\mathcal M$
	by triggering the firing of several transitions of $\N$. We will detail
	this simulation after the specification of $\N$.
	
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (10,0) node[draw,rectangle,minimum height=1.5cm,minimum width=4cm] () {};
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q0) {\small{$q_0$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q1) {\small{$q_1$}};
			\path (4,2) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q2) {};
			\path (4,-2) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q3) {};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q4) {\small{$\ell_0$}};
			\path (10,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q5) {\small{$\ell$}};
			\path (12,0) node[draw,circle,accepting,inner sep=2pt,minimum size=0.8cm] (q6) {\small{$\ell_f$}};
			
			
			\path (10,2) node[]  {\small{The simulation part of $\mathcal A$}};
			
			\path (9,0) node[]  {\small{$\cdots$}};
			\path (11,0) node[]  {\small{$\cdots$}};
			
			\draw[arrows=-latex'] (-1,0) -- (q0)  ;
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$next$}} ;
			\draw[arrows=-latex'] (q1) -- (3.5,1)--(q2) node[pos=0,left] {\tiny{$from_a$}} ;
			\draw[arrows=-latex'] (q2) -- (4.5,1)--(q1) node[pos=0,right] {\tiny{$to_a$}} ;
			\draw[arrows=-latex'] (q1) -- (3.5,-1)--(q3) node[pos=0,left] {\tiny{$from_b$}} ;
			\draw[arrows=-latex'] (q3) -- (4.5,-1)--(q1) node[pos=0,right] {\tiny{$to_b$}} ;
			\draw[arrows=-latex'] (q1) -- (q4) node[pos=0.5,above] {\tiny{$run$}} ;
			
			
			\draw[-latex'] (q0) .. controls +(55:60pt) and +(125:60pt) .. (q0)
			node[pos=.5,above] {\tiny{$t_a,t_b$}};
			
			
		\end{tikzpicture}
	\end{center}
	
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (4,1.2) node[]  {\small{$\delta(\ell,a)=(\ell',b,\rightarrow)$}};
			
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q0) {\small{$\ell$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q1) {};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q2) {\small{$\ell'$}};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$right_{a}^{\rightarrow}$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$left_{b}^{\rightarrow}$}} ;
			
			
			\path (12,1.2) node[]  {\small{$\delta(\ell,a)=(\ell',b,\leftarrow)$}};
			
			
			\path (10,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q10) {\small{$\ell$}};
			\path (14,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q11) {};
			\path (18,1) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q12) {\small{$\ell_{a,a}$}};
			\path (18,-1) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (r12) {\small{$\ell_{a,b}$}};
			\path (22,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q13) {\small{$\ell'$}};
			
			\draw[arrows=-latex'] (q10) -- (q11) node[pos=0.5,above] {\tiny{$upd_{a,b}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q11) -- (q12) node[pos=0.5,above] {\tiny{$left_{a}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q12) -- (q13) node[pos=0.5,above] {\tiny{$right_{a}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q11) -- (r12) node[pos=0.5,above] {\tiny{$left_{b}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (r12) -- (q13) node[pos=0.5,above] {\tiny{$right_{b}^{\leftarrow}$}} ;
			
			\path (4,-1.8) node[]  {\small{$\delta(\ell,\flat)=(\ell',b,\rightarrow)$}};
			
			
			\path (0,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q20) {\small{$\ell$}};
			\path (4,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q21) {};
			\path (8,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q22) {\small{$\ell'$}};
			
			\draw[arrows=-latex'] (q20) -- (q21) node[pos=0.5,above] {\tiny{$check_{\flat}$}} ;
			\draw[arrows=-latex'] (q21) -- (q22) node[pos=0.5,above] {\tiny{$left_{b}^{\rightarrow}$}} ;
			
			\path (12,1.2) node[]  {\small{$\delta(\ell,a)=(\ell',b,\leftarrow)$}};
			
			
			\path (10,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q30) {\small{$\ell$}};
			\path (13,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q30b) {};
			\path (16,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q31) {};
			\path (19,-2) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q32) {\small{$\ell_{\flat,a}$}};
			\path (19,-4) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (r32) {\small{$\ell_{\flat,b}$}};
			\path (22,-3) node[draw,circle,inner sep=2pt,minimum size=0.8cm] (q33) {\small{$\ell'$}};
			
			\draw[arrows=-latex'] (q30) -- (q30b) node[pos=0.5,above] {\tiny{$check_{\flat}$}} ;
			\draw[arrows=-latex'] (q30b) -- (q31) node[pos=0.5,above] {\tiny{$upd_{\flat,b}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q31) -- (q32) node[pos=0.5,above] {\tiny{$left_{a}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q32) -- (q33) node[pos=0.5,above] {\tiny{$right_{a}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (q31) -- (r32) node[pos=0.5,above] {\tiny{$left_{b}^{\leftarrow}$}} ;
			\draw[arrows=-latex'] (r32) -- (q33) node[pos=0.5,above] {\tiny{$right_{b}^{\leftarrow}$}} ;
			
			\path (12,-1.8) node[]  {\small{$\delta(\ell,\flat)=(\ell',b,\leftarrow)$}};
			
			
		\end{tikzpicture}
	\end{center}
	
	
	
	$\mathcal N$ is defined as follows.
	Its set of places is $P=\{p_a \mid a \in \Sigma\}\cup \{root,right,left,start,ret\}$.
	We now define the set of transitions $T$. The first subset 
	corresponds to the generation of a representation of the input word of  $\mathcal M$.
	\begin{itemize}[nosep]
		\item For all $a\in \Sigma$, $t_a\in T_{ab}$ with $W^-(t_a)=start$, $W^+(t_a)=ret$ and $\Omega(t_a)=start+p_a$;
		\item $next\in T_{el}$ with  $W^-(next)=start$ and $W^+(next)=ret$;
		\item For all  $a\in \Sigma$, $from_a\in T_{\tau}$  $W^-(from_a)=ret+p_a$;
		\item For all  $a\in \Sigma$, $to_a\in T_{ab}$ with  $W^-(to_a)=right$, $W^+(to_a)=right$ and $\Omega(to_a)=right+p_a$;
		\item $run\in T_{el}$ with $W^-(run)=root+ret$ and $W^+(run)=root$
	\end{itemize}
	
	The second subset corresponds to the simulation of $\mathcal M$.
	\begin{itemize}[nosep]
		\item For all $a\in \Sigma$, $right_{a}^{\rightarrow}\in T_{\tau}$ with $W^-(right_{a}^{\rightarrow})=right+p_a$;
		\item For all $a\in \Sigma$,  $left_{a}^{\rightarrow}\in T_{ab}$ with $W^-(left_{a}^{\rightarrow})=W^+(left_{a}^{\rightarrow})=left$\\  
		and $\Omega(left_{a}^{\rightarrow})=left+p_a$;
		\item For all $a,b \in \Sigma$,
		$upd_{a,b}^{\leftarrow}\in T_{el}$ with $W^-(upd_{a,b}^{\leftarrow})=right+p_a$ and $W^+(upd_{a,b}^{\leftarrow})=right+p_{b}$
		
		\item For all $a\in \Sigma$, $left_{a}^{\leftarrow}\in T_{\tau}$ with $W^-(left_{a}^{\leftarrow})=left+p_a$
		\item For all $a\in \Sigma$, $right_{a}^{\leftarrow}\in T_{ab}$ with $W^-(right_{a}^{\leftarrow})=W^+(right_{a}^{\leftarrow})=right$\\  
		and $\Omega(right_{a}^{\leftarrow})=right+p_a$
		\item $check_{\flat}\in T_{el}$ with  $W^-(check_{\flat})=W^+(check_{\flat})=right+root$;
		\item For all $b \in \Sigma$,
		$upd_{\flat,b}^{\leftarrow}\in T_{ab}$ with $W^-(upd_{\flat,b}^{\leftarrow})=right$, $W^+(upd_{\flat,b}^{\leftarrow})=right$\\
		and $\Omega(upd_{\flat,b}^{\leftarrow})=right+p_b$.
	\end{itemize}
	The initial state is $s[r,root+start+left+right]$. 
	
	Let us explain how the simulation works. 
	Let $abc$ be the word on the tape of $\mathcal M$. Then firing $(r,t_a)(v_1,t_b)(v_2,t_c)$ one gets:
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$root+left+right$}}] (q0) {\small{$r$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_a$}}] (q1) {\small{$v_1$}};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_b$}}] (q2) {\small{$v_2$}};
			\path (12,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_c+start$}}] (q3) {\small{$v_3$}};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$ret$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$ret$}} ;
			\draw[arrows=-latex'] (q2) -- (q3) node[pos=0.5,above] {\tiny{$ret$}} ;
			
		\end{tikzpicture}
	\end{center}
	
	After firing  $(v_3,next)(v_3,from_c)(r,to_c)(v_2,from_b)(u_1,to_b)(v_1,from_a)(u_2,to_a)(r,run)$ one gets:
	
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$root+left$}}] (q0) {\small{$r$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_c$}}] (q1) {\small{$u_1$}};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_b$}}] (q2) {\small{$u_2$}};
			\path (12,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_a+right$}}] (q3) {\small{$u_3$}};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q2) -- (q3) node[pos=0.5,above] {\tiny{$right$}} ;
			
		\end{tikzpicture}
	\end{center}
	
	Let us describe the two cases of tape simulation. Assume that the content of
	the tape is $abcd\flat^\omega$ and that the head of $\mathcal M$ is over $c$ then
	the corresponding state is the following one. The ``left'' branch contains the content of the tape
	on the left of the head while descending to the leaf and the ``right'' branch contains the relevant content of the tape
	on the right of the head (including the cell under the head) while ascending from the leaf. Thus
	the token in place $right$ points to the thread corresponding to the cell under the head
	while the token in place $left$ points to the thread corresponding to the cell immediately on the left
	of the head. The state of $\mathcal M$ is the state of $\mathcal A$.
	
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$root$}}] (q0) {\small{$r$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_d$}}] (q1) {};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_c+right$}}] (q2) {\small{$v$}};
			\path (-4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_a$}}] (q3) {};
			\path (-8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_b+left$}}] (q4) {\small{$u$}};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q0) -- (q3) node[pos=0.5,above] {\tiny{$left$}} ;
			\draw[arrows=-latex'] (q3) -- (q4) node[pos=0.5,above] {\tiny{$left$}} ;
			
		\end{tikzpicture}
	\end{center}
	
	Assume that the content of
	the tape is $abcd\flat^\omega$ and that the head of $\mathcal M$ is over the first $\flat$ then
	the corresponding state is the following one.
	
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$root+right$}}] (q0) {\small{$r$}};
			\path (-4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_a$}}] (q1) {};
			\path (-8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_b$}}] (q2) {};
			\path (-12,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_c$}}] (q3) {};
			\path (-16,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_d+left$}}] (q4) {};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$left$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$left$}} ;
			\draw[arrows=-latex'] (q2) -- (q3) node[pos=0.5,above] {\tiny{$left$}} ;
			\draw[arrows=-latex'] (q3) -- (q4) node[pos=0.5,above] {\tiny{$left$}} ;
			
		\end{tikzpicture}
	\end{center}
	It is routine to check that the simulation works. Let us illustrate it with one example.
	Assume that the content of
	the tape is $abcd\flat^\omega$,  the head of $\mathcal M$ is over $c$ and the current
	state is $\ell$. Let $\delta(\ell,c)=(\ell',e,\leftarrow)$.
	Then after firing $(v,upd_{c,e}^{\leftarrow})(u,left_{b}^{\leftarrow})(v,right_{b}^{\leftarrow})$, one gets:
	\begin{center}
		\begin{tikzpicture}[xscale=0.65,yscale=0.65]
			
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$root$}}] (q0) {\small{$r$}};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_d$}}] (q1) {};
			\path (8,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_e$}}] (q2) {\small{$v$}};
			\path (-4,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_a+left$}}] (q3) {};
			\path (12,0) node[draw,circle,inner sep=2pt,minimum size=0.8cm,
			label={[xshift=0cm, yshift=0cm]\tiny{$p_b+right$}}] (q4) {};
			
			\draw[arrows=-latex'] (q0) -- (q1) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q1) -- (q2) node[pos=0.5,above] {\tiny{$right$}} ;
			\draw[arrows=-latex'] (q0) -- (q3) node[pos=0.5,above] {\tiny{$left$}} ;
			\draw[arrows=-latex'] (q2) -- (q4) node[pos=0.5,above] {\tiny{$right$}} ;
			
		\end{tikzpicture}
	\end{center}
	For all $a\in \Sigma$, the homomorphism $h$ maps $t_a$ to $a$  
	and for all $t \notin \{t_a\}_{a\in \Sigma}$, $h$ maps $t$ to $\varepsilon$.
	
\end{proof}




Obviously, the family of RPNs coverability languages include the family of PNs coverability languages.
In~\cite{HP-icatpn99}, Proposition~1 establishes that the family of context-free languages is included
in family of reachability languages for RPNs. The proof relies on simulating the leftmost
derivations of a context-free grammar within particular two places $b_X$ and $e_X$
per nonterminal symbol $X$ where a token in $b_X$ means that $X$ must derived and
a token in $e_X$ means that the derivation of $X$ into a word has been achieved. In order to adapt
this result for the family of coverability languages for RPNs, it is enough to consider w.l.o.g. 
that the initial symbol $I$ never appears on the right hand side of a rule and to specify
$s[r,e_I]$ as final state. We refer the reader to~\cite{HP-icatpn99} for more details.
%In order to show its expressive power, let us introduce context-free
%grammars and languages. Let
%$G=(V,\Sigma,R,S)$ be a context-free grammar defined by
%$V$ the non terminal symbols including $S$, the start symbol and
%$\Sigma$ the terminal symbols.
%The set of rules $R$ is defined by
%$R=\{r_1,\ldots,r_n\}$ such that $r_i= (v_i,u_i)$,
%with $v_i\xrightarrow{r_i}  u_{i}$, $v_i\in V$ and $u_i\in (V \cup \Sigma)^*$
%a word of length $n_i$.
%W.l.o.g. one assumes that the start symbol $S$
%does not occur in the right-hand side of any production rule of $G$
%and that $n_i>0$ except possibly for a rule $S\rightarrow \varepsilon$.
%Given a word $\alpha v_i \beta \in (V \cup \Sigma)^*$, an application of rule $r_i$
%yields the word  $\alpha u_i \beta$, denoted
%$\alpha v_i \beta \xrightarrow{r_i} \alpha v_i \beta$. A \emph{derivation} from $\alpha$ to $\beta$ is a consecutive application
%of a sequence of rules, and is denoted $\alpha \xrightarrow{\sigma} \beta$.
%The associated language $\mathcal L(G)$ is defined by:
%$$\mathcal L(G)=\{w\in \Sigma^* \mid \exists\sigma\ S \xrightarrow{\sigma} w\}$$
%
%
%A \emph{leftmost derivation} always applies rules on the leftmost non terminal symbol
%of a word of $(V \cup \Sigma)^*$. Using only leftmost derivations let unchanged the language.

\begin{restatable}{proposition}{CFinRPN}
	%\begin{proposition}
	\label{prop:CFinRPN}
	The family of Context-free languages is included
	in the family of coverability languages of RPNs.
	%\alain{coverability or covering languages ?}
	%\end{proposition}
\end{restatable}
Since  universality is undecidable for the family of context-free languages, we deduce that universality of the family of RPN coverability languages is undecidable.	 

%\begin{proof}
%	Let $G=(V,\Sigma,R,S)$ be a context-free grammar.
%	We define a labelled marked net $\N$ as follows.
%	
%	\noindent $\bullet$ The set of places is defined
%	by:\\
%	\centerline{$P=\{b_v,e_v \mid v\in V\}\cup \{p_{i,j} \mid 1\leq i\leq n \wedge 0\leq j<n_i\}$}
%	
%	\noindent $\bullet$ $\mathcal{F} =\{m_v\}_{v\in V\setminus\{S\}}$ where $\ m_v(e_v)= 1$ and for all $p\neq e_v$, $m_v(p)=0$.
%	
%	\noindent $\bullet$ The set of transitions is defined by $T=\bigcup_{i\leq n} T_i$
%	where all abstract transitions\\
%	\hspace*{0.3cm}are labelled by $\varepsilon$ and:
%	\begin{itemize}[nosep]
%		%
%		\item If $n_i=0$ then $T_i=\{t_{i,0}\}$ with $W^-(t_{i,0})=b_{S}$
%		and $W^+(t_{i,0})=e_{S}$,\\
%		$t_{i,0}\in T_{el}$ and $\lambda(t_{i,0})=\varepsilon$;
%		%
%		\item Otherwise $T_i=\{t_{i,0},t_{i,1},\ldots,t_{i,n_i}\}$ with:
%		\begin{enumerate}[nosep]
%			%
%			\item  $W^-(t_{i,0})=b_{v_i}$ and $W^+(t_{i,0})=p_{i,0}$;
%			$t_{i,0}\in T_{el}$ and $\lambda(t_{i,0})=\varepsilon$;
%			%
%			\item  for all $1< j<n_i$ $W^ -(t_{i,j})=p_{i,j}$
%			and $W^+(t_{i,0})=p_{i,j+1}$;
%			%
%			\item  $W^-(t_{i,n_i})=p_{i,n_i-1}$ and $W^+(t_{i,n_i})=e_{v_i}$;
%			%
%			\item   for all $1< j\leq n_i$ if $u_{i,j}\in V$ then $t_{i,j}\in T_{ab}$ and
%			$\Omega(t_{i,j})=b_{u_{i}[j]}$\\
%			else $t_{i,j}\in T_{el}$, $\lambda(t_{i,j})=u_{i}[j]$.
%		\end{enumerate}
%		%
%	\end{itemize}
%	$\bullet$ The initial state is $s_0=s[r,b_S]$. 
%	We want to show that $\mathcal L(G)=\mathcal L(\N,s_0,\{s_f\})$
%	where $s_f=s[r,e_S]$.
%	
%	\smallskip \noindent
%	The result of a (possibly partial) leftmost derivation, not leading to empty word,
%	is represented by:
%	
%	\centerline{$(w,u_{i_k}[j_k,n_k],u_{i_{k-1}}[j_{k-1},n_{k-1}],\ldots,
%		u_{i_1}[j_1,n_1])$}
%	
%	\noindent
%	with
%	(1) for all $\ell\leq k$ $0<n_{\ell}$,
%	(2) $1\leq j_k\leq n_{k}+1$, and (3) for all $\ell<k$ $1<j_\ell\leq n_{\ell+1}$ where:
%	\begin{itemize}[nosep]
%		%
%		\item $w\in \Sigma^*$ is the subword already generated;
%		%
%		\item $(i_1,j_1)\cdots(i_k,j_k)$ are the current nested rules with the index
%		of the next symbol to be processed (none when $j_{\ell}=n_{\ell}+1$).
%		%
%	\end{itemize}
%	The leftmost derivations are simulated by the net as follows.
%	There is a firing sequence with trace $w$ leading
%	to a reachable state defined by:
%	\begin{itemize}[nosep]
%		%
%		\item if $k=0$ then  $s[r,e_{S}]$;
%		%
%		\item if $k\geq 1$ and $j_k=n_k+1$
%		then a single branch of length $k-1$
%		labelled by $t_{i_1,j_1-1},\ldots t_{i_{k-1}-1,j_{k-1}-1}$
%		with all markings empty except the last one consisting of a token in $e_{v_k}$;
%		%
%		\item if $k\geq 1$, $j_k\leq n_k$ and $u_{i_k}[j_k]\in \Sigma$
%		then a single branch of length $k-1$
%		labelled by\\$t_{i_1,j_1-1},\ldots t_{i_{k-1}-1,j_{k-1}-1}$
%		with all markings empty except the last one consisting of a token in $p_{i_k,j_k}$;
%		%
%		\item if $k\geq 1$, $j_k\leq n_k$ and $u_{i_k}[j_k]\in V$
%		then a single branch of length $k$
%		labelled by $t_{i_1,j_1-1},\ldots t_{i_{k},j_{k}-1}$
%		with all markings empty except the last one consisting of a token in $b_{u_{i_k}[j_k]}$;
%		%
%	\end{itemize}
%	
%	\noindent
%	Let us describe the simulation.
%	\begin{itemize}[nosep]
%		%
%		\item If $j_k\leq n_{k}$ and $u_{i_{k}}[j_{k}]\in V$ then the derivation
%		consists in choosing some rule\\ $r_{i_{k+1}}=u_{i_{k}}[j_{k}] \rightarrow u_{i_{k+1}}$
%		leading to
%		$(w,u_{i_{k+1}}[1,n_{k+1}],u_{i_k}[j_k+1,n_k],\ldots,
%		u_{i_1}[j_1,n_1])$.\\
%		This is simulated by the firing of elementary transition
%		$t_{i_{k+1},0}$ possibly followed by the firing of abstract transition $t_{i_{k+1},1}$
%		when $u_{i_{k+1}}[1]\in V$;
%		%
%		\item If $j_k\leq n_{k}$ and $u_{i_{k}}[j_{k}]\in \Sigma$ then the derivation
%		consists in concatenating the letter $u_{i_k}[j_k]$ to the word $w$
%		leading to
%		$(wu_{i_k}[j_k],u_{i_k}[j_k+1,n_k],u_{i_{k-1}}[j_{k-1},n_{k-1}],\ldots,
%		u_{i_1}[j_1,n_1])$.\\
%		This is simulated by the firing of elementary transition
%		$t_{i_{k},j_{k}+1}$ possibly followed by the firing of abstract transition $t_{i_{k},j_{k}+1}$
%		when $j_{k}+1\leq n_{k}$ and $u_{i_{k}}[j_{k}+1]\in V$;
%		%
%		\item If $j_k=n_{k}+1$ then the derivation
%		consists in deleting the empty word $u_{i_k}[j_k,n_k]$
%		leading to $(w,u_{i_{k-1}}[j_{k-1},n_{k-1}],\ldots,
%		u_{i_1}[j_1,n_1])$.\\
%		This is simulated by the cut transition in the leaf of the branch
%		producing the token specified by the postcondition of $t_{i_{k-1},j_{k-1}-1}$
%		possibly followed by the firing of abstract transition $t_{i_{k-1},j_{k-1}}$
%		when $j_{k-1}\leq n_{k-1}$ and $u_{i_{k-1}}[j_{k-1}]\in V$;
%		%
%	\end{itemize}
%	
%	
%	\noindent
%	The case of the empty word is straightforward.
%	
%	\noindent
%	Conversely the simulation from traces of firing sequences to words generated by (possibly partial)
%	leftmost derivations are done in a similar way.
%\end{proof}

Let  $\mathcal L_1=\{a^mb^nc^p \mid m\geq n \geq p\}$.
Denote by $\mathcal L_2 = \{w\tilde{w}\mid w\in \{d,e\}^*\}$ where $\tilde{w}$ is the mirror of $w$.
Let  $\mathcal L_3=\{a^nb^nc^n \mid  n \in \nat\}$.
Observe that given the final marking $p_f$ we get that the net in Figure~\ref{fig:PN_for_L1_and_L3} has $\mathcal L_1$ as its coverability language, and $\mathcal L_3$ its reachability language.

\begin{figure}[h]
		\begin{center}
		\begin{tikzpicture}[xscale=1,yscale=1]
			
			\path (0,0) node[] {$\bullet$};
			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p1) {};
			\path (1,0.5) node[] {$\varepsilon$};
			\path (1,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t1) {};
			\path (2,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p2) {};
			\path (3,0.5) node[] {$\varepsilon$};
			\path (3,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t2) {};
			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p3) {};
			\path (4,0.5) node[] {$p_f$};
			
			\path (0,-1.5) node[] {$a$};
			\path (0,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t3) {};
			\path (1,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p4) {};
			
			\path (2,-1.5) node[] {$b$};
			\path (2,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t4) {};
			\path (3,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p5) {};
			
			\path (4,-1.5) node[] {$c$};
			\path (4,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t5) {};
			
			\draw[arrows=-latex] (p1) -- (t1) ;
			\draw[arrows=-latex] (t1) -- (p2) ;
			\draw[arrows=-latex] (p2) -- (t2) ;
			\draw[arrows=-latex] (t2) -- (p3) ;
			
			\draw[arrows=-latex] (t3) -- (p4) ;
			\draw[arrows=-latex] (p4) -- (t4) ;
			
			\draw[arrows=-latex] (t4) -- (p5) ;
			\draw[arrows=-latex] (p5) -- (t5) ;
			
			\draw[arrows=-latex] (p1) -- (-0.2,-0.5)-- (t3) ;
			\draw[arrows=-latex] (t3) -- (0.2,-0.5)-- (p1) ;
			
			\draw[arrows=-latex] (p2) -- (1.8,-0.5)-- (t4) ;
			\draw[arrows=-latex] (t4) -- (2.2,-0.5)-- (p2) ;
			
			\draw[arrows=-latex] (p3) -- (3.8,-0.5)-- (t5) ;
			\draw[arrows=-latex] (t5) -- (4.2,-0.5)-- (p3) ;
			
			
		\end{tikzpicture}
	\end{center}
\caption{A Petri net for the languages $\mathcal L_1 $ and $ \mathcal L_3 $}
\label{fig:PN_for_L1_and_L3}
\end{figure}


\smallskip
The next proposition witnesses a Petri net language interesting from an expressiveness
point of view. A similar result can be found page~179 in Peterson's book~\cite{nla.cat-vn2956435}.
\begin{restatable}{proposition}{PNnotCF} 
	%\begin{proposition}
	\label{prop:PNnotCF}
	$\mathcal L_1$ is the coverability language of some Petri net but it
	is not a context-free language.
	%\end{proposition}
\end{restatable}

\begin{proof}
	Let us recall (a weak version of) Ogden lemma~\cite{ogden1968helpful}. For any context-free language
	$\mathcal L$ there exists an integer $N$ such for any word $w \in \mathcal L$
	with $N$ marked positions, there exists a decomposition
	$w=w_1w_2w_3w_4w_5$ such that $w_2w_4$ contains at least a marked position and
	for all $n\geq 0$, $w_1w_2^nw_3w_4^nw_5 \in \mathcal L$.
	
	\noindent
	The proof that $\mathcal L_1$ is not a context-free language is similar to the proof of the folk
	result that $\mathcal L_3$ is not a context-free language.
	Assume that $\mathcal L_1$ is a context-free language and consider
	the word $w=a^Nb^Nc^N$ with all $c$ positions marked.
	So let $w=w_1w_2w_3w_4w_5$ with the decomposition fulfilling the requirements
	of Ogden lemma. Since $w'=w_1w_2^2w_3w_4^2w_5\in \mathcal L_1$,
	$w_2$ and $w_4$ are mono-letter words. Furthermore one of these words
	is equal to $c^q$ for some $q>0$. If $w_2=c^q$ then $w_4=c^{q'}$
	and thus $w'$ contains too much $c$'s to belong to $\mathcal L_1$. If $w_4=c^q$ then either
	$w_2=a^{q'}$, $w_2=b^{q'}$ or $w_2=c^{q'}$. Whatever the case, $w'$ misses either $a$'s or $b$'s
	to belong to $\mathcal L_1$.
%	
%	\begin{center}
%		\begin{tikzpicture}[xscale=1,yscale=1]
%			
%			\path (0,0) node[] {$\bullet$};
%			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p1) {};
%			\path (1,0.5) node[] {$\varepsilon$};
%			\path (1,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t1) {};
%			\path (2,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p2) {};
%			\path (3,0.5) node[] {$\varepsilon$};
%			\path (3,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t2) {};
%			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p3) {};
%			\path (4,0.5) node[] {$p_f$};
%			
%			\path (0,-1.5) node[] {$a$};
%			\path (0,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t3) {};
%			\path (1,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p4) {};
%			
%			\path (2,-1.5) node[] {$b$};
%			\path (2,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t4) {};
%			\path (3,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p5) {};
%			
%			\path (4,-1.5) node[] {$c$};
%			\path (4,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t5) {};
%			
%			\draw[arrows=-latex] (p1) -- (t1) ;
%			\draw[arrows=-latex] (t1) -- (p2) ;
%			\draw[arrows=-latex] (p2) -- (t2) ;
%			\draw[arrows=-latex] (t2) -- (p3) ;
%			
%			\draw[arrows=-latex] (t3) -- (p4) ;
%			\draw[arrows=-latex] (p4) -- (t4) ;
%			
%			\draw[arrows=-latex] (t4) -- (p5) ;
%			\draw[arrows=-latex] (p5) -- (t5) ;
%			
%			\draw[arrows=-latex] (p1) -- (-0.2,-0.5)-- (t3) ;
%			\draw[arrows=-latex] (t3) -- (0.2,-0.5)-- (p1) ;
%			
%			\draw[arrows=-latex] (p2) -- (1.8,-0.5)-- (t4) ;
%			\draw[arrows=-latex] (t4) -- (2.2,-0.5)-- (p2) ;
%			
%			\draw[arrows=-latex] (p3) -- (3.8,-0.5)-- (t5) ;
%			\draw[arrows=-latex] (t5) -- (4.2,-0.5)-- (p3) ;
%			
%			
%		\end{tikzpicture}
%	\end{center}
%	
	\noindent
%	Consider the net above and the coverability language associated with the empty marking.
	As mentioned before the coverability language for the net in Figure~\ref{fig:PN_for_L1_and_L3} with final marking $p_f$ is $\mathcal L_1$.
%	It is routine to check that this language is /
\end{proof}



Using the previous results, the next theorem emphasises 
the expressive power of coverability languages of RPNs. 
\begin{theorem}\label{context-free}
	The family of coverability languages of RPNs strictly include
	the union of the family of coverability languages of PNs
	and the family of context-free languages.
\end{theorem}
\begin{proof}
	The inclusion is an immediate consequence of Proposition~\ref{prop:CFinRPN}.
	Consider the language
	$\mathcal L=\mathcal L_1 \cup \mathcal L_2$.
	
	\noindent
	Since (1) by Proposition~\ref{prop:closedunion}, the family of
	coverability languages of RPNs is closed under union,
	(2) $\mathcal L_1$  is a PN language, and
	(3) the language
	of palindromes is a context-free language, we deduce that $\mathcal L$ is an RPN language.
	
	\noindent
	PN and context-free languages are closed under homomorphism.
	Since the projection of $\mathcal L$ on $\{a,b,c\}$ is the language
	of Proposition~\ref{prop:PNnotCF}, $\mathcal L$ is not a context-free language.
	The projection of $\mathcal L$ on $\{d,e\}$ is the language
	of palindromes. Since it was seen in~\cite{Lambert92}  that the language of (2 letters) palindromes 
	is not a coverability language for any PN we are done.
%	$\mathcal L$ is not a PN language (see~\cite{Lambert92}).

\end{proof}

\input{reach-cov}

The transformation presented in the above proof can be performed in polynomial
time and this will be used in the next section.
The next proposition establishes that, as for Petri nets, coverability
does not ensure the power of ``exact counting''. The proof is interesting by itself
since it combines an argument based on WSTS (case 1) and an argument \emph{\`a la} Ogden (case 2). 


\begin{proposition}
	\label{prop:ReachPNnotCovRPN}
	
	$\mathcal L_3$ is the reachability language of the Petri net of Figure~\ref{fig:PN_for_L1_and_L3} but it
	is not the coverability language of any RPN.
\end{proposition}
\begin{proof}
	%We first introduce some additional notations: in a firing sequence $\sigma$
	%a thread is \emph{aborted} if it disappears due to a cut step
	%in some ancestor,  it is \emph{cut} if it disappears by performing a cut step.
	%
	%\smallskip \noindent
%	Consider the net below and $p_f$ be the single marking to be reached. Then its language
%	is $\mathcal L_3$.
	
%	\begin{center}
%		\begin{tikzpicture}[xscale=1,yscale=1]
%			
%			\path (0,0) node[] {$\bullet$};
%			\path (0,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p1) {};
%			\path (1,0.5) node[] {$\varepsilon$};
%			\path (1,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t1) {};
%			\path (2,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p2) {};
%			\path (3,0.5) node[] {$\varepsilon$};
%			\path (3,0) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t2) {};
%			\path (4,0) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p3) {};
%			\path (4,0.5) node[] {$p_f$};
%			
%			\path (0,-1.5) node[] {$a$};
%			\path (0,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t3) {};
%			\path (1,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p4) {};
%			
%			\path (2,-1.5) node[] {$b$};
%			\path (2,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t4) {};
%			\path (3,-1) node[draw,circle,inner sep=2pt,minimum size=0.4cm] (p5) {};
%			
%			\path (4,-1.5) node[] {$c$};
%			\path (4,-1) node[draw,rectangle,inner sep=2pt,minimum width=0.2cm,minimum height=0.4cm] (t5) {};
%			
%			\draw[arrows=-latex] (p1) -- (t1) ;
%			\draw[arrows=-latex] (t1) -- (p2) ;
%			\draw[arrows=-latex] (p2) -- (t2) ;
%			\draw[arrows=-latex] (t2) -- (p3) ;
%			
%			\draw[arrows=-latex] (t3) -- (p4) ;
%			\draw[arrows=-latex] (p4) -- (t4) ;
%			
%			\draw[arrows=-latex] (t4) -- (p5) ;
%			\draw[arrows=-latex] (p5) -- (t5) ;
%			
%			\draw[arrows=-latex] (p1) -- (-0.2,-0.5)-- (t3) ;
%			\draw[arrows=-latex] (t3) -- (0.2,-0.5)-- (p1) ;
%			
%			\draw[arrows=-latex] (p2) -- (1.8,-0.5)-- (t4) ;
%			\draw[arrows=-latex] (t4) -- (2.2,-0.5)-- (p2) ;
%			
%			\draw[arrows=-latex] (p3) -- (3.8,-0.5)-- (t5) ;
%			\draw[arrows=-latex] (t5) -- (4.2,-0.5)-- (p3) ;
%			
%			
%		\end{tikzpicture}
%	\end{center}
%	
	\noindent
	Due to Proposition~\ref{prop:cov-inc-reach}, it is enough to prove that there does not exist
	$(\N,s[r,m_0])$ such that $\mathcal L_3=\mathcal L_R(\N,s[r,m_0],\{\emptyset\})$.
	Assume  by contradiction that there exists such  $(\N,s[r,m_0]\})$.
	%Define the subset of abstract
	%transitions $T_\varepsilon$ such that for $t \in T_\varepsilon$ there exists
	%a firing sequence labelled by $\varepsilon$ starting
	%from a single thread marked by $\Omega(t)$ that reaches the empty tree.
	%Adding a set of elementary transitions $\{t_\varepsilon \mid t \in T_\varepsilon\}$
	%where $t$ and  $t_\varepsilon$ have same incidence and label does not modify the language
	%of the net.
	For all $n$, let $\sigma_n$ be a firing sequence reaching $\emptyset$
	such that $\lambda(\sigma_n)=a^nb^nc^n$
	and $\sigma'_n$ be the prefix of $\sigma_n$ whose last transition corresponds the last occurrence of $a$.
	Denote $s_n$ the state reached by $\sigma'_n$ and the decomposition by $\sigma_n=\sigma'_n\sigma''_n$.
	Among the possible $\sigma_n$, we select one such that $s_n$ has a minimal number of threads.
	Let $Post$ be the finite set of $\nat^P$ defined by: $Post=\{W^+(t)\}_{t\in T_{ab}}$.
	
	\begin{center}
		\begin{tikzpicture}[triangle/.style = {regular polygon, regular polygon sides=3 },xscale=0.45,yscale=0.45]
			
			
			
			\path (0,3.4) node[label={[xshift=0.0cm, yshift=-0.2cm]\small{$s[r,m_0]$}}] (s0) {$\bullet$};
			\path (8,0) node[draw,minimum size=3cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=0cm]$s_n$}] (sn) {};
			\path (16,3.4) node[] (fn) {$\emptyset$};
			%\path (16,-0.5) node[fill=black,draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.5cm, yshift=-0.5cm]\scriptsize{$Tr$}}] (tr) {};
			
			\draw[arrows=-latex'] (s0) -- (8,3.4) node[pos=0.5,above] {$\sigma'_n$} ;
			\draw[arrows=-latex'] (8,3.4) -- (fn) node[pos=0.5,above] {$\sigma''_n$} ;
			
			
			%\draw (16,3.4) -- (16,0) node[pos=0.6,right] {\scriptsize{$\!\!Br$}}node[pos=0.1,left] {\scriptsize{$s_f$}};
			
			\path (4,2.5) node[] {\scriptsize{$\sigma'_n=\rho t$}};
			\path (4,1.5) node[] {\scriptsize{$\lambda(\rho)=a^{n-1}$}};
			\path (4,0.5) node[] {\scriptsize{$\lambda(t)=a$}};
			\path (12,1.5) node[] {\scriptsize{$\lambda(\sigma''_n)=b^{n}c^n$}};
			\path (12,1.5) node[] {\scriptsize{$\lambda(\sigma''_n)=b^{n}c^n$}};
			%\path (20,2.5) node[] {\scriptsize{$ s_f\succeq s \in \mathcal F$}};
			%\path (20,1.5) node[] {\scriptsize{$f(s) = Tr$}};
			%\path (20,1) node[] {\tiny{when omitting markings}};
			\path (8,-2) node[] {\tiny{minimal number of threads of $s_n$}};
			
			
		\end{tikzpicture}
	\end{center}
	
	
	\noindent
	{\bf Case 1.} There exists a bound $B$ of the depths of the trees corresponding to $\{s_n\}_{n\in \nat}$.
	Let $S_B$ be the set of abstract states of depth at most $B$ and different from $\emptyset$. Observe that $S_0$
	can be identified to $\nat^P$
	and  $S_B$ can be identified to $\nat^P \times {\sf Multiset}(Post \times S_{B-1})$.
	Furthermore  the (component) order on $\nat^P$ and the equality on $Post$
	are well quasi-orders. Since well quasi-order is preserved by the multiset operation and the cartesian product,
	$S_B$ is well quasi-ordered by a quasi-order denoted $<$. By construction, $s\leq s'$ implies $s\preceq_r s'$. Thus there
	exist $n<n'$ such that $s_{n}\preceq_r s_{n'}$ which entails that $\sigma'_{n'}\sigma''_{n}$ is a firing
	sequence with trace $a^{n'}b^{n}c^{n}$ reaching $\emptyset$ yielding a contradiction.
	
	
	
	\noindent
	{\bf Case 2.} The depths of the trees corresponding to $\{s_n\}_{n\in \nat}$ are unbounded.
	%Let $C$ be a strict upper bound of the depths of the initial state and the final states.
	There exists $n$ such that the depth of $s_n$ is greater than $(2|Post|+1)$.
	%\alain{this last statement don't need that the depths are unbounded  but just that there exists at least one that is larger than $(2|Post|+1)$ ?}
	Thus in $s_n$ for $1\leq j\leq 3$, there are edges $u_j \xrightarrow{m}_{s_n}v_j$ 
	% in the same branch  such that $v_j$ is at level $i_jC$ with 
	and denoting $i_j$ the depth of $v_j$, one has $0<i_1<i_2<i_3$.
	% Denote $Tr$ the subtree of the final state of $\sigma_n$ that matches the state to be covered
	%and $Br$ the branch leading to $Tr$ in the final state.
	%Due to the choice of $C$, there exists $1 \leq \ell< 5$ such that:
	%\begin{itemize}[nosep]
	%%
	%    \item $Br_\ell$ and $Br_{\ell+1}$ the branches from $v_\ell$ to $v_{\ell+1}$ and from $v_{\ell+1}$ to $v_{\ell+2}$, do not intersect $Tr$;
	%%
	%    \item either $Br_\ell$ and $Br_{\ell+1}$ do not intersect $Br$ or $Br_\ell$  and $Br_{\ell+1}$ are included in $Br$.
	%%
	%\end{itemize}
	%We have illustrated below three possible situations (the other ones are similar). Observe that here we have merged the trees of $s_n$ and $s_f$.
	%For instance in the first figure, $v_6$ could have disappeared in $s_f$ while $T_r$ could not yet exist in $s_n$.
	%
	%\begin{center}
	%\begin{tikzpicture}[triangle/.style = {regular polygon, regular polygon sides=3 },xscale=0.45,yscale=0.45]
	%
	%\path (0,0) node[label={[xshift=-0.3cm, yshift=-0.4cm]$r$}] (r) {$\bullet$};
	%\path (0,-2) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_1$}] (v1) {$\bullet$};
	%\path (0,-4) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_2$}] (v2) {$\bullet$};
	%\path (0,-6) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_3$}] (v3) {$\bullet$};
	%\path (0,-8) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_4$}] (v4) {$\bullet$};
	%\path (0,-10) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_5$}] (v5) {$\bullet$};
	%\path (0,-12) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_6$}] (v6) {$\bullet$};
	%
	%\path (2,-6) node[fill=black,draw,minimum size=0.8cm,triangle,inner sep=0pt,
	%label={[xshift=0.5cm, yshift=-0.5cm]\scriptsize{$Tr$}}] (tr) {};
	%
	%\draw (r)[thick] -- (v1) ;
	%\draw (v1)[thick] -- (0,-3) ;
	%\draw (0,-3)[thick] -- (2,-5) node[pos=0.1,right] {\scriptsize{$Br$}};
	%\draw (v1) -- (v2) node[pos=0.5,left] {\scriptsize{$Br_1$}};
	%\draw (v2) -- (v3) node[pos=0.5,left] {\scriptsize{$Br_2$}};
	%\draw (v3) -- (v4) node[pos=0.5,left] {\scriptsize{$Br_3$}};
	%\draw (v4) -- (v5) node[pos=0.5,left] {\scriptsize{$Br_4$}};
	%\draw (v5) -- (v6) node[pos=0.5,left] {\scriptsize{$Br_5$}};
	%
	%\path (10,0) node[label={[xshift=-0.3cm, yshift=-0.4cm]$r$}] (dr) {$\bullet$};
	%\path (10,-2) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_1$}] (dv1) {$\bullet$};
	%\path (10,-4) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_2$}] (dv2) {$\bullet$};
	%\path (10,-6) node[] (dv3) {$\bullet$};
	%\path (10,-8) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_4$}] (dv4) {$\bullet$};
	%\path (10,-10) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_5$}] (dv5) {$\bullet$};
	%\path (10,-12) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_6$}] (dv6) {$\bullet$};
	%
	%
	%\path (10,-6) node[fill=black,draw,minimum size=0.8cm,triangle,inner sep=0pt,
	%label={[xshift=0.5cm, yshift=-0.5cm]\scriptsize{$Tr$}}] (tr) {};
	%
	%\draw (dr)[thick] -- (dv1) ;
	%\draw (dv2)[thick] -- (10,-5) ;
	%%\draw (10,-3)[thick] -- (12,-5) ;
	%\draw (dv1)[thick] -- (dv2) node[pos=0.5,left] {\scriptsize{$Br_1$}}node[pos=0.1,right] {\scriptsize{$Br$}};
	%\draw (dv2) -- (dv3) node[pos=0.5,left] {\scriptsize{$Br_2$}};
	%\draw (dv3) -- (dv4) node[pos=0.5,left] {\scriptsize{$Br_3$}};
	%\draw (dv4) -- (dv5) node[pos=0.5,left] {\scriptsize{$Br_4$}};
	%\draw (dv5) -- (dv6) node[pos=0.5,left] {\scriptsize{$Br_5$}};
	%
	%\path (20,0) node[label={[xshift=-0.3cm, yshift=-0.4cm]$r$}] (rr) {$\bullet$};
	%\path (20,-2) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_1$}] (tv1) {$\bullet$};
	%\path (20,-4) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_2$}] (tv2) {$\bullet$};
	%\path (20,-6) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_3$}] (tv3) {$\bullet$};
	%\path (20,-8) node[] (tv4) {$\bullet$};
	%\path (20,-10) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_5$}] (tv5) {$\bullet$};
	%\path (20,-12) node[label={[xshift=-0.3cm, yshift=-0.4cm]$v_6$}] (tv6) {$\bullet$};
	%
	%\path (20,-8) node[fill=black,draw,minimum size=0.8cm,triangle,inner sep=0pt,
	%label={[xshift=0.5cm, yshift=-0.5cm]\scriptsize{$Tr$}}] (tr) {};
	%
	%\draw (rr)[thick] -- (tv1) ;
	%\draw (tv2)[thick] -- (20,-5)node[pos=0.5,right] {\scriptsize{$Br$}} ;
	%\draw (tv1)[thick] -- (tv2) node[pos=0.5,left] {\scriptsize{$Br_1$}};
	%\draw (tv2)[thick] -- (tv3) node[pos=0.5,left] {\scriptsize{$Br_2$}};
	%\draw (tv3)[thick]  -- (tv4) node[pos=0.5,left] {\scriptsize{$Br_3$}};
	%\draw (tv4) -- (tv5) node[pos=0.5,left] {\scriptsize{$Br_4$}};
	%\draw (tv5) -- (tv6) node[pos=0.5,left] {\scriptsize{$Br_5$}};
	%
	%\path (-5,-1) node[] {\tiny{$(Br_3\cup Br_4)\cap (Br\cup Tr)=\emptyset$}};
	%\path (5,-1) node[] {\tiny{$(Br_4\cup Br_5)\cap (Br\cup Tr)=\emptyset$}};
	%\path (15,-0.5) node[] {\tiny{$(Br_1\cup Br_2)\subseteq Br $}};
	%\path (15,-1.5) node[] {\tiny{$(Br_1\cup Br_2)\cap Tr=\emptyset$}};
	%
	%\end{tikzpicture}
	%\end{center}
	
	
	\noindent
	For $k\in \{1,2,3\}$, consider of the sequence $\rho_k$ performed in the subtree rooted in $v_k$
	by the firings of $\sigma_n$. Among these three firing sequences two of them either (1)  both finish by a cut transition in $v_k$
	or (2) both do not finish by a cut transition in $v_k$. Let us call $i,j$ with $i<j$ the indices of these sequences and $w_i$  and $w_j$
	their traces. We have illustrated the situation below. 
	
	
	\begin{center}
		\begin{tikzpicture}[triangle/.style = {regular polygon, regular polygon sides=3 },xscale=0.45,yscale=0.45]
			
			
			
			\path (0,3.4) node[label={[xshift=0.0cm, yshift=-0.2cm]\small{$s[r,m_0]$}}] (s0) {$\bullet$};
			
			%\path (0,2.2) node[draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]$s_0$}] (s0) {};
			\path (6,1.7) node[draw,minimum size=1.5cm,triangle,inner sep=0pt,
			label={[xshift=-0.2cm, yshift=-0.7cm]{}}] (s1) {};
			\path (12,0.6) node[draw,minimum size=2.5cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (s2) {};
			\path (18,0) node[draw,minimum size=3cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-1.5cm]{}}] (sn) {};
			
			\path (30,3.4) node[] (fn) {$\emptyset$};
			%\path (30,-1) node[draw,minimum size=4cm,triangle,inner sep=0pt] (fn) {};
			
			\path (30,0.8) node[] (fn1) {$\:\:$};
			\path (30,-0.8) node[] (fn2) {$\:\:$};
			
			\path (12,-0.2) node[draw,color=blue,minimum size=1cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st2) {};
			
			\path (18,-0.8) node[draw,color=blue,minimum size=1.6cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st3) {};
			
			\path (18,-1.4) node[draw,color=red,minimum size=0.5cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su3) {};
			
			%\path (30,-1.8) node[draw,color=blue,minimum size=2.53cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st4) {};
			%
			%\path (30,-2.4) node[draw,color=red,minimum size=1.51cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su4) {};
			%
			%\path (30,-2.2) node[fill=black,draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.5cm, yshift=-0.5cm]\scriptsize{$Tr$}}] (tr) {};
			
			\draw[arrows=-latex'] (s0) -- (18,3.4) node[pos=0.5,above] {$\sigma'_n$} ;
			\draw[arrows=-latex'] (18,3.4) -- (fn) node[pos=0.5,above] {$\sigma''_n$} ;
			
			\draw[color=blue,arrows=-latex'] (6,0.8)  -- (fn1) node[pos=0.8,above] {$\rho_i$} ;
			\draw[color=red,arrows=-latex'] (12,-0.8)  -- (fn2) node[pos=0.7,above] {$\rho_{j}$} ;
			
			%\draw (30,3.4) -- (30,0) node[pos=0.6,right] {\scriptsize{$\!\!Br$}}node[pos=0.1,left] {\scriptsize{$s_f$}};
			
			\draw (6,3.4) -- (6,0.8);
			\path (6,0.8) node[label={[xshift=-0.3cm, yshift=-0.7cm]$v_i$}] {$\bullet$};
			
			\draw (12,3.4) -- (12,0.8);
			\path (12,0.8) node[] {$\bullet$};
			\path (12,-0.8) node[label={[xshift=-0.3cm, yshift=-0.7cm]$v_{j}$}] {$\bullet$};
			\draw (12,0.8) -- (12,-0.8);
			
			\path (18,0.8) node[] {$\bullet$};
			\path (18,-0.8) node[] {$\bullet$};
			\draw (18,0.8) -- (18,-0.8);
			
			%\path (30,0.8) node[] {$\bullet$};
			%\path (30,-0.8) node[] {$\bullet$};
			%\draw (30,0.8) -- (30,-1.2);
			
			
		\end{tikzpicture}
	\end{center}
	
	\noindent
	One can build two firing sequences that still reach $\emptyset$ and thus whose labels
	belong to the language. The first one consists of mimicking the ``behavior'' of the subtree rooted
	in $v_{j}$ starting from $v_i$, which is possible due to the choice of $i$ and $j$,  as illustrated below.
	
	\begin{center}
		\begin{tikzpicture}[triangle/.style = {regular polygon, regular polygon sides=3 },xscale=0.45,yscale=0.45]
			
			
			\path (0,3.4) node[label={[xshift=0.0cm, yshift=-0.2cm]\small{$s[r,m_0]$}}] (s0) {$\bullet$};
			
			%\path (0,2.2) node[draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]$s_0$}] (s0) {};
			\path (6,1.7) node[draw,minimum size=1.5cm,triangle,inner sep=0pt,
			label={[xshift=-0.2cm, yshift=-0.7cm]{}}] (s1) {};
			\path (12,1.1) node[draw,minimum size=2.1cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (s2) {};
			%\path (18,0) node[draw,minimum size=3cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-1.5cm]{}}] (sn) {};
			%\path (24,0) node[draw,minimum size=3cm,triangle,inner sep=0pt] (fn) {};
			\path (24,3.4) node[] (fn) {$\emptyset$};
			\path (24,0.8) node[] (fn1) {$\:\:$};
			
			%\path (12,-0.2) node[draw,color=blue,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st2) {};
			
			%\path (18,-0.8) node[draw,color=blue,minimum size=1.6cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st3) {};
			
			\path (12,0.2) node[draw,color=red,minimum size=0.5cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su3) {};
			
			%\path (30,-1.8) node[draw,color=blue,minimum size=2.53cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st4) {};
			
			%\path (24,-0.8) node[draw,color=red,minimum size=1.51cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su4) {};
			%
			%\path (24,-0.6) node[fill=black,draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.5cm, yshift=-0.5cm]{}}] (tr) {};
			
			\draw[arrows=-latex'] (s0) -- (fn) node[pos=0.5,above] {} ;
			%\draw[arrows=-latex'] (12,3.4) -- (24,3.4) node[pos=0.5,above] {} ;
			
			%\draw[color=blue,arrows=-latex'] (6,0.8)  -- (30,0.8) node[pos=0.8,above] {$\rho_i$} ;
			\draw[color=red,arrows=-latex'] (6,0.8)  -- (fn1) node[pos=0.7,above] {$\rho_{j}$} ;
			
			%\draw (24,3.4) -- (24,0) ;
			
			\draw (6,3.4) -- (6,0.8);
			\path (6,0.8) node[label={[xshift=-0.3cm, yshift=-0.7cm]$v_i$}] {$\bullet$};
			
			\draw (12,3.4) -- (12,0.8);
			\path (12,0.8) node[] {$\bullet$};
			%\path (12,-0.8) node[label={[xshift=-0.4cm, yshift=-0.7cm]$v_{i+1}$}] {$\bullet$};
			%\draw (12,0.8) -- (12,-0.8);
			
			%\path (18,0.8) node[] {$\bullet$};
			%\path (18,-0.8) node[] {$\bullet$};
			%\draw (18,0.8) -- (18,-0.8);
			
			%\path (24,0.8) node[] {$\bullet$};
			%\path (24,-0.8) node[] {$\bullet$};
			%\draw (24,0.8) -- (24,-1.2);
			
			
		\end{tikzpicture}
	\end{center}
	
	\noindent
	The second one consists of mimicking the ``behavior'' of the subtree rooted
	in $v_{i}$ starting from $v_{j}$ as illustrated below.
	
	\begin{center}
		\begin{tikzpicture}[triangle/.style = {regular polygon, regular polygon sides=3 },xscale=0.35,yscale=0.35]
			
			
			\path (0,3.4) node[label={[xshift=0.0cm, yshift=-0.2cm]\small{$s[r,m_0]$}}] (s0) {$\bullet$};
			
			%\path (0,2) node[draw,minimum size=1cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]$s_0$}] (s0) {};
			\path (6,1.3) node[draw,minimum size=1.5cm,triangle,inner sep=0pt,
			label={[xshift=-0.2cm, yshift=-0.7cm]{}}] (s1) {};
			\path (12,0.2) node[draw,minimum size=2.2cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (s2) {};
			\path (18,-0.7) node[draw,minimum size=2.8cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-1.5cm]{}}] (sn) {};
			
			\path (26,-1.4) node[draw,minimum size=3.3cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-1.5cm]{}}] (ssn) {};
			
			\path (36,3.4) node[] (fn) {$\emptyset$};
			\path (36,-1.4) node[] (fn1) {$\:\:$};
			\path (36,-2.7) node[] (fn2) {$\:\:$};
			
			%\path (36,-2.3) node[draw,minimum size=4cm,triangle,inner sep=0pt] (fn) {};
			
			\path (12,-0.9) node[draw,color=blue,minimum size=0.7cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st2) {};
			
			\path (18,-2.2) node[draw,color=blue,minimum size=0.7cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st2bis) {};
			
			\path (26,-3) node[draw,color=blue,minimum size=1cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st3) {};
			
			\path (26,-3.3) node[draw,color=red,minimum size=0.5cm,triangle,inner sep=0pt,
			label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su3) {};
			
			%\path (36,-3.9) node[draw,color=blue,minimum size=1.8cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (st4) {};
			%
			%\path (36,-4.3) node[draw,color=red,minimum size=1.2cm,triangle,inner sep=0pt,
			%label={[xshift=0.0cm, yshift=-0.7cm]{}}] (su4) {};
			%
			%\path (36,-4.4) node[fill=black,draw,minimum size=0.8cm,triangle,inner sep=0pt,
			%label={[xshift=0.5cm, yshift=-0.5cm]{}}] (tr) {};
			
			\draw[arrows=-latex'] (s0) -- (fn) node[pos=0.5,above] {} ;
			%\draw[arrows=-latex'] (18,3.4) -- (30,3.4) node[pos=0.5,above] {$\sigma''_n$} ;
			
			\draw[color=blue,arrows=-latex'] (6,0.2)  -- (12,0.2) node[pos=0.8,above] {} ;
			%\draw[color=red,arrows=-latex'] (12,-0.8)  -- (30,0-.8) node[pos=0.7,above] {$\rho_{j}$} ;
			
			\draw[color=blue,arrows=-latex'] (12,-1.4)  -- (fn1) node[pos=0.8,above] {$\rho_i$} ;
			\draw[color=red,arrows=-latex'] (18,-2.7)  -- (fn2) node[pos=0.7,above] {$\rho_{j}$} ;
			
			%\draw (36,3.4) -- (36,0);
			
			\draw (6,3.4) -- (6,0.2);
			\path (6,0.2) node[label={[xshift=-0.3cm, yshift=-0.7cm]$v_i$}] {$\bullet$};
			
			\draw (12,3.4) -- (12,0.2);
			\path (12,0.2) node[] {$\bullet$};
			\path (12,-1.4) node[label={[xshift=-0.4cm, yshift=-0.7cm]$v_{j}$}] {$\bullet$};
			\draw (12,0.8) -- (12,-1.4);
			
			\path (18,0.2) node[] {$\bullet$};
			\path (18,-1.4) node[] {$\bullet$};
			\path (18,-2.7) node[] {$\bullet$};
			\draw (18,0.2) -- (18,-2.7);
			
			\path (26,0.2) node[] {$\bullet$};
			\path (26,-1.4) node[] {$\bullet$};
			\path (26,-2.7) node[] {$\bullet$};
			\draw (26,0.2) -- (26,-2.7);
			
			%\path (36,0.2) node[] {$\bullet$};
			%\path (36,-1.4) node[] {$\bullet$};
			%\path (36,-2.7) node[] {$\bullet$};
			%\draw (36,0.8) -- (36,-3.3);
			
			
		\end{tikzpicture}
	\end{center}
	
	
	\noindent
	{\bf Case $w_i=w_{j}$.} Then the firing sequence reaching $\emptyset$ obtained by mimicking in $v_i$
	the behaviour of $v_{j}$ has trace $a^nb^nc^n$ 
	and leads to another state $s_n$ with less threads yielding a contradiction, since $s_n$ 
	was supposed to have a minimal number of threads.
	
	\noindent
	{\bf Case $w_i\neq w_{j}$.}  Let $w\neq \varepsilon$ be the trace of  the sequence performed in the subtree rooted in $v_i$
	without the  trace of  the sequence performed in the subtree rooted in $v_{j}$.
	Let us consider the firing sequence $\sigma$ reaching $\emptyset$ obtained by mimicking in $v_{j}$
	the behaviour of $v_{i}$. The trace of $\sigma$ is an interleaving of $a^nb^nc^n$ and $w$ and it belongs to $\mathcal L_3$
	which implies that $w=a^qb^qc^q$ for some $q>0$. Furthermore
	$\sigma$ can be chosen in such a way that the firing subsequences in the subtrees rooted at $v_i$ and $v_{j}$ are performed in one
	shot which implies that its trace is $\ldots a^qa^qw_{j}b^qc^q b^qc^q\ldots$ yielding a contradiction.
	
\end{proof}
The following corollary shows that extending the family of coverability languages of PNs by substituting either (1) coverability by reachability or (2) PNs by RPNs is somewhat ``orthogonal''.
%The following corollary shows that extending coverability languages
%of Petri nets substituting (1) coverability by reachability
%or (2)  Petri nets by RPNs are somewhat ``orthogonal''.
\begin{corollary}
	\label{cor:ReachPNuncompCovRPN}
	The families of reachability languages of Petri nets and
	the family of coverability languages of RPNs are incomparable.
\end{corollary}
\begin{proof}
	One direction is a consequence of Proposition~\ref{prop:ReachPNnotCovRPN}
	while the other direction is a consequence of Proposition~\ref{prop:CFinRPN}
	observing that the language of palindromes is not the reachability
	language of any Petri net.
\end{proof}
The next corollary exhibits a particular feature of RPNs languages
(e.g.  Petri nets  or context-free languages are closed under intersection with a regular language).
\begin{corollary}\label{col:intersection_rpn_and_regular}
	The family of coverability languages of RPNs is not closed under
	intersection with a regular language and under complementation.
\end{corollary}
\begin{proof}
	Due to Proposition~\ref{prop:ReachPNnotCovRPN},
	the family of coverability languages of RPNs
	is strictly included in the family of recursively enumerable languages.
	Since the former family is closed under homomorphism, Theorem~\ref{theo:re}
	implies that it is not closed under intersection with a regular language and a fortiori 
	with another coverability language.
	Since intersection can be obtained by union and complementation and since the family of RPN coverability languages is closed
	under union, they are not closed under complementation.
	
\end{proof}

Combining Propositions~\ref{prop:reach-inc-cov},~\ref{prop:cov-inc-reach} and~\ref{prop:ReachPNnotCovRPN}, one gets the following theorem.
\begin{theorem}
	The family of coverability languages of RPNs is strictly included
	in the family of reachability languages of RPNs.
\end{theorem}
Figure~\ref{fig:lang_compare} illustrates the hierarchy of the languages presented in this work. 
\begin{figure}[h]
	\input{lan_compare.tex}
	\caption{$\mathcal L_1 =\{a^mb^nc^p\mid m\geq n\geq p \};\mathcal  L_2= \{w\in\{d,e\}^* \mid w=\widetilde{w}\};\mathcal  L_3 = \{a^nb^nc^n\mid n\in\nat\}  $}
		\label{fig:lang_compare}
\end{figure}





%\alain{to compensate for this negative result, what would be the subclass of regular languages $L$ such that $L$ intersected with an RPN would be still an RPN ?}

%\begin{proof}
%	Assume for contradiction that the universality of RPN coverability languages is decidable. By Theorem \ref{theo:re} for any recursively enumerable language $\mathcal L$ there exist and RPN coverability language $\mathcal L'$, a regular language $ \mathcal R_2$ and a homomorphism $h$ such that $\mathcal L = h(\mathcal L' \cap \mathcal R_2 )$. Therefore since the universality for regular languages is decidable we get that determining the universality of $\mathcal L$ is also decidable. \alain{why ??? explain your reasonning because I don't understand how you reach the conclusion. I ithink that your reasonning is  $L=\Sigma^*$ iff $L'=\Sigma^*$ and $\mathcal R_2 =\Sigma^*$ and $h(\Sigma^*)=\Sigma^*$ but I am not sure that $L'$ has the same alphabet than $L$. I may imagine .$L=a^*$ and $L'=\{a^nb^m, m \leq n\}$ and $\mathcal R_2 =a^*$ and $h(a)=a, h(b)=\epsilon$ and $L$ is universal but $L'$ is not.}: But since it is a known result that universality of recursively enumerable languages is undecidable we get a contradiction. 
%\end{proof}

%\begin{corollary}
%	The word problem in of RPN coverability languages is decidable.	 
%\end{corollary}




%- is it true that $L_C(RPN) \subseteq L_R(RPN)$ ? \\


%\alain{make a figure showing the inclusions and incomparabilities between classes of languages}

%\igor{Is Fig \ref{fig:lang_compare} good? }
%\alain{I would suggest to put four color or hash/... to simplify the view of the sets}

% \alain{From the last result, we know that ReachPN $\neq$ CoverRPN.
% Do we know more on the relations between ReachPN and CoverRPN ?
% Whether one is included in the other or may there is no inclusion ?
% Do we know if CoverRPN $\neq$ ReachRPN ?}

%
%\igor{
%	\begin{proposition}
%		The family of RPN coverability languages is closed under concatenation and Kleen star.
%	\end{proposition}
%}
%\begin{figure}[h]
%	\input{concatination_Kleen}
%	\caption{The RPN $\N$  for which $\mathcal{L}_R(\N,s[r,p_I],\{\emptyset\}) = \mathcal{L}_1\cdot\mathcal{L}_2^*\cdot\mathcal{L}_3$, where $\mathcal{L}_i =\mathcal{L}_R(\N_1,s[r_i,m_i],\{\emptyset\}) $. The squares in the figure with $\N_i$ are a short hand for the entire structure of $\N_i$.}\label{fig:conc_kleen}
%\end{figure}
%\igor{
%	We do not prove of this corollary, but let us try to give the intuition. Using the rooted RPN and the equality to the family to cut languages, it is a straight forward construction. See for example Figure\ref{fig:conc_kleen}.
%}
%
%



==> finitness-2.tex <==
% !TEX root =main.tex
\section{Finiteness and boundedness are \EXPSPACE-complete}
\label{sec:finiteness}
In this section we will show that the finiteness and boundedness problems for RPNs are $\EXPSPACE$-complete w.r.t. $\eta=size(\N,s_{0})$, i.e. the accumulated size of the RPN and the initial state. 
For Petri nets the finiteness problem, which is equivalent to the boundedness problem, has been shown to be $\EXPSPACE$-complete:
\begin{theorem}[\cite{Lipton76,Rac78}]
	\label{thm:Finiteness Bound For PN }The finiteness problem for Petri
	nets is $\EXPSPACE$-complete.
\end{theorem}
$\EXPSPACE$-hardness follows immediately from  $\EXPSPACE$-hardness of the finiteness problem for Petri nets~\cite{Lipton76}. 

Moreover by applying Proposition~\ref{col:rooted} like in previous sections we will assume that $s_0=s[r,m_0]$.
Given two vertices $u,v$ in a graph $\mathcal G$, the \emph{distance} between them $dist_{\mathcal G}(u,v)$ is
the length of a shortest path going from one to the other.

\begin{lemma} \label{lem:Form a path in ab to a path in RPN}
	Let $(\N,s_0)$ be a marked RPN and $G_{\N,s_{0}}=(V_a,E_a,M_a)$ be its abstract graph. Then for all $v\in V_a$, there exists $s\in Reach(\N, s_{0})$ and $u\in V_s $ such that $ M_s(u)=M_a(v)$.
\end{lemma}

\begin{proof}
	We show the lemma by induction on $dist_{G_{\N,s_{0}}}(r,u)$. If $dist_{G_{\N,s_{0}}}(r,v) =0$ then $v=r$ and $M_a(r)=m_0$.	
	Assume that we have shown the lemma for any $v$ such that $dist_{G_{\N,s_{0}}}(r,v)<n$, and pick $v\in V_a$ such that $dist_{G_{\N,s_{0}}}(r,v)=n$. Since $dist_{G_{\N,s_{0}}}(v,r)>0$, $v=v_t$ for some $t\in T_{ab}$. Moreover there is some $(u,v_t)\in E_a$ such that $dist_{G_{\N,s_{0}}}(r,u)=n-1$ and by the induction hypothesis there is a sequence $s_{0}\xrightarrow{\sigma_u}s_u$ and some $w\in V_{s_u}$ such that $M_{s_u}(w)=M_a(u)$. From the definition of $G_{\N,s_{0}}$ there is a fireable sequence $ s[w,M_a(w)]\xrightarrow{\sigma_t(w,t)}$. Combining these sequences, we get $s_{0}\xrightarrow{\sigma_u}s_u\xrightarrow{\sigma_t(w,t)}s_{v_t}$, where the newly created thread $w'$ fulfills $M_{s_v}(w')=\Omega(t)=M_a(v_t)$.
\end{proof}
The following lemma shows that we can simulate the behaviour of every thread by a Petri net. 
\begin{lemma} \label{lem:every marking is covered by ab graph}
	Let $(\N,s_{0})$ be a marked RPN and $G_{\N,s_{0}}=(V_a,E_a,M_a)$ be its abstract graph.
	Then:
	$$
	\bigcup_{s\in Reach(\N,s_{0})}\{M_s(v) \}_{v\in V_s}= \bigcup_{u\in V_a} Reach(\widehat{\N}_{el}, M_a(u)).
	$$
\end{lemma}


\begin{proof}
	
	\noindent $\bullet$ Let $m\in\bigcup_{s\in Reach(\N,s_{0})}\{M_s(u) \}_{u\in V_s} $. There exists $s_0\xrightarrow{\sigma}s$ with some $v\in V_s $ such that  $M_s(v)=m$. By Proposition~\ref{prop:omniciant} there is an omniscient sequence in $s_0\xrightarrow{\widehat{\sigma}}_{\widehat{\N}}s$. We split $\widehat\sigma$ into $s_0\xrightarrow{\widehat{\sigma}_1}_{\widehat{\N}}s_v\xrightarrow{\widehat{\sigma}_2}_{\widehat{\N}}$ where $s_v$ is the the state where the thread $v$ first appears. Note that there is $u\in V_a$ for which $M_{s_v}(v) = M_a(u)$. Let $(v,\widehat{\sigma}_2')$ consisting of all firings
	of $v$ in $\widehat{\sigma}_2$. $(v,\widehat{\sigma}_2')$ is fireable from $s_v$ since $\widehat{\sigma}_2$ is omniscient implying that there will be not cut transition fired by a child of $v$. By construction of $\widehat{\N}_{el}$, the sequence $\widehat{\sigma}_2'$ is a firing sequence
	of $(\widehat{\N}_{el},M_a(u))$ thus $ m\in Reach(\widehat{\N}_{el}, M_a(u))$.
	
	\noindent $\bullet$ Let $u\in V_a $ and $m\in Reach(\widehat{\N}_{el}, M_a(u))$, i.e. $M_a(u)\xrightarrow{\sigma}_{\widehat{\N}_{el}}m$ for some $n\in \nat$. First by Lemma~\ref{lem:Form a path in ab to a path in RPN} there exists $s_0\xrightarrow{\sigma_u}_\N s_u$ where for some $v\in V_{s_u}$ we have $M_{s_u}(v) = M_a(u)$. By construction of $\widehat{\N}$ we also have $s_0\xrightarrow{\sigma_u}_{\widehat{\N}} s_u$. By  construction of $\widehat{\N}_{el}$ we get that $s_u\xrightarrow{(v,\sigma)}_{\widehat{\N}}s$ where $M_s(v) = m$. By Proposition~\ref{prop:equivreach}, $s\in Reach(\N,s_{0})$, which concludes the proof.
	
	%	Due to Proposition \ref{prop: translating from RPN to sim}, there is a \wellOrd\ sequence $s_{0}\xrightarrow{\widehat{\sigma}}s$.
	%	In $\widehat{\sigma}$ there is a contiguous subsequence $\sigma_{v}\sigma^{ab}_{v}\sqsubseteq \widehat{\sigma}$ where all the elementary (resp. abstract) firings of thread $v$ are performed in $\sigma_v$ (resp. $\sigma_v^{ab}$). Denote by $s_v$ the state from which $\sigma_{v}\sigma^{ab}_{v}$ is fired. 
	%	The thread $v$ is either the root $r$ or it was created by an abstract transition $t$. 
	%	If $v=r$, then  $M_{s_v}(v)= M_a(v)$, otherwise $v$ was created by an abstract transition then $M_{s_v}(v)=\Omega(t)= M_a(v)$.
	%	Therefore by denoting $\sigma_{v}\sigma^{ab}_{v} = (v,t_i)_{i=1}^n$ we get that $(t_i)_{i=1}^n$ is a sequence in $\widehat{\N}_{el}$. It is fireable from the marking $M_{s_v}(v) = M_a(v)$ hence 
	%	\centerline{$
	%			M_a(v)\xrightarrow{\sigma'} M_a(v)+\sum_{i\leq n}W^+(t_i) - W^-(t_i) = M_s(v)
	%		$}
\end{proof}
Using the previous Lemma and Rackoff's Theorem we establish the complexity of the boundedness problem:
\begin{proposition}
	The boundedness problem of RPN is \EXPSPACE-complete.
\end{proposition}
\begin{proof}
	Hardness of the problem comes from hardness of Petri nets.
	Let $(\N,s_0)$ be a marked RPN. First by Corollary~\ref{col:rooted} we can assume that $s_0 = s[r,m_0]$.
	By Lemma \ref{lem:every marking is covered by ab graph} checking whether $\N,s_0$ is bounded
	is equivalent to whether for $v \in V_a$, $(\widehat{\N}_{el}, M_a(u))$ is bounded which, due to Rackoff,
	can be performed in exponential space.
	
	
\end{proof}

Let $(\N,s_{0})$ be a marked RPN. If $s_{0}=\emptyset$ then the number of reachable states is finite (one), hence from now on we  assume that $s_{0}\neq\emptyset$. Next, if there exists $t\in T_{ab}$ with $W^-(t)=0$ then there are infinitely many reachable states since one can fire $t$ repeatedly which provides us with a sequence of states with an unbounded number of threads. Therefore from now on we  assume that for all $t\in T_{ab}$, $W^-(t)>0$.

We now establish a connection between the boundedness of $\widehat{\N}_{el}$ and the maximal number of children of the root in $\N$: 
\begin{lemma}\label{lem:bounded num of children}
	Let $\N$ be an RPN such that $(\widehat{\N}_{el},m_0)$ is bounded. Then: 
	\[
	\sup_{s'\in Reach(\N,s[r,m_0])}|\{v\in V_{s'}\mid r_{s'}\rightarrow_{s'} v\}|< \infty
	\] 
\end{lemma}

\begin{proof}
	Assume that there exists a family of sequences $ \{\sigma_n\}_{n\in\nat} $ such that $s[r,m_0]\xrightarrow{\sigma_n}_{\N}s_n$ and the number of children of $r$ in $s_n$ is greater than $n$. By Proposition~\ref{prop:omniciant} for all $\sigma_n$ there exists an omniscient sequence $\widehat{\sigma}_n$ in $\widehat{\N}$ from $s[r,m]$ reaching $s_n$. We remove from $\widehat{\sigma}_n$ all the transitions not fired from the root getting $(r,\widehat{\sigma}_n')$ which is also fireable from $s[r,m]$ and which leads to a state where the root has a number of children greater than $n$. Since an abstract transition consumes tokens from the root (for all $t\in T_{ab}$, $W^-(t)>0$) one can remove them from  $(r,\widehat{\sigma}_n')$ and get $(r,\widehat{\sigma}_n'')$ for which $s\xrightarrow{(r,\widehat{\sigma}_n'')}_{\widehat{\N}}s_n''$ and $\sum_{p\in P}M_{s_n''}(r)(p)>n$.
	Since $ \widehat{\sigma}_n''$ is fireable from $m$ in $\widehat{\N}_{el}$ this contradicts the hypothesis of the lemma.	
\end{proof}
Combining the above results, we get a characterization of the  finiteness problem:

\begin{proposition}\label{prop:const finitness is equvalent to}
	Let $(\N,s_{0})$ be a marked RPN. Then $Reach(\N, s_{0})$ is finite if and only if both of the following assertions hold:\\
	%	\begin{enumerate}[nosep]
	1. There is no loop in $G_{\N,s_{0}}=(V_a,E_a,M_a)$;\\
	2. For all $v\in V_a$, $(\widehat{\N}_{el},M_a(v))$ is bounded.
	%	\end{enumerate}
\end{proposition}
\begin{proof}
	$\bullet$ Assume that assertions 1 and 2 hold. Due to Assertion~1 and Lemma~\ref{lem:Finidng unbounded path using at} any reachable state has its depth bounded by some constant. Due to Assertion~2 and Lemmas~\ref{lem:every marking is covered by ab graph} and~\ref{lem:bounded num of children} each thread in any reachable state has a bounded number of children, and a bounded number of different reachable markings. Therefore $Reach(\N,s_0)$ is finite.\smallskip	
	
	\noindent $\bullet$ Assume that Assertion~1 does not hold. By Lemma~\ref{lem:Finidng unbounded path using at} there is a deep infinite sequence. Hence there is an infinite sequence of states with growing depth. Therefore $Reach(\N,s_0)$ is not finite.
	
	\noindent $\bullet$ Assume that Assertion~2 does not hold for some vertex $v$. By Lemma~\ref{lem:Form a path in ab to a path in RPN} there exists a state $s\in Reach(\N, s_{0})$ and a vertex $u\in V_s $ such that $ M_s(u)=M_a(v)$. By the definition of $\widehat{\N}_{el}$, for any $m\in Reach(\widehat{\N}_{el},M_s(v))$, there exists a firing sequence $(r,\sigma')$ in $\widehat{\N}$ such that $s\xrightarrow{(r,\sigma')}_{\widehat{\N}}s'$ with $M_{s'}(v)=m$. Therefore $Reach(\widehat{\N},s)\subseteq Reach(\widehat{\N},s_0)$. Due to Proposition~\ref{prop:equivreach}, $Reach(\widehat{\N},s_0)= Reach(\N,s_0)$.
	%	\igor{not double contradiction (not a equiv b)}
	%	$\bullet$ $Reach(\N, s_{0})$ is finite.
	%	
	%	\noindent Assume by contradiction that there exists a loop in $G_{\N,s_{0}}$. Due to Lemma \ref{lem:Finidng unbounded path using at}   there is a deep infinite sequence, denoted $\sigma$. 
	%	In the states visited by $\sigma$ there are some unbounded branches. This implies that $Reach(\N, s_{0})$  is infinite which is a contradiction.	
	%	
	%    \noindent Assume by contradiction that there exists $v\in V_a$ such that $(\widehat{\N}_{el},M_a(v))$ is unbounded. 
	%	Due to Lemma \ref{lem:Form a path in ab to a path in RPN} there is a constrained sequence $s_{0}\xrightarrow{\sigma}s$ with $u\in V_s$ such that $M_s(u)=M_a(v)$.
	%	Due to Proposition \ref{prop:Length of an abstract transition in RPN}, any sequence $\sigma$ in $\widehat{\N}_{el},M_a(u)$ can be translated to a sequence $\sigma'$ in $\N,s[u,M_a(u)]$, by replacing any $t_r\in \sigma$ by the appropriate $\sigma_{t_r}$. So, the infinite set of reachable markings in $\widehat{\N}_{el},M_a(v)$ are also markings of reachable states from $s$, and hence from $s_{0}$, which is a contradiction.  
	%	
	%	\smallskip
	%	\noindent $\bullet$ $ConstReach(\N, s_{0})$ is infinite.
	%	
	%	\noindent Assume by contradiction that assertions 1 and 2 hold. 
	%	Since there is no reachable loop in $G_{\N,s_{0}}$ all states reachable by a constrained sequence from $s_{0}$ have depth bounded by the maximal length of paths in $G_{\N,s_{0}}$, denote by $D$.  	
	%	
	%	\noindent Due to the Lemma \ref{lem:bounded num of children} there exists $B\in \nat $ such that for any $v\in V_a$ and for any firing sequence from $s[v,M_a(v)]$ the root has at most $B$ children. Thus any vertex of $s\in ConstReach(\N, s_{0})$ has at most $B$ children. Therefore any state has at most $B^{D+1}$ vertices. 
	%	Due to Assertion 2 and Lemma \ref{lem:every marking is covered by ab graph} there exists $C\in\nat$ such that:\\
	%	\centerline{$C= \left|\{ m\mid \exists s\in ConsReach(\N,s_{0}) , \exists u\in V_s, m= M_s(u) \}\right|$
	%	}	
	%	Denote by $\alpha$ the number of tree structures (labeled by $T_{ab}$) with at most $B^{D+1}$ vertices. Then \\
	%	\centerline{ $|ConstReach(\N, s_{0})|<\alpha C^{B^{D+1}}$}
\end{proof}



\begin{theorem}
	\label{prop:constraind finitness in EXPSPACE}
	The finiteness problem of RPN is \EXPSPACE-complete.
\end{theorem}

\begin{proof}
	The algorithm proceeds by checking Assertions~1 and~2 of Proposition\ref{prop:const finitness is equvalent to}.
	It builds in exponential space (by Lemma~\ref{lem:abstract graph in expspace}) the \at\ graph and
	checks whether there is no loop in $G_{\N,s_{0}}$.
	In the negative case, it checks in exponential space for any vertex $v\in V_a$, whether
	the marked Petri net $(\widehat{\N}_{el},M_{a}(v))$
	is bounded.	
\end{proof}
%We now conclude that the finiteness problem is \EXPSPACE\ by reducing it in \EXPSPACE\ 
%to an exponential
%number of instances of the constrained finitness problem with similar size:
%\begin{theorem}\label{thm:finitness}
%	The finiteness problem of RPN is \EXPSPACE-complete.
%\end{theorem}
%
%\begin{proof}
%	Let $(\N,s_{0})$ be a marked RPN.
%	W.l.o.g. we assume that $\N$ has been enlarged to $\widehat{\N}$
%	since the finiteness problem remains unchanged
%	by this transformation.	
%	For any $U\subseteq V_{s_{0}}$ closed by the descendent relation, denote by \\
%	\centerline{ $Reach_U(\N,s_{0}) = \{s\in Reach(\N,s) \mid  V_s\cap V_{s_{0}} = V_{s_{0}}\!\!\setminus\! U  \}$
%	}
%	and note that  $ Reach(\N,s_{0})= \bigcup_{\text{closed }U\subseteq V_{s_{0}}} Reach_U(\N,s_{0}) $. Hence, $Reach(\N,s_{0})<\infty$ if and only if for all $U\subseteq V_{s}$ closed, $Reach_U(\N,s_{0}) <\infty$.
%	By Proposition \ref{prop: translating from RPN to sim} given $s\in Reach_U(\N,s_{0})$ there exists a \wellOrd\ firing sequence, such that $s_{0}\xrightarrow{\sigma_U}s_{0}\backslash U\xrightarrow{\sigma'}s$. Hence if $s_{0}\backslash  U$ is reachable then $Reach_U(\N,s_{0}) = ConstReach(\N,s_{0}\backslash  U)$ and otherwise $ Reach_U(\N,s_{0}) = \emptyset $. 
%By Proposition~\ref{prop:reacabilty of s_u}, we can check in \EXPSPACE, whether $s_{0}\backslash  U$ is reachable, and in the positive case solve in \EXPSPACE, the constrained finiteness problem for $(\N,s_{0}\backslash U)$.
%\end{proof}



==> introduction.tex <==
% !TEX root =main.tex
\section{Introduction}
\label{sec:introduction}

{\bf Verification problems for Petri nets.}
Petri net is a useful formalism for the analysis of concurrent programs
for several reasons. From a modeling
point of view (1) due to the locality of the firing rule, one easily models
concurrent activities and (2) the (a priori) unbounded marking of places allows
to represent a dynamic number of activities. From a verification point of view,
most of the usual properties are decidable. However, Petri nets suffer
two main limitations: they cannot model recursive features and the computational
cost of verification may be very high. More precisely,
all the known algorithms solving reachability
are nonprimitive recursive (see for instance~\cite{Mayr84})
and it has been proved recently that the reachability
problem is non elementary~\cite{abs-1809-07115} but primitive recursive when
the dimension is fixed~\cite{DBLP:conf/lics/LerouxS19}.
Fortunately some interesting properties like coverability,
termination, finiteness, and boundedness are \EXPSPACE-complete~\cite{Rac78}
and thus still manageable by a tool. So an important research direction
consists of extending Petri nets to support new modeling features
while still preserving decidability of properties checking and if possible with a "reasonable" complexity.


\noindent
{\bf Extended Petri nets.}
Such extensions may be partitioned between those whose states are still markings
and the other ones.
The simplest extension consists of adding inhibitor arcs
which yields undecidability of most of the verification problems.
However adding a single inhibitor arc preserves the decidability of
the reachability, coverability, and boundedness problems~\cite{Reinhardt08,BFLZ-lmcs12,Bonnet11}.
When adding reset arcs, the coverability problem becomes
Ackermann-complete ~\cite{PhS-mfcs10} and boundedness undecidable~\cite{dufourd98}
%		\alain{I modify the reference}.
%Post-self-modifying nets are obtained by specifying the weight of the
%output arcs of a transitions as an affine function of the current marking:
%their coverability and boundedness problems belong to \EXPSPACE\ \cite{BFP-fsttcs12}.

In $\nu$-Petri nets, the tokens are colored where colors are picked in
an infinite domain: their coverability problem is double-Ackermann
%			\alain{I add a - between double and Ackermann}
time
complete~\cite{lazic:hal-01265302}.
%In Petri nets equipped with a stack, the reachability and coverability problems
%are not only
%\TOWER-hard~\cite{abs-1809-07115,Lazic13}
%but their decidability status is still unknown.
In Petri nets with a stack, the reachability problem may be reduced
to the coverability problem and both are at least not elementary ~\cite{abs-1809-07115,Lazic13}
while their decidability status is still unknown~\cite{Lazic13}.
%			\alain{I removed a sentence later that repeats this one}
In branching vector addition systems with states (BVASS)
a state is a set of threads with associated markings.
A thread either fires a transition as in Petri nets or forks, transferring
a part of its marking to the new thread. For BVASS,
the reachability problem is also
\TOWER-hard~\cite{LazicS14}
and its decidability is still an open problem while the coverability
and the boundedness problems are  2-\EXPTIME-complete~\cite{jcss12-DJLL}.
%R. Mayr defined and studied Process Rewrite Systems (PRS) in~\cite{Mayr00} ;
%PRS strictly subsume Petri nets, PA-processes, and pushdown processes;
%no complexity bounds are known for termination and coverability.
The analysis of subclasses of Petri nets
with a stack is an active field of research~\cite{AtigG11,MavlankulovOTSZ18,DassowT09,Zetzsche15}.
However, for none of the above extensions, the coverability and termination problems
belong to \EXPSPACE.


\noindent
{\bf Recursive Petri nets (RPN).} This formalism has been introduced
to model distributed planning of multi-agent systems for which counters and recursivity were necessary for specifying resources
and delegation of subtasks~\cite{EFH-icmas96}.
Roughly speaking, a state of an RPN consists of a tree of \emph{threads}
where the local state of each thread is a marking.
Any thread fires an \emph{elementary}, \emph{abstract} or \emph{cut} transition. When the transition is elementary,
the firing updates its marking as in Petri nets; when it is abstract, this only consumes
the tokens specified by the input arcs of the transition
and creates a child thread initialized with the \emph{initial marking} of
the transition. When a cut transition is fired,
the thread and its subtree are pruned, producing in its parent
the tokens specified by the output arcs of the abstract transition that created it.
In RPN, reachability, boundedness and termination
are decidable~\cite{HP-icatpn99,haddad:hal-01573071}
by reducing these properties to reachability problems of Petri nets. So the corresponding algorithms are nonelementary.
LTL model checking is undecidable for RPN but becomes decidable for the subclass of sequential RPN~\cite{HaddadP01}.
In~\cite{HaddadP07}, several modeling features are proposed while preserving the decidability of
the verification problems.



%\alain{harmoniser les notations de classes de complexités}

\noindent
{\bf Our contribution.}
We first study the expressive power of RPN from the point of view of coverability
languages (reachability languages were studied in \cite{HP-icatpn99}).
We first introduce a quasi-order on states of RPN compatible with the firing rule and establish that it is not a well quasi-order. Moreover, we show that there cannot exist a transition-preserving compatible well quasi-order, preventing us to use the framework of Well Structured Transition Systems
%	(with some natural transition-preserving compatible quasi-order)
to prove that coverability is decidable.
We show that the RPN languages
are \emph{quite close} to recursively enumerable languages since the closure under homomorphism and intersection with a regular language is the family of recursively enumerable languages.
More precisely, we show that  RPN coverability
(as reachability) languages strictly include the union of context-free languages
and Petri net coverability languages.
Moreover, we prove that  RPN coverability
languages and reachability languages of Petri nets
are incomparable. We prove that RPN coverability languages are a strict subclass of RPN reachability languages.
In addition, we establish that
the family of RPN languages is closed under union, homomorphism
but neither under intersection with a regular language nor under complementation.

% \alain{are we able to say something
% about the relations between RPN and VASS+1stack and BVASS ?}
From an algorithmic point of view, we show that, as for Petri nets, coverability, termination,
boundedness, and finiteness are
\EXPSPACE-complete. Thus the increase of expressive power does
not entail a corresponding increase in complexity.
In order to solve the coverability problem, we show that if there exists
a covering sequence there exists a `short' one
(i.e. with a length at most doubly exponential w.r.t. the size of the input).
%The core of the proof consists of turning an arbitrary covering sequence
%into a structured one where all threads perform their firings in one shot.
In order to solve the termination problem, we
	consider two cases for an infinite sequence
	depending (informally speaking) whether the depth of the trees
	corresponding to states are bounded or not along the sequence. For the unbounded case, we introduce the abstract graph that expresses the ability to create threads from some initial state.
The decidability of the finiteness and boundedness problems
are also mainly based on this abstract graph.

Let us mention that this paper is an extended version of \cite{FHK-atpn19} that contains new results about expressiveness like the characterization of the RPN coverability languages, decidability and complexity of finiteness and boundedness and we greatly simplified the proofs of coverability, termination, and finiteness. We also provided a more elegant definition of the (now inductive) syntax and the semantics of RPN.



\noindent
{\bf Outline.} In section~\ref{sec:recursive}, we introduce RPNs and
state ordering and establish basic results related to these notions.
In section~\ref{sec:reductions}, we introduce decision problems and some reductions between them.
In section~\ref{sec:expressiveness}, we study the expressiveness
of coverability languages. Then in
sections~\ref{sec:coverability},~\ref{sec:termination}, and~\ref{sec:finiteness}
we show that the coverability, termination, boundedness, and finiteness problems are \EXPSPACE-complete.
In section~\ref{sec:conclusion}, we conclude and give some perspectives to this work.



==> reach-cov.tex <==
% !TEX root =main.tex
The next propositions show that the family of coverability languages of an RPN
is a particular family of reachability languages of an RPN : the family of \emph{cut languages}.
A cut language of an RPN is a reachability language with a single final state $\emptyset$.

\begin{proposition}
\label{prop:reach-inc-cov}
The family of cut languages of RPNs
is included in the family of coverability languages of RPNs.
\end{proposition}
\begin{proof}
        Due to the correspondence between firing sequences of $(\N,s_0)$ and those of $(\rooted{\N},\sr)$,
        established in the previous section,
        one can assume w.l.o.g. that the initial markings of the RPNs have a single vertex.
Let $\mathcal L_R(\N,s[r,m_0],\{\emptyset\})$ be such a reachability language.\\
$\N'$ is obtained by adding places $todo$ and $done$
and a transition $start \in T'_{ab}$ with:\\ 
\centerline{$\lambda'(start)=\varepsilon$, $W'^-(start)=todo$, $W'^+(start)=done$,  $\Omega'(start)=m_0$.}\\
Then it is routine
to check that $\mathcal L_C(\N',s[r,todo],\{s[r,done]\})=\mathcal L_R(\N,s[r,m_0],\{\emptyset\})$.
\end{proof}

Establishing the converse inclusion is more intricate.

\begin{proposition}
\label{prop:cov-inc-reach}
The family of coverability languages of RPNs is included
in the family of cut languages of RPNs. 
\end{proposition}
\begin{proof}
        Due to the correspondence between firing sequences of $(\N,s_0)$ and those of $(\rooted{\N},\sr)$,
        established in the previous section,
        one can assume w.l.o.g. that the initial markings of the RPNs have a single vertex.
Let $\mathcal L_C(\N,s[r,m_0],S_f)$ be a coverability RPN language. 


\noindent {\bf Case $\emptyset \in S_f$.}
Observe that in this case we can reduce  $S_f$ to $\{\emptyset\}$.
Then  $\N'$ is obtained from $\N$ by adding a place $root$
and a cut transition $t_{root}$ with $\lambda'(t_{root})=\varepsilon$ and $W'^{-}(t_{root})=root$. It is routine
to check that the reachability language 
$\mathcal L_R(\N',s[r,m_0+root],\{\emptyset\})=\mathcal L_C(\N,s[r,m_0],\{\emptyset\})$.

\smallskip
\noindent {\bf Case $\emptyset \notin S_f$.}
Consider the net $\N^*$ obtained from $\N$ by adding two places $start$ and $run$
with  $m^*_0=start$, transitions $t_{run}\in T_{el}$
and $t_{start}\in T_{ab}$ with $\lambda^*(t_{run})=\lambda^*(t_{start})=\varepsilon$ and:\\
$W^{*-}(t_{run})=run$, $W^{*+}(t_{run})=2run$,\\
$W^{*-}(t_{start})=start$, $W^{*+}(t_{start})={\bf 0}$ and $\Omega^*(t_{start})=m_0+run$.
\begin{itemize}[nosep]
%
  \item For all $t\in T_{el}$, 
           $W^{*-}(t)=W^{*-}(t)+run$ and $W^{*+}(t)=W^{+}(t)$;
%
  \item For all $t\in T_{ab}$,  $\Omega^*(t)=\Omega(t)+run$, 
           $W^{*-}(t)=W^{-}(t)+run$ and $W^{*+}(t)=W^{+}(t)+run$;
%
  \item For all $t\in T_{\tau}$,  $W^{*-}(t)=W^{-}(t)+run$.
\end{itemize}
Let $S^*_f$ be $S_f$ where all markings are increased by $run$.\\
Then it is routine
to check that: 
$\mathcal L_C(\N^*,s[r,m^*_0],S^*_f)=\mathcal L_C(\N,s[r,m_0],S_f)$.\\ 
Furthermore (1) the empty tree is not reachable in $(\N^*,s[r,m^*_0])$
and (2) for any coverability sequence $s[r,m^*_0] \xrightarrow{\sigma} s\succeq s_f \in S^*_f$,
$r$ does not belong to the image of the corresponding mapping $f$.
Thus in the rest of the proof
we assume that $(\N,s[r,m_0],S_f)$ fulfills these properties. 
We also assume
w.l.o.g. that all vertices in $S_f$ are distinct. We denote $V_f$ this set of vertices.

\smallskip
\noindent
Let $\N'$ obtained as follows.\\
One adds  places $todo,done,cut,\{p_v\mid v\in V_f\}, \{p_{u,v}\mid s \in S_f,u\xrightarrow{m_v}_s v\}$.
\begin{itemize}[nosep]
%
  \item For all $t\in T_{el}$, 
           $W'^{-}(t)=W^{-}(t)$ and $W'^{+}(t)=W^{+}(t)$;
%
  \item For all $t\in T_{ab}$,   
           $W'^{-}(t)=W^{-}(t)$, $W'^{+}(t)=W^{+}(t)$ and $\Omega'(t)=\Omega(t)+cut$;
%
  \item For all $t\in T_{\tau}$,  $W'^{-}(t)=W^{-}(t)+cut$.
%
\end{itemize}
For all $t \in T_{ab}$, one adds the following abstract transitions:
\begin{itemize}[nosep]
%
	\item one adds $t_{Br}\in T'_{ab}$ with $\lambda'(t_{Br})=\lambda(t)$ and\\
	$W'^-(t_{Br})=W^-(t)+todo$, $W'^+(t_{Br})=done$, $\Omega'(t_{Br})=\Omega(t)+todo$;
%
	\item For all $r_s$ with $s\in S_f$
	one adds  $t_{r_s}\in T'_{ab}$ with $\lambda'(t_{r_s})=\lambda(t)$ and\\
	$W'^-(t_{r_s})=W^-(t)+todo$, $W'^+(t_{r_s})=done$, $\Omega'(t_{r_s})=\Omega(t)+(|\{r_s\xrightarrow{m_w}_s w\}|+1)p_{r_s}$;
%
	\item For all $v \in V_s\setminus\{r_s\}$ with $s\in S_f$ and $u \xrightarrow{m_v}_s v$ such that $W^+(t)\geq m_v$,\\
	one adds  $t_{v}\in T'_{ab}$ with $\lambda'(t_{v})=\lambda(t)$ and\\
	$W'^-(t_{v})=W^-(t)+p_u$, $W'^+(t_{v})=p_{u,v}$, $\Omega(t_{v})=\Omega(t)+(|\{v\xrightarrow{m_w}_s w\}|+1)p_{v}$.
%
\end{itemize}
One adds the following cut transitions:
\begin{itemize}[nosep]
%
	\item One adds $\tau_{done}\in  T_{\tau}$ with $W'^{-}(\tau_{done})=done$ and $\lambda'(\tau_{done})=\varepsilon$.
%
	\item For all $v \in V_s$ with $s\in S_f$
	one adds  $\tau_{v}\in T'_{\tau}$ with $\lambda'(\tau_{v})=\varepsilon$ and\\
	$W'^-(\tau_{v})=M_s(v)+p_{v}+\sum_{v\xrightarrow{m_w}_s w}p_{v,w}$.
%
\end{itemize}
\noindent
Let us prove that
$\mathcal L_R(\N',s[r,m_0+todo],\{\emptyset\})=\mathcal L_C(\N,s[r,m_0],S_f)$.

\smallskip\noindent
$\bullet$ $\mathcal L_C(\N,s[r,m_0],S_f)\subseteq \mathcal  L_R(\N',s[r,m_0+todo],\{\emptyset\})$.
Consider in $\N$ a coverability sequence $s[r,m_0] \xrightarrow{\sigma} s\succeq s_f \in S_f$ with
$f$ the mapping from $V_{s_f}$ to $V_s$. Let $Br$ be the branch in $s$ from $r$ to $f(r_{s_f})$,
excluding $f(r_{s_f})$. 
We build a sequence $\sigma'$ as follows.
\begin{itemize}[nosep]
%
	\item Let $v \in Br\setminus\{r\}$ and $(u,t)$ be the firing in $\sigma$ that creates $v$.\\ 
	 Then we substitute $(u,t)$ by $(u,t_{Br})$;
%
	\item Let $(u,t)$ be the firing in $\sigma$ that creates $f(r_{s_f})$. 
	 Then we substitute $(u,t)$ by $(u,t_{r_{s_f}})$;
%
	\item Let $v \in V_{s_f}\setminus \{r_{s_f}\}$ and  $(u,t)$ be the firing in $\sigma$ that creates $f(v)$.\\
	Then we substitute $(u,t)$ by $(u,t_{r_{s_f}})$. 
%
\end{itemize}
Then $\sigma'$ is a firing sequence of $(\N',s[r,m_0+todo])$ that leads to $s'$ with the
same tree structure (and vertices) as the one of $s$ and where the markings labelling $s'$
are defined as follows.
\begin{itemize}[nosep]
%
	\item For all $v \in V_{s'}\setminus (Br\cup f(V_{s_f}))$, $M_{s'}(v)=M_{s}(v)+cut$,\\
	and all $u\xrightarrow{m'_v}_{s'} v$ and  $u\xrightarrow{m_v}_{s} v$, one has $m'_v=m_v$;
%
	\item  For all $v \in Br$, $M_{s'}(v)=M_{s}(v)$. For all $v\xrightarrow{m'_w}_{s'} w$ with $w \in Br \cup \{f(r_{s_f})\}$,
	$m'_w=done$;
%
	\item For all $v \in V_{s_f}$, $M_{s'}(f(v))=M_{s}(f(v))+p_v$.
	For all $f(v)\xrightarrow{m'_w}_{s'} f(w)$,
	$m'_w=p_{v,w}$.
%
\end{itemize}
Observe that $\lambda(\sigma')=\lambda(\sigma)$. Then one completes $\sigma'$ by
firing $\{(f(v),\tau_v)\}_{v\in V_{s_f}}$ bottom up followed by firing $\{(v,\tau_{done})\}_{v\in Br}$ bottom up
leading to $\emptyset$. 

\smallskip\noindent
$\bullet$ $\mathcal L_R(\N',s[r,m_0+todo],\{\emptyset\})\subseteq \mathcal L_C(\N,s[r,m_0],S_f)$.
Observe that in $(\N',s[r,m_0+todo])$ the only way to reach $\emptyset$ is to fire $\tau_{done}$ since in $r$
(by induction) only abstract transitions of $T_{ab}$, $\{t_{Br}\mid t\in T_{ab}\}$ and
$\{t_{r_s}\mid t\in T_{ab} \wedge s\in S_f\}$ are fireable 
and places $cut$ and $\{p_v\}_{v\in V_f}$ are initially unmarked. Furthermore a single firing
$\{t_{Br}\mid t\in T_{ab}\}$ and
$\{t_{r_s}\mid t\in T_{ab} \wedge s\in S_f\}$ is at most possible in $r$ since
no transition can produce tokens for $todo$ in $r$.

\noindent
So consider in $\N'$ a firing sequence $s[r,m_0+todo] \xrightarrow{\sigma'} \emptyset$.
Due to the previous observation before the firing $(r,\tau_{done})$ ending $\sigma'$, there has been  in $\sigma'$ a firing
of $(r,t_{Br})$ or $(r,t_{r_s})$ for some $t\in T_{ab}$ and $s\in S_f$ creating a vertex $v_1$ followed by the firing of a cut transition in $v_1$. 
Since $\Omega'(t_{Br})=\Omega(t)+todo$, if  $v_1$ has been created by $(r,t_{Br})$ then the only cut transition that can be fired in $v_1$
is $\tau_{done}$. Since $\lambda'(\tau_{done})=\varepsilon$ and $W'^+(t_{Br})=done$, this firing can delayed in $\sigma'$ just before
the firing of $(r,\tau_{done})$.

\noindent
Furthermore there
must have been before this firing, the firing of  $(v_1,t_{Br})$ or $(v_2,t_{r_s})$ for some $t\in T_{ab}$ and $s\in S_f$ creating a vertex $v_2$ 
followed by the firing of a cut transition in $v_2$.
Since this iterated reasoning must  end, there must be some $v_k$ created by the firing of $(v_{k-1},t_{r_s})$ (with $v_0=r$)
for some $t\in T_{ab}$ and  $s\in S_f$. We denote by $f(r_s)$ the vertex $v_k$. 

\noindent
Since  $\Omega'(t_{r_s})=\Omega(t)+(|\{r_s\xrightarrow{m_w}_s w\}|+1)p_{r_s}$, the only  cut transition that can be fired in $f(r_s)$ is $\tau_{r_s}$. Since $\lambda'(\tau_{r_s})=\varepsilon$ and $W'^+(t_{r_s})=done$, this firing can delayed 
in $\sigma'$ just before the firing of $(v_{k-1},\tau_{done})$.
Furthermore  the firing of this cut transition must have been preceded for all $r_s\xrightarrow{m_w}_s w$
by the firing of some abstract transition $(v_k,t_w)$ creating a vertex denoted $f(w)$ followed by the firing
of a cut transition in $f(w)$. 

\noindent
Applying the same reasoning for $f(w)$ as the one for $f(r_s)$, one gets that 
the only  cut transition that can be fired in $f(w)$ is $\tau_{w}$ and that all the firings related to these $w$'s 
can be delayed before the firing  $(f(r_s),\tau_rs)$.

\noindent
Iterating this process, one obtains that $\sigma'$ can be reordered as $\sigma''\sigma_{\tau}$ with 
$\lambda'(\sigma'')=\lambda'(\sigma')$, and $\sigma_{\tau}$ is a sequence of 
cut transition firings with $\lambda(\sigma_\tau)=\varepsilon$. 

\noindent
Let $s''$ be the state of reached by $\sigma''$: it includes a branch created by the firings 
among $\{t_{Br}\}_{t\in T_{ab}}$ followed by a tree whose set vertices is $f(V_s)$ and every vertex $f(v)$ has
been created by the firing of some transition in $\{t_{v}\}_{t\in T_{ab}}$. Observe that due to our observations
on $(\N',s[r,m_0+todo])$ all other firings of $\sigma''$ are firings of transitions in $T$. By substituting
in $\sigma''$ all $t_{Br}$ by $t$ and all $t_{v}$ by $t$, one gets a firing sequence $\sigma$ of $(\N,s[r,m_0])$
with $\lambda(\sigma)=\lambda'(\sigma')$ that covers $s$.

\end{proof}



==> recursive-2.tex <==
% !TEX root =main.tex
\global\long\def\P{\mathbb{P}}
\global\long\def\R{\mathbb{R}}


\section{Recursive Petri Nets}
\label{sec:recursive}

\subsection{Presentation}


The state of an RPN has a structure akin to a `directed rooted tree' of Petri nets. Each vertex of the tree,
hereafter \emph{thread}, is an instance of the RPN and possessing some marking on it.
Each of these threads can fire \emph{three} types of transitions.
An \emph{elementary} transition updates its own marking according
to the usual Petri net firing rule.
An \emph{abstract} transition consumes tokens from the thread firing it
and creates a new child (thread) for it. The marking of the new thread is determined
according to the fired abstract transition.
A \emph{cut} transition can be fired by a thread
if its marking is greater or equal
than some marking.
Firing a cut transition, the thread erases itself and all of its descendants.
Moreover, it creates tokens in its parent,
which are specified by the abstract transition that created it.




\begin{definition}[Recursive Petri Net]
	\noindent A \emph{Recursive Petri Net} is a 6-tuple
	$\N=\langle P,T,W^{+},W^{-},\Omega\rangle$ where:
	\begin{itemize}
		%
		\item $P$ is a finite set of places;
		%
		\item $T=T_{el}\uplus T_{ab} \uplus T_{\tau}$ is a finite set of transitions with $P\cap T=\emptyset$,
		and $T_{el}$ (respectively $T_{ab}, T_{\tau}$) is the subset of elementary (respectively abstract, cut) transitions;
		%
		\item $W^{-}$ is the $\nat^{P\times T}$ backward incidence matrix;
		%
		\item $W^{+}$ are the $\nat^{P\times (T_{el}\uplus T_{ab})}$ forward incidence matrix;
		%
		\item $\Omega : T_{ab} \rightarrow \nat^P$ is a function that labels every abstract transition with a initial marking;
		%
	\end{itemize}
\end{definition}
Figure~\ref{fig:rpn_example} graphically describes an example of an RPN  with:
\begin{align*}
	&P=\{p_{ini},p_{fin},p_{beg},p_{end}\}\cup\{p_{b_i},p_{a_i}:i\leq 2 \}; \\
	&T_{el}=\{t_{b_1},t_{b_3},t_{a_1},t_{a_3},t_{sa},t_{sb}\}\,;\,T_{ab}=\{t_{beg},t_{b_2},t_{a_2}\};\\
	&T_{\tau}=\{t_{\tau_1},t_{\tau_2}\}.
\end{align*}
and for instance $ W^-(p_{ini},t_{beg})=1 $ and $ \Omega(t_{b_2})= p_{beg} $ (where  $ p_{beg} $ denotes the marking with one token in place $ p_{beg} $ and zero elsewhere).

For brevity reasons, we denote by $W^+(t)$ a vector in $\nat^P$,
where for all $p\in P$, $W^+(t)(p)=W^+(p,t)$, and we do the same for $W^-(t)$.

\begin{figure}[h]
	\begin{center}
		\input{rpn_example}
	\end{center}
	\caption{An example of a marked RPN.}
	\label{fig:rpn_example}
\end{figure}


A \emph{concrete state} $s$ of an RPN is a labeled
tree representing relations between threads and their associated markings.
Every vertex of $s$ is a thread and edges are labeled by abstract transitions. 
We introduce a countable set $\mathcal V$ of vertices in order to pick new vertices when necessary. 

\begin{definition}[State of an RPN]
	A \emph{concrete state (in short, a state)} $s$ of an RPN is a tree over the finite set of vertices $V_s\subseteq \mathcal V$, inductively defined as follows:
	\begin{itemize}
		%
		\item either $V_s=\emptyset$ and thus $s=\emptyset$ is the empty tree;
		%
		\item or $V_s=\{r_s\}\uplus V_1\uplus \ldots \uplus V_k$ with $0\leq k$ and
		$s=(r_s,m_0,\{(m_i,s_i)\}_{1\leq i\leq k})$ is defined as follows:
		\begin{itemize}
			%
			\item $r_s$ is the root of $s$ labelled by a marking $m_{0} \in \nat^P$;
			%
			\item For all $i\leq k$, $s_i$ is a state over $V_i\neq \emptyset$
			
			and there is an edge $r_s\xrightarrow{m_i}_s r_{s_i}$ with $m_i\in \{W^+(t)\}_{t\in T_{ab}}$.
		\end{itemize}
	\end{itemize}
\end{definition}
For all $u,v\in V_s$, one denotes $M_s(u)$ the marking labelling $u$
and when $u\xrightarrow{m}_s v$, one writes $\Lambda(u,v):=m$. 
State $s_v$ is the (maximal) subtree of $s$ rooted in $v$.
%

While the set of vertices $V_s$ will be important for analyzing the behavior of a firing sequence in an RPN, one can omit it and get a more abstract representation of the state. Note that contrary to the previous definition where $ \{(m_i,s_i)\}_{1\leq i\leq k} $ was a set, in the following definition we need a multiset $Child_s$.

\begin{definition}[Abstract state of an RPN]
	An \emph{abstract state} $s$ of an RPN is inductively defined as follows:
	\begin{itemize}
		%
		\item either $s=\emptyset$ is the empty set ;
		%
		\item or $s=(m_s,Child_s)$ where $m_s \in \nat^P$ 
		and $Child_s$ is a finite multiset of pairs $(m',s')$
		
		where $m'\in \{W^+(t)\}_{t\in T_{ab}}$ and $s'$ is an abstract state different from $\emptyset$.
		%
	\end{itemize}
	
\end{definition}
Given a concrete state $s$, we denote by $\abst{s}$ its abstract state.
Except if explicitly stated, a state is a concrete state.%	\igor{from concrete to abstract states}

In the other direction, given an abstract state $s$, one recovers its set of concrete states by 
picking an arbitrary set of vertices $V_s\subseteq \mathcal V$ of appropriate cardinality and, inductively, arbitrarily splitting $V_s$ between the root and the pairs $(m,s')$.

%\begin{definition}[ State of an RPN]
% A state $s=\left\langle V,M,E,\Lambda \right\rangle $ of an RPN
% $\N=\left<P,T,W^+,W^-,\Omega,\mathcal{F}\right>$
% is a  $4$-tuple where:
%\begin{itemize}
%%
%  \item $V$ is a finite set of vertices;
%%
%  \item $M: V\rightarrow\nat^{P}$ is a function that labels vertices with markings;
%%
%  \item $E\subseteq V\times V$ is a set of edges such that $(V,E)$ is a $T_{ab}$-labeled directed tree;
%%
%  \item $\Lambda : E \rightarrow T_{ab}$ is a function that labels edges with abstract transitions.
%\end{itemize}
%
%
%
%In the following,
%we denote by: $ V_s:=V $, $ M_s:=M $, $ E_s:=E $ and $ \Lambda_s:=\Lambda $.
%
%
%
%
%
%\end{definition}
%A state $s$ can be viewed as labelled tree (empty if $s=\emptyset$) inductively defined 
%for $s=(m_s,Child_s)$ as follows. The root is labelled by $m_s$ and there
%is one child per $(m',s')\in Child_s$ whose edge from the root is labelled by $m'$ and whose subtree
%is the one associated with $s'$. The vertices of this tree are called \emph{threads}. In the sequel,
% we associate with a thread  the state corresponding to its subtree.

For example, on the right side of Figure~\ref{fig:rpn_example},
there is a  (concrete) state of the RPN $ \N$. This state consists of three threads with markings
$ \bf 0,0,$ and $p_{end}$ (where $\bf 0 $ is the \emph{null marking})
and two edges with the labels $ W^+(t_{beg})$ and $W^+(t_{b_2}) $.
%Since a state consists of a directed tree, 
%it has a \emph{root thread }denoted by $r_s$ or when the context is clear
%more concisely $r$.

Let $ s $ be a state of some RPN.
Every thread $u$ different from the root has an unique \emph{parent}, denoted by $prd(u)$.
%We call the vertices $v$ for which there exists $(u,v)\in E$ a \emph{child} of $u$.
The \emph{descendants} of a thread $u$ consists of threads
in the subtree rooted in $u$ including $u$ itself.
We denote this set by $Des_{s}(u)$.
%Similarly the \emph{ancestors} of $u$ are the threads for
%which $u$ is a descendant of, i.e. $Asc_s(u)=\{v\mid u\in Des_s(v)\}$.
%For any two vertices $u,v$ in the same tree, denote by $dist(u,v)$ 
%the length of the elementary undirected path from one to the other, and 
%for a set of vertices $W$, let us denote $dist(u,W)=\min\{dist(u,w)\mid w\in W \}$.
For $m\in \nat^P$,
denote by $s[r,m]:=(r,m,\emptyset)$, the state consisting of a single vertex $r$ whose
marking is $m$.
As usual, two markings $m,m'\in \nat^P$, over a set of places $P$,
are partially ordered as follows:
$m\leq m'$ if for all places $p\in P$, $m(p) \leq m'(p)$.

\begin{definition}[Operational semantics]
	Let $s=(r,m_0,\{(m_i,s_i)\}_{1\leq i\leq k})$ be a state. 
	Then the firing rule $s\xrightarrow{(v,t)}s'$ where $v\in V_s $ and $t\in T$ is inductively defined as follows:
	\begin{itemize}
		%
		\item Let $t\in T_{el}$ such that $W^-(t)\leq m_0$, then one has $s\xrightarrow{r,t} (r,m_0-W^-(t)+W^+(t), \{(m_i,s_i)\}_{i\leq k})$
		%
		\item Let $t\in T_{ab}$ such that $W^-(t)\leq m_0$, then one has $s\xrightarrow{r,t} (r,m_0-W^-(t), \{(m_i,s_i)\}_{i\leq k+1}))$
		
		where $m_{k+1}=W^+(t)$, $s_{k+1}=s[v,\Omega(t)]$ with $v\in \mathcal V \setminus V_s$
		%
		\item Let $t\in T_{\tau}$ such that $W^-(t)\leq m_0$, then one has $s\xrightarrow{r,t} \emptyset$
		%
		\item Let $i\leq k$ such that $s_i \xrightarrow{v,t} s'_i$  \\
		if $s'_i=\emptyset$ then $s \xrightarrow{v,t} (m_0+m_i,\{(m_j,s_j)\}_{1\leq j\neq i\leq k})$ 
		
		else     $s \xrightarrow{v,t} (m_0,\{m_j,s_j\}_{1\leq j\neq i\leq k}\cup \{m_i,s'_i\})$
	\end{itemize}
	
\end{definition}

%The RPN moves from one state to another
%by one of the threads firing an  elementary, abstract or cut transition.
%Let us present the first two kinds:
%
%\begin{definition}[operational semantics]
%Let $\N= \left<P,T,W^+,W^-,\Omega,\mathcal{F}\right>$ be an RPN, $s$ be a state with some thread $v$ and $t$
%be a transition (elementary or abstract). We say that $t  \in T$ is 
%\emph{fireable} by $v$ from $s=\left\langle V,M,E,\Lambda \right\rangle$ 
%if  $M(v)\geq W^-(t)$. When fireable, its firing leads to  
%$s'=\left\langle V',M',E',\Lambda' \right\rangle$, denoted $s\xrightarrow{(v,t)}s'$, 
%where $s'$ is defined below:
%\begin{itemize}
%	%
%	\item If $t \in T_{el}$ then $s'=\left\langle V,M',E,\Lambda \right\rangle $
%	where $M'(u)=M(u)$ for all $u \in V\setminus\{v\}$\\and $M'(v)=M(v)-W^-(t)+W^+(t)$;
%	%
%	\item If $t \in T_{ab}$ then:
%	\begin{itemize}[nosep]
%		%
%		\item $V'=V\cup \{w\}$ where $w$ is a fresh identifier ($w \not\in V$);
%		%
%		\item $M'(u)=M(u)$ for all $u \in V\setminus\{v\}$, $M'(v)=M(v)-W^-(t)$ and $M'(w)=\Omega(t)$;
%		%
%		\item $E'=E\cup\{(v,w)\}$;
%		%
%		\item $\Lambda'(e)=\Lambda(e)$ for all $e \in E$ and $\Lambda((v,w))=t$.
%		%
%	\end{itemize}
%	%
%\end{itemize}

%\end{definition}
Figure \ref{fig:firing_example} illustrates a sequence of  transition
firings in the RPN described by Figure~\ref{fig:rpn_example}. The first transition $t_{beg}\in T_{ab}$ is fired  by the root.
Its firing results in a state for which the root has a new child (denoted by $ v $)
and a new outgoing edge with  label $ p_{fin} $.
The marking of the root is decreased to ${\bf 0}$
and $v$ is initially marked by $ \Omega(t_{beg})=p_{beg} $.
The second firing is due to an elementary transition
$t_{b_1}\in T_{el}$ which is fired by $v$.
Its firing results in a state for which the marking of $v$ is changed to
$M_s'(v)=M_s(v)+W^+(t_{b_1})-W^-(t_{b_1})=p_{b_1}$.
The fifth transition
to be fired  is the cut transition $t_{\tau_2}$, fired by the thread
with the marking $p_{end}$ (denoted by $w$).
Its firing results in a state where the thread $ w $ is erased,
and the marking of its parent is increased by $ W^+(t_{b_2})=p_{b_2}$.

\begin{figure}[h]
	
	\begin{center}
		\input{firing_sequance}
	\end{center}
	\caption{Firing sequence for the RPN in Figure \ref{fig:rpn_example}}
	\label{fig:firing_example}
\end{figure}


%We now introduce the last type of transition: \emph{cut transition}.
%In order to do so, we define \emph{pruning} operations.
%Given a state $s=\left\langle V,M,E,\Lambda \right\rangle$
%\igor{maybe move to sec 5-6?}
%Let $s=(r,m_0,\{(m_i,s_i)\}_{1\leq i\leq k})$ be a state and  $v\in V_s$. Then
%$s\backslash v $ is inductively defined by: \\
%if $v=r$ then $s\backslash v =\emptyset$ \\ else \\
% if $v\in V_{s_i}$ and $s_i\backslash v =\emptyset$ then $s\backslash v =(r,m_0+m_i,\{(m_j,s_j)\}_{1\leq j\neq i\leq k})$ \\
%else $s\backslash v =(r,m_0,\{(m_j,s_j)\}_{1\leq j\neq i\leq k}\cup (m_i, s_i\backslash v =\emptyset)$.\\
%Let $U\subseteq V_s\setminus \{r\}$ be a set closed by the descendant relation
%and $R = \{v\in U\mid prd(u) \notin U \}$
%be the set of \emph{roots} of $U$. Denote $R=\{u_1,\ldots,u_k\}$.
%Then $s\backslash U=s\backslash u_1\backslash u_2\backslash\ldots \backslash u_k$.
%It should be clear that the enumeration order of $R$ is irrelevant.
%This extended pruning will be used for solving the termination
%and finiteness problems.

%\begin{definition}[$\tau$ cut transition]
%Let $\N=\left<P,T,W^+,W^-,\Omega,\mathcal{F}\right>$ be an RPN, $s=\left\langle V,M,E,\Lambda \right\rangle$ be a state of $\mathcal N$ and $v\in V$.
%$\tau$ is \emph{fireable} by $v$ from $s$ if
%there exists $m\in \mathcal{F}$
%such that $M(v)\geq m$. When fireable, its firing
%leads to $s\backslash v$ and is denoted by $s\xrightarrow{(v,\tau)}s\backslash v$.
%\end{definition}
%For example, in Figure \ref{fig:firing_example} 


\smallskip
A \emph{firing sequence} is a sequence of transition firings, written
in a detailed way:
$s_0\xrightarrow{(v_1,t_1)}s_1\xrightarrow{(v_2,t_2)}\cdots\xrightarrow{(v_n,t_n)}s_n$,
or when the context allows it, in a more concise way like $s_0\xrightarrow{\sigma} s_n$ for
$\sigma=(v_1,t_1)(v_2,t_2)\dots(v_n,t_n)$.
Let $\sigma \in T^*$ with $\sigma=t_1\ldots t_n$ and $v$ be a vertex, $(v,\sigma)$
is an abbreviation for $(v,t_1)\ldots(v,t_n)$.
When we deal with several nets, we indicate by a subscript in which net, say $\N$,
the firing sequence takes place: $s_0\xrightarrow{\sigma}_{\N} s_n$.
Infinite firing sequences are similarly defined.
In a firing sequence, a thread $v$ that has been deleted is \emph{never reused} (which is possible
since $\mathcal V$ is countable).
A thread is \emph{final} (respectively \emph{initial}) w.r.t.
$\sigma$ if it occurs in the final (respectively initial) state of $\sigma$.
We say that $v\in Des_{\sigma}(u) $ if there exists $ i\leq n $ such that $ v\in Des_{s_i}(u) $.
We call $\sigma'$ a \emph{subsequence} of $\sigma$,
denoted by $\sigma'\sqsubseteq \sigma$, if there exists $k$ indexes $ i_1, i_2 \dots i_k$ such that $ 1 \leq i_1<i_2<\dots i_k\leq n $ and
$\sigma'=(v_{i_1},t_{i_1})(v_{i_2},t_{i_2})\dots (v_{i_k},t_{i_k})$.

\begin{remark}
	In the sequel, when we write ``RPN $\N$'', we mean $\N=\left<P,T,W^+,W^-,\Omega\right>$, 
	unless we explicitly write differently. An RPN $\N$ equipped 
	with an initial state $s$ is a \emph{marked~RPN} and denoted $(\N,s)$. 
	Similarly a \emph{marked Petri net} $(\N,m)$ is a Petri net $\N$ 
	equipped with an initial marking $m$.
\end{remark}
For a marked RPN $(\N,s_0)$, let $Reach(\N,s_0)=\{\abst{s}\mid \exists\sigma\in T^* \text{ s.t. } s_0\xrightarrow{\sigma} s\}$ be its \emph{reachability set}, i.e. the set of all the reachable \emph{abstract} states.

\subsection{An order for Recursive Petri Nets}


We now define a quasi-order $\preceq $ on the states of an RPN.
Given two states $ s,s' $ of an RPN $\N$,
we  say that $ s $ is \emph{smaller or equal} than $ s' $, denoted by $s\preceq  s'$,
if there exists a subtree in $ s' $, which is isomorphic to $ s $,
where markings are greater or equal
on all vertices and edges.

\begin{definition}
	Let $s \neq \emptyset$ and $s'$ be states of an RPN $\N$.
	Then $ s\preceq  s'$ if there exists an injective mapping $f$ from $V_s$
	to $V_{s'}$ such that for all $v\in V_s$:
	\begin{enumerate}[nosep]
		%
		\item $M_{s}(v) \leq M_{s'}(f(v))$, and, 
		%
		\item for all $v\xrightarrow{m}_sw$, there exists an edge $f(v) \xrightarrow{m'}_{s'}f(w)$ with $m\leq m'$.
		%	
	\end{enumerate}
	In addition, $\emptyset \preceq s$ for all states $s$.
	
	\noindent When $f(r_s)$ is required to be $r_{s'}$, one denotes this relation $s\preceq_r  s'$
	with $\emptyset \preceq_r s$ if and only if $s=\emptyset$.
	
\end{definition}


%\begin{definition}
%	Let  $s=\left\langle V,M,E,\Lambda \right\rangle $
%	and  $s'=\left\langle V',M',E',\Lambda' \right\rangle $ be states of an RPN $\N$. 
%	Then $s\preceq  s'$ if  there exists an injective (total) function 
%	$f:V \rightarrow V'$ such that:
%	\begin{enumerate}
%		\item For any edge $(u,v)\in E$, we have $(f(u),f(v)) \in E'$;
%	%
%		\item For any edge $(u,v)\in E$, we have
%		$W^+(\Lambda(u,v))\leq W^+(\Lambda'(f(u),f(v)))$;
%	%
%		\item For any thread $v\in V$, we have $M(v)\leq M'(f(v))$.
%	%
%	\end{enumerate}
%	$s$ and $s'$ are equivalent, denoted $s\simeq s'$, if 
%        $s\preceq  s'$ and $s'\preceq  s$.
%\end{definition}
%Intuitively the previous definition basically says that if $ s\preceq s' $ then $ s $ is a sub-tree of $ s' $ where (1) the markings of threads in $ s $  are smaller than their respective markings in $ s' $ and (2) if we cut $ v $ and $ f(v) $ from their respective states then the order on the new states remains.


Figure~\ref{fig:order example} illustrates these quasi-orders.
\begin{figure}[h]
	
	\begin{center}
		\input{comparing_states}
	\end{center}
	\caption{We have that $s\preceq  s'$, but $s\not\preceq_r  s'$ because the marking of the root of $s'$ is too small.}
	\label{fig:order example}
\end{figure}

While this is irrelevant for the results presented here, let us mention
that checking whether $s\preceq s'$ can be done in polynomial time
by adapting a standard algorithm for the subtree problem
(see for instance~\cite{Stadel78}).

\begin{restatable}{lemma}{partialorder}
	%\begin{lemma}
	The relations $\preceq $ and $\preceq_r$ are quasi-orders.
	%\end{lemma}
\end{restatable}

\begin{proof}
	Let, $ s,s',s''$ be states of an RPN $ \N $ with $s=(r,m_0,\{(m_i,s_i)\}_{1\leq i\leq k})$,  
	$s'=(r',m'_0,\{(m'_i,s'_i)\}_{1\leq i\leq k'})$ and  $s''=(r'',m''_0,\{(m''_i,s''_i)\}_{1\leq i\leq k''})$. 
	Let us show that the relation $\preceq $ is a quasi-order.
	\begin{enumerate}
		%
		\item Reflexivity: the identity function $ Id$ on  $V_s$ insures that $s\preceq s$.
		%
		\item Transitivity: Given $ s\preceq s'\preceq s'' $, 
		there exist two injective functions  $f:V_s \rightarrow V_{s'}$ and  $f':V_{s'} \rightarrow V_{s''}$. 
		Let $ g: V_{s} \rightarrow V_{s''}$ be defined by $ g=f'\circ f $. Then $g$ is injective.
		For any edge $v\xrightarrow{m}_sw$, there exists an edge $f(v) \xrightarrow{m'}_{s'}f(w)$ with $m\leq m'$
		and there exists an edge $f'(f(v)) \xrightarrow{m''}_{s''}f'(f(w))$ with $m\leq m'\leq m''$.
		For all $v\in V_s$, one has
		$M_s(v)  \leq M_{s'}(f(v)) \leq M_{s''}(f'(f(v)))=M_{s''}(g(v)).$
		Therefore  $s \preceq s''$.	
	\end{enumerate}
	The proof for the relation $\preceq_r$ is similar.
\end{proof}
Consider the equivalence relation $\simeq:=\preceq \cap \preceq^{-1}$.
Given a set of states $A$, one denotes by $\bigslant{A}{\simeq}$ the quotient set
by the equivalence relation $\simeq$. Observe that $s \simeq s'$ if and only if their
abstract representations are equal and that $\simeq=\preceq_r \cap \preceq^{-1}_r$.

%Even when omitting the identifier of vertices, this quasi-order is not a partial order
%since there could be abstract transitions $t\neq t'$ with $W^+(t)=W^+(t')$.

A quasi-order $\leq$ on the states of an RPN
is \emph{strongly compatible} (as in \cite{Alain01}) if for all states $s,s'$ such that $s\leq s'$
and for all transition firings  $s\xrightarrow{(v,t)}s_1$, there exist a state  $s'_1$ and a transition firing
$s'\xrightarrow{(v',t')}s'_1$ with $s_1 \leq s'_1$.
\begin{restatable}{lemma}{strongcompatibility}
	%\begin{lemma}
	\label{lem:strongcompatibility}
	The quasi-orders $\preceq $ and  $\preceq_r$ are strongly compatible.
	%\end{lemma}
\end{restatable}
\begin{proof}
	Let $s\preceq s'$ and let $f$ be the mapping associated with the relation $\preceq$ and $s\xrightarrow{v,t}s_1$.\\ 
	Thus $s_v\xrightarrow{v,t}s_2$ for some $s_2$.\\
	We will exhibit some $s'_1$ such that $s_1\preceq s'_1$ with some $f'$ as associated mapping.\\
	Since $M_s(v) \leq M_{s'}(f(v))$, one has $s'_{f(v)}\xrightarrow{f(v),t}s'_2$ for some $s'_2$ and by induction $s'\xrightarrow{f(v),t}s'_1$
	for some $s'_1$.\\
	It remains to define $f'$.
	\begin{itemize}[nosep]
		%
		\item If $t \in T_{el}$ then $f'=f$; 
		%
		\item If $t \in T_{ab}$ then for all threads $u$ of $s$, $f'(u)=f(u)$  and if $v^*$ (resp. $w^*$)
		is the thread created by the firing $(v,t)$ (resp. $(f(v),t)$) then $f(v^*)=w^*$;
		%
		\item If $t \in T_{\tau}$ then $f'$ is equal to $f$ restricted to the remaining vertices.
		%	
	\end{itemize}
	It is routine to check that the inequalities between corresponding markings of $s$ and $s'$ are fulfilled.
	The proof for $\preceq_r$ is similar.
	
\end{proof}
%\begin{proof}
%	Let us prove that for any two states $s\preceq q$ and an elementary step $s\xrightarrow{(v,t)}s'$, the elementary step $(f(v),t)$ is also fireable from $q$ and we have $q\xrightarrow{(f(v),t)}q'$ with $s' \preceq q'$.We consider three cases according to the type of the elementary transition $t$ in $(v,t)$.
%	\begin{enumerate}[nosep]
%		\item  $ t\in T_{el} $. First, $(f(v),t)$ is fireable from $q$ since:
%		\[
%		M_q(f(v))\geq M_s(v)\geq W^{-}(t).
%		\]
%		Now since the set of threads and the edges didn't change we let $f'=f$,
%		and get the clauses 1 and 2 from the definition of $\preceq$ hold. The only change in $s'$ and $q'$ is the marking of the vertex $v$ and $f(v)$ respectably. Therefore its enough to show that $M_{q'}(f(v))\geq M_{s'}(v)$. But this is true since:
%		\[
%		M_{q'}(f'(v))=M_q(f(v))+W^{+}(t)-W^{-}(t)\geq M_s(v)+W^{+}(t)-W^{-}(t)=M_{s'}(v).
%		\]
%		Therefore clause 3 also holds and hence we get that $s'\preceq q'$.\\
%		%
%		\item $ t\in T_{ab} $. The step $(f(v),t)$ is fireable from $q$ for the same reason as for the previous step. Since it was an abstract transition, there is a new vertex in $V_{s'}$ and in $V_{q'}$, denote it by $u_{s'}$ and $u_{q'}$ respectively. Let $f':V_{s'}\rightarrow V_{q'}$  be the function:
%		\[
%		f'(v):=\begin{cases}
%		f(v) & v\in V_s\\
%		u_{q'} & v=u_{s'}
%		\end{cases}.
%		\]
%		The changes in $s'$ and $q'$ are in the marking of the threads $v$ and $f(v)$, the new threads $u_{s'},u_{q'}$ and their respective edges $\left(v,u_{s'}\right)$ and $(f(v),u_{q'})$. Hence it is enough to show that $f'$ 'respects' theses changes i.e. :
%		\begin{enumerate}[nosep]
%			\item For the marking of the thread $v$, we have:
%			\[
%			M_{q'}(f'(v)) = M_q(f(v))-W^{-}(t)\geq M_s(v)-W^{-}(t)=M_{s'}(v).
%			\]
%			%
%			\item For the marking of the thread $u_{s'}$ we have
%			\[
%			M_{s'}(u_{s'})=\Omega\left(t\right)=M_{q'}(u_{q'})=M_{q'}(f(u_{s'})).
%			\]
%			%
%			\item For the new edge $(v,u_{s})\in E_s'$ we have that
%			\[
%			(f'(v),f'(u_{s}))=(f(v),u_{q'})\in E_{q'}.
%			\]
%			Where its label in $q'$ is the same one as in $s'$ since they both were created by the same abstract transition $ t $.\\
%		\end{enumerate}
%		
%		Therefore clauses 1,2,3 from the definition of $\preceq$ hold and hence we get that $s'\preceq q'$.\\
%		%
%		\item The elementary step $(v,t)$ is a cutting step, i.e. $ t=\tau $. Same as in the first two cases $(f(v),\tau)$ is fireable from $q$. Since $t$ is a cutting step, the changes in $s'$ and $q'$ are the following: we remove all the threads in $Des_s(v)$ and $Des_q(f(v))$ respectively, and change the marking of the threads $pred_s(v)$ and $pred_q(f(v))$. Denote by $f':V_{s'}\rightarrow V_{q'}$ the function $f'(v):=f(v).$ We first note that $pred_q(f(v))=f(pred_s(v))$ because there is only
%		one father for each thread and by clause 1 of the definition of $\preceq$ we have that $(pred_s(v),v)\in E_s$ if and only if $(f(pred_s(v)),f(v))\in E_q$.
%		Since we only have less edges in $s'$ and since we take a projection of $f$ we get clauses 1 and 2 immediately. The marking on $pred_s(v)$ has:
%		\begin{align*}
%		M_{q'}(pred(f'(v))) & =M_q(pred(f(v)))+W^{+}(\Lambda_q(f(pred(v),f(v)))\geq\\
%		& \geq M_s(pred(v))+W^{+}(\Lambda_s(pred(v),v))=M_{s'}(pred(v)).
%		\end{align*}
%		Therefore clause 3 also holds and hence we get that $s'\preceq q'$.
%	\end{enumerate}
%\end{proof}

%\alain{say that the other orders (ex Kruskal order on trees) are not adaptated...}
These quasi-orders may contain an infinite set of
incomparable states (i.e. an infinite \emph{antichain}).
For example, see Figure~\ref{fig:antichain} where any two states $s_i$ and $s_j$ are incomparable.
\begin{figure}[h]
	\begin{center}
		\input{anitchain}
	\end{center}
	\caption{An RPN with an antichain of states}
	\label{fig:antichain}
\end{figure}
Indeed, for any $ i<j $: (1)  $  s_j\not\preceq s_i$
since $ |V_{s_j}|>|V_{s_{i}}| $ there cannot be any injective function from $ V_{s_j}$ to $ V_{s_{i}} $, and (2) $ s_i\not\preceq s_j$
since for any injective function from $ V_{s_i}$ to $ V_{s_{j}} $,
at least one of the edges with the marking $ p_r $ would be mapped to an edge with a marking $p_\ell$.
Since $s\preceq_r s'$ implies $s\preceq s'$, this is also an antichain for $\preceq_r$.

Observe also that these quasi-orders are not only strongly compatible. They are \emph{transition-preserving compatible}
meaning that  for all states $s,s'$ such that $s\leq s'$
and for all transition firings  $s\xrightarrow{(v,t)}s_1$, there exist $s'_1$ and a transition firing
$s'\xrightarrow{(v',t)}s'_1$ with $s_1 \leq s'_1$. In Petri net, the standard order on $\nat^P$ is
a well quasi-order which is transition-preserving compatible. The next proposition establishes
that such a quasi-order does not exist in RPN. 

\begin{proposition} There does not exist a well quasi-order on states of RPN
	which is transition-preserving compatible.
\end{proposition}
\begin{proof}
	Consider the net of Figure~\ref{fig:antichain} and the family of states $\{s_n\}_{n\geq 1}$.
	By a simple examination one gets that for all $n\geq 1$, 
	$s_n\xrightarrow{(v_{n+1},\tau_{\ell})\ldots (v_{1},\tau_{\ell})(v_{0},\tau_{r})} \emptyset$.
	Moreover for all $n'\neq n$, there does not exist a firing sequence from $s_{n'}$ labelled
	by $\tau_{\ell}^{n+1}\tau_{r}$. Thus for any transition-preserving compatible quasi-order $\leq$,
	these states are incomparable establishing that $\leq$ is not a well quasi-order.
	
\end{proof}

Since $\preceq$ is not a well quasi-order, RPNs with the relation $\preceq$  are not well structured transition 
systems (WSTS)~\cite{Alain01} for which coverability is decidable. %	and it is often solved in exponential space. 
Therefore to solve coverability, one needs to find another way. 




==> reductions.tex <==
% !TEX root =main.tex
\section{Decision problems and reductions}
\label{sec:reductions}
In this section, we introduce the decision problems that we are going to solve and establish reductions to simpler problems in order to shorten the proofs of subsequent sections. 

Let $(\N,s_0)$ be a marked RPN and $s_f$ be a state of $\N$.
\begin{itemize}
	%
	\item The \emph{cut problem} asks whether there exists a firing sequence $\sigma$ such that $s_0\xrightarrow{\sigma}\emptyset$?
	%
	\item The \emph{coverability problem} asks whether there exists a firing sequence $\sigma$ such that $s_0\xrightarrow{\sigma}s\succeq s_f$?
	%
	\item The \emph{termination problem} asks whether there exists an infinite firing sequence?
	%
	\item The \emph{finiteness problem} asks whether $Reach(\N,s_0)$ is finite?
	%
	\item The \emph{boundedness problem} asks whether there exists $B\in \nat$ such that for all $s\in Reach(\N,s_0)$ 
	and for all $v\in V_s$, one has $\max(M_s(v)(p))_{p\in P} \leq B$?
	%
\end{itemize} 
Observe that contrary to Petri nets, the finiteness and boundedness problems are different and not equivalent.
Indeed, an RPN can be bounded while due to the unbounded number of vertices, its reachability set can be infinite. 

We introduce the ``rooted'' version of the above problems: for these versions, $s_0$ is required to be some $s[r,m_0]$.
In order to establish a reduction from the general problems to their rooted versions, 
given a marked RPN $(\N,s_0)$, we build a marked RPN $(\rooted{\N},s[r,\rooted{m_0}])$ that in a way simulates 
the former marked RPN.
We do this by adding a place $p_v$ for every vertex $v\neq r$ of $s_0$ 
and we add an abstract transition $t_v$ that consumes a token from this place and creates a new vertex with initial marking in $M_{s_0}(v)+\sum_{v\xrightarrow{m_{v'}}_{s_0} v'}$. This will allow to create the children of $v$ in $s_0$ (see Figure \ref{fig:RPN_to_rooted_rpn}). 
In order to similarly proceed in the root, $\rooted{m_0}=M_{s_0}(r)+\sum_{r\xrightarrow{m_{v'}}_{s_0} v'}$.

\begin{definition}
	Let $(\N,s_0)$ be a marked RPN. Then $(\rooted{\N},\sr)$ is defined by:
	\begin{itemize}[nosep]
		%
		\item $\rooted{P} = P \cup \{p_v \mid v\in V_{s_0}\setminus\{r_{s_0}\}\}$ ;
		%
		\item  $\rooted{T}_{ab}=T_{ab}\cup T_V$, $\rooted{T}_{\tau} = T_{\tau}$, 
		$\rooted{T}_{el}=T_{el}$ with $ T_V=\{t_v \mid v\in  V_s\setminus\{r_s\}\}$ ;
		%
		\item for all $t\in T$,	one has $\rooted{W}^-(t)=W^-(t)$ 
		and  all $t\in T_{ab}\cup T_{el}$, $\rooted{W}^+(t)=W^+(t)$ ;
		%
		\item for all $t_v\in T_V$ and $u\xrightarrow{m_v}_{s_0} v$, $\rooted{W}^-(t_v)=p_v$ and $\rooted{W}^+(t_v)=m_v$ ; 
		%
		\item for all $t\in T_{ab}$, $\rooted{\Omega}(t) = \Omega(t)$ ;
		%
		\item for all $t_v\in T_V$,  $\rooted{\Omega}(t_v)=M_{s_0}(v)+\sum_{v\xrightarrow{m_{v'}}_{s_0} v'} p_{v'}$ ;
		%
		\item $\sr = s[r,M_{s_0}(r_s)+\sum_{r_{s_0}\xrightarrow{m_v}_{s_0} v} p_{v}]$.
		%
	\end{itemize}
	
\end{definition}
\begin{figure}[h]
	\input{rooted_rpn}
	\caption{From a marked RPN to a rooted one}\label{fig:RPN_to_rooted_rpn}
\end{figure}

Let $m\in \nat^{\rooted{P}}$,  we denote by $m_{|_{P}}\in\nat^{P}$ the projection of $m$ on  $P$. 
Let $s$ be a state of  $\rooted{N}$,  we denote $s_{|_{P}}$ a state of $\N$ obtained by projecting  every marking of $s$ on $P$.

\smallskip
\noindent{\bf Observations.} 
\begin{enumerate}[nosep]
	%
	\item The encoding size of $(\N,s_0)$ is linear w.r.t. the encoding size of $(\rooted{\N},\rooted{s_0})$.
	%
	\item Let $e:=(v_i)_{0\leq i\leq k}$ be an enumeration of $V_{s_0}$ such that $v_0=r_{s_0}$
	and for all $0< i\leq k$, $prd(v_i)\in \{v_j\}_{j<i}$. Consider $\sigma^e_{s_0} = (prd(v_i),t_{v_i})_{i=1}^{k}$.
	Such an enumeration is called \emph{consistent}.
	By construction of $\rooted{\N}$, $\sr \xrightarrow{\sigma^e_{s_0}}_{\rooted{\N}} s'_0$ with $s'_{0|P}=s_0$
	and all places of $P_V$ unmarked in $s'_0$.
	%
	\item Let $\sr\xrightarrow{\sigma}_{\rooted{\N}}s$. Then by construction, for all $v\in V_{s_0} \setminus \{r_{s_0}\}$,  
	there is at most one occurrence of $t_v$ which furthermore is fired in $prd(v)$. Moreover since these firings consume
	tokens in $P_V$ that were not used for firings of $T$, they can be  pushed at the beginning of $\sigma$ (denoted by $\sigma_1$)
	and completed by the missing firings of $T_V$ in $\sigma$ (denoted by $\sigma_2$) getting a consistent enumeration $e$. 
	Summarizing, denoting $\sigma_{| \N}$, $\sigma$ without the firings of $T_V$,
	one gets that: \\
	(1)  $\sr\xrightarrow{\sigma_1\sigma_{| \N}}_{\rooted{\N}}s$,\\
	(2) $\sr\xrightarrow{\sigma\sigma_2}_{\rooted{\N}}s'$ and \\
	(3) $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$
	with $s'_{|P}=s''$ and all places of $P_V$ are unmarked in $s'$.
	%
	
\end{enumerate}
Due to observation~2, we immediately get that: 
\begin{lemma}
	\label{lemma:fromNtoroot}
	Let $(\N,s_0)$ be a marked RPN and $s_0\xrightarrow{\sigma}_{\N}s$. 
	Then  for every consistent enumeration $e$, there exists a firing sequence $\sr\xrightarrow{\sigma^e_{s_0}{\sigma}}_{\rooted{\N}}s'$ with ${s'}_{|_P} = s$
	and all places of $P_V$ are unmarked in $s'$.
\end{lemma}

%\begin{proof}
%	From the construction above we can fire first $\sr\xrightarrow{\sigma_{s_0}}s_1$ where ${s_1}_{|_P}=s_0$. Hence $\sigma$ is fireable from $s_1$, and $s_1\xrightarrow{\sigma}s'$ where $s'_{|_P}=s$.
%\end{proof}

Due to observation~3, we immediately get that: 
\begin{lemma}
	\label{lemma:fromroottoN}
	Let $(\N,s_0)$ be a marked RPN and $\sr\xrightarrow{\sigma}_{\rooted{\N}}s$. 
	Then there exist a consistent enumeration $e$ and a decomposition $\sigma^e_{s_0}=\sigma_1\sigma_2$
	such that $\rooted{s_0}\xrightarrow{\sigma_1\sigma_{| \N}}_{\rooted{\N}}s$, 
	$\sr\xrightarrow{\sigma\sigma_2}_{\rooted{\N}}s'$ and $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$
	with $s'_{|P}=s''$ and all places of $P_V$ are unmarked in $s'$.
\end{lemma}

Due to the previous lemmas, we get that: 
\begin{proposition}\label{col:rooted}
	The cut (resp. coverability, termination, finiteness, boundedness) problem 
	is polynomially reducible to the rooted cut (resp. coverability, termination, finiteness, boundedness)  problem.
\end{proposition}
\begin{proof}
	
	\noindent
	Let $(\N,s_0)$ be a marked RPN and $s_f$ be a state of $\N$. Define $\rooted{s}_f$ 
	a state of $\rooted{\N}$ be as $s_f$ with in all markings of $s_f$, all places of $\rooted{P} \setminus P$ unmarked. 
	
	\noindent
	$\bullet$ Assume that there exists  $s_0\xrightarrow{\sigma}_{\N}\emptyset$. Then by Lemma~\ref{lemma:fromNtoroot}, 
	$\sr\xrightarrow{\sigma^e_{s_0}{\sigma}}_{\rooted{\N}}\emptyset$. Assume that there exists
	$\sr\xrightarrow{\sigma}_{\rooted{\N}}\emptyset$ which means that the last transition is fired in the root
	and is a cut transition. Then by Lemma~\ref{lemma:fromroottoN}, $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$ for some $s''$. Since
	the last firing of  of $\sigma_{| \N}$ is the cut transition fired in the root $s''=\emptyset$.
	
	\noindent
	$\bullet$ Assume that there exists  $s_0\xrightarrow{\sigma}_{\N}s\succeq s_f$. Then by Lemma~\ref{lemma:fromNtoroot}, 
	$\sr\xrightarrow{\sigma^e_{s_0}{\sigma}}_{\rooted{\N}}\rooted{s}$ with $\rooted{s}_{|P}=s$. 
	Thus  $\rooted{s}\succeq \rooted{s}_f$. Assume that there exists
	$\sr\xrightarrow{\sigma}_{\rooted{\N}}s\succeq \rooted{s}_f$. 
	Then by Lemma~\ref{lemma:fromroottoN}, there exists $\sigma_2$ a firing sequence of $T_V$
	with  $\sr\xrightarrow{\sigma\sigma_2}_{\rooted{\N}}s'$,  $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$
	and $s'_{|P}=s''$. Since $\sigma_2$ only creates vertices and deletes tokens from $P_V$, 
	$s'\succeq \rooted{s}_f$. Thus $s'' \succeq s_f$.
	
	\noindent
	$\bullet$ Assume that there exists  $s_0\xrightarrow{\sigma}_{\N}$ with $\sigma$ infinite. Then by Lemma~\ref{lemma:fromNtoroot}, 
	$\sr\xrightarrow{\sigma^e_{s_0}{\sigma}}_{\rooted{\N}}$. Assume that there exists
	$\sr\xrightarrow{\sigma}_{\rooted{\N}}$ with $\sigma$ infinite. 
	Then by Lemma~\ref{lemma:fromroottoN}, $s_0 \xrightarrow{\sigma_{| \N}}_{\N}$ with $\sigma_{| \N}$ infinite
	since there are only a finite number of firings of $T_V$. 
	
	\noindent
	$\bullet$ Assume that $Reach(\N,s_0)$ is infinite. For all $s \in Reach(\N,s_0)$, define $\rooted{s}$ a state
	of $\rooted{\N}$  as $s$  with all places of $P_V$ in  markings of $s$ unmarked. Due to 
	Lemma~\ref{lemma:fromNtoroot}, $\rooted{s}\in Reach(\rooted{\N},\rooted{s_0})$. Since this mapping is injective,
	$Reach(\rooted{\N},\rooted{s_0})$ is infinite. Assume that $Reach(\rooted{\N},\rooted{s_0})$ is infinite. 
	Let $s \in Reach(\rooted{\N},\rooted{s_0})$. Due to  Lemma~\ref{lemma:fromroottoN},
	consider $s \xrightarrow{\sigma_2}_{\rooted{\N}}s'$ and $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$
	with $s'_{|P}=s''$ and all places of $P_V$ unmarked in $s'$. Thus $s''\in Reach(\N,s_0)$.
	The mapping from $s$ to $s''$ is not injective. However, the inverse image of $s''$ by this mapping is finite since there are a finite number of consistent enumerations and prefixes of such enumerations. Thus $Reach(\N,s_0)$ is infinite.
	
	\noindent
	$\bullet$ Assume that $(\N,s_0)$ is unbounded. For all $s \in Reach(\N,s_0)$, define $\rooted{s}$ a state
	of $\rooted{\N}$  as $s$  with all places of $P_V$ in  markings of $s$ unmarked. Due to 
	Lemma~\ref{lemma:fromNtoroot}, $\rooted{s}\in Reach(\rooted{\N},\rooted{s_0})$. 
	Thus $(\rooted{\N},\rooted{s_0})$ is unbounded. Assume that $(\rooted{\N},\rooted{s_0})$ is unbounded.
	By construction, the marking of places in $P_V$ is bounded. 
	Let $s \in Reach(\rooted{\N},\rooted{s_0})$. Due to  Lemma~\ref{lemma:fromroottoN},
	consider $s \xrightarrow{\sigma_2}_{\rooted{\N}}s'$ and $s_0 \xrightarrow{\sigma_{| \N}}_{\N}s''$
	with $s'_{|P}=s''$ and all places of  $P_V$ unmarked in $s'$. Thus $s''\in Reach(\N,s_0)$.
	Since for all vertex $v$ of $s$, $v$ is also present in $s''$ and for all $p\in P$,
	$M_s(v)(p)=M_{s''}(v)(p)$. Then $Reach(\N,s_0)$ is unbounded.
\end{proof}

%\begin{proof}
%	Lets us begin by showing that for any state $s'$ of $\N$ has that $s'\in Reach(\N,s_0)$ if and only if $\rooted{s}'\in Reach(\rooted{\N},\rooted{s_0})$ where $s' = \rooted{s'}|_P$.
%	
%	\noindent On one hand consider the firing sequence $s_0\xrightarrow{\sigma}s'$ in $\N$, 
%	we show that there exists a firing sequence $\rooted{s_0}\xrightarrow{\rooted{\sigma}} \rooted{s}\succeq s$ in $\rooted{\N}$.
%	One starts by firing all transitions of $T_s$ in a top-down way
%	to get a state $\rooted{s'_1}$ such that $s_0 =  \rooted{s'_1}|_P$. Let us denote by $\sigma_0$
%	this sequence and get that $ \rooted{s_0}\xrightarrow{\sigma_0} \rooted{s'_1} \xrightarrow{\sigma}\rooted{ s'} $ where $s' = \rooted{ s'} |_P$.\\
%	On the other hand, consider the firing sequence $\rooted{s_0}\xrightarrow{\rooted{\sigma}} \rooted{s}'$ in $\rooted{\N}$, 
%	we show that there exists a firing sequence  $s_0\xrightarrow{\sigma}s'$ in $\N$ with $s' = \rooted{ s'}|_P$ .
%	By construction of $\rooted{\N}$, all occurrences of transitions of $T_s$
%	can be pushed at the beginning of the sequence leading to a firing
%	sequence $\sigma'=\sigma_1\sigma_2$ where $\sigma_1$
%	consists of such occurrences. 	
%	Then $\sigma_1$ can be completed 
%	by the missing occurrences
%	still in a top-down way producing $\sigma'_1$ and 
%	yielding a coverability sequence $\sigma''=\sigma'_1\sigma_2$.
%	Firing $\sigma''$ we get $\rooted{s_0}\xrightarrow{\sigma_1'} \rooted{{s_1}}\xrightarrow{\sigma_2} \rooted{{s_2}}$ where $ \rooted{s_1}|_P = s_0  $  and $ \rooted{{s_2}}|_P = \rooted{{s}'}|_P $.	
%	Thus $s_0\xrightarrow{\sigma_2}s'$ in $\N$ where $s' = \rooted{{s}'}|_P$. 
%	
%	
%	\noindent From what we've shown the four equivalences are immediate.
%	
%	%	\igor{We show the proposition for coverability (i.e. 1.) the rest are equivalent}.
%	%	On one hand consider a coverability sequence $s_0\xrightarrow{\sigma}s'\succeq s$ in $\N$, 
%	%	we show that there exists a coverability sequence $\rooted{s_0}\xrightarrow{\rooted{\sigma}} \rooted{s}\succeq s$ in $\rooted{\N}$.
%	%	One starts to fire all transitions of $T_s$ in a top-down way
%	%	to get a state $s'_1$ such that (when omitting places $\{p_e\}$) 
%	%	both $s_0\simeq s'_1$ and
%	%	so that we identify the corresponding threads. Let us denote $\sigma_0$
%	%	this sequence. We get that $$ \rooted{s_0}\xrightarrow{\sigma_0} s_1 \xrightarrow{\sigma} s\succeq s $$
%	%	
%	%	On the other hand assume consider a coverability sequence $\rooted{s_0}\xrightarrow{\rooted{\sigma}} \rooted{s}\succeq s$ in $\rooted{\N}$, 
%	%	we show that there exists a coverability sequence  $s_0\xrightarrow{\sigma}s'\succeq s$ in $\N$.
%	%	By construction of $\rooted{\N}$, all  occurrences of transitions of $T_s$
%	%	can be pushed at the beginning of the sequence leading to a covering
%	%	sequence $\sigma'=\sigma_1\sigma_2$ where $\sigma_1$
%	%	consists of such occurrences. Then $\sigma_1$ can be completed 
%	%	by the missing occurrences
%	%	still in a top-down way producing $\sigma'_1$ and 
%	%	yielding a coverability sequence $\sigma''=\sigma'_1\sigma_2$.
%	%	Moreover the state $s_1$ (when omitting places $\{p_v\}$) reached from $\sigma'_1$
%	%	is equivalent to $s_0$. Thus $s_0\xrightarrow{\sigma_2}s'\succeq s$ in $\N$. 
%	%	
%\end{proof}

%\subsection{Well Ordered Sequences}
%Part of the richness of RPNs comes from their ability to create and later on destroy threads. Unfortunately, this is also adds to the difficulty of analyzing them. In this subsection we show how to get an omniscient sequence that knows from the start which threads it will not need to keep and hence does not create them.  
Let $\sigma$ be a firing sequence.
A thread is \emph{extremal} w.r.t.
$\sigma$ if it is an initial or final thread.

\begin{definition}
	Let $\N$ be an RPN. Then $T_{ret}\subseteq T_{ab}$, the set of \emph{returning transitions} is defined by:
	$$\{t\in T_{ab}\mid \exists s[r,\Omega(t)] \xrightarrow{\sigma}\emptyset\}$$
\end{definition}
For all $t\in T_{ret}$, we define $\sigma_{t}$ to be some arbitrary
shortest \emph{returning sequence} (i.e. $s[r,\Omega(t)] \xrightarrow{\sigma_t}\emptyset$).
We now introduce $\widehat{\N}$ obtained from $\N$ by adding elementary transitions that mimic
the behaviour of a returning sequence. Observe that the size of $\widehat{\N}$
is linear w.r.t. the size of $\N$.

\begin{definition} Let $\N$ be an RPN. Then
	$\widehat{\N}=\left<P,\widehat{T},\widehat{W}^+,
	\widehat{W}^-,\Omega\right>$ is defined by:
	\begin{itemize}[nosep]
		%
		\item $\widehat{T}_{ab}=T_{ab}$, $\widehat{T}_{\tau} = T_{\tau} $ , 
		$\widehat{T}_{el}=T_{el}\uplus \{t^r\mid t\in T_{ret} \}$; 
		%
		\item for all $t\in T$,	$\widehat{W}^-(t)=W^-(t)$ 
		and  all $t\in T_{ab}\cup T_{el}$, $\widehat{W}^+(t)=W^+(t)$;
		%
		\item for all $t\in T_{ab}$,	$\widehat{\Omega}(t)=\Omega(t)$; 
		%
		\item for all $t\in T_{ret}$,	$\widehat{W}^-(t^r)=W^-(t)$ 
		and  $\widehat{W}^+(t^r)=W^+(t)$.
		%
	\end{itemize}
Figure~\ref{fig:RPN_hat} has an example of an RPN $\N$ and its $\widehat{\N}$.
\end{definition}
\begin{figure}[h]
	\input{rpn_hat}
	\caption{From $\N$ to $\widehat{\N}$ and $\widehat{\N}_{el}$}\label{fig:RPN_hat}
\end{figure}

Note that since $\widehat{\N}$ enlarges $\N$ by adding transitions and that any firing of $t^r$ in $\widehat{\N}$ 
can be replaced by the firing of $t\sigma_t$ in $\N$ we get:
\begin{proposition}
	\label{prop:equivreach}
	Let $(\N,s_0)$ be a marked RPN. Then $Reach(\N,s_0)=Reach(\widehat{\N},s_0)$. 
\end{proposition}

%
%\begin{proof}
%	On one hand we know that $ Reach(\N,s_0) \subseteq Reach(\widehat{\N},s_0)$ since any fireable sequence in  $ {\N},s_0 $ is well defined and fireable in $ \widehat{\N},s_0 $ and reaches the same state.
%	On the other hand given a 
%\end{proof}

%The key ingredient of the existence of a short sequence is that
%in $\widehat{\N}$ every sequence can be turned into a \emph{\wellOrd}\
%sequence reaching the same state. Along such a sequence, (1) there
%are only extremal threads, (2) firings are performed in one shot
%by threads, and (3) only initial threads disappear
%and final threads perform firings of abstract transitions.

We call a firing sequence $\sigma$ \emph{omniscient} if any thread created during its firing is a final thread.

\begin{proposition}\label{prop:omniciant}
	Let $(\N,s_0)$ be a marked RPN and $s_0\xrightarrow{\sigma}_{\N}s$.
	Then there exists  a firing sequence $s_0\xrightarrow{\widehat{\sigma}}_{\widehat{\N}} s$ such that $\widehat{\sigma}$ is omniscient.  
\end{proposition}

\begin{proof}
	Assume that we have an extremal thread $u$ which fires $ t\in T_{ab} $ creating a non final thread $ v $ that disappears by a matching cut transition $ (v,t_\tau)\in \sigma $ for $t_\tau\in T_\tau$.
	One builds $\sigma'$ by (1) deleting from $\sigma $ the transition $ (u,t) $, (2) deleting all the firings from $ Des_{\sigma}(v) $ in $\sigma$ and (3) replacing the transition $ (v,t_\tau) $ by $(u,t^r)$. We claim that $s\xrightarrow{\sigma}s' $. Indeed
	in $u$ the transition $(u,t^r)$ has the same incidence in $u$
	as the transition  $(u,t)$ followed by $(v,t_\tau)$ (`anticipating' $(v,t_\tau)$ only add tokens in intermediate states)
	and the other deleted firings are performed by threads in $Des_{\sigma}(v) $ which do not exist anymore.
	By taking $\widehat\sigma$ the sequence obtained by iterating the process, we get the omniscient sequence.
\end{proof}
%\begin{definition}
%	Let $ \N $  be an RPN and
%	$\sigma$ be a firing sequence. Then $\sigma$ is \emph{\wellOrd}\ if $\sigma=\sigma_{1}(v_1,t_{\tau_1})\sigma_{2}(v_2,t_{\tau_2})\ldots
%	\sigma_{\ell}(v_\ell,t_{\tau_\ell})\sigma_{\ell+1}\sigma^{ab}_{\ell+1}
%	\ldots\sigma_{k}\sigma^{ab}_{k}$ where:\smallskip
%	
%	\noindent$\bullet$  $t_{\tau_i}\in T_\tau$ for $1\leq i \leq \ell$;\\
%	\noindent$\bullet$ The threads $v_i$ are initial for $1\leq i \leq \ell$;\\
%	$\bullet$ The threads $v_i$ are final for $\ell+1\leq i \leq k $;\\
%	$\bullet$ The firing sequence $\sigma_i\in (\{v_i\}\times T_{el})^*$ for $1\leq i \leq k$;\\
%	$\bullet$ The firing sequence $\sigma_i^{ab}\in (\{v_i\}\times T_{ab})^*$ for $\ell+1\leq i \leq k $.
%	%	
%	
%\end{definition}
%
%\begin{restatable}{proposition}{fromRPNtosim}
%	%\begin{proposition}
%	\label{prop: translating from RPN to sim}
%	Let $\N$ be an RPN
%	and $ s\xrightarrow{\sigma} s' $ be a firing sequence.
%	There exists  a \wellOrd\ firing sequence $s\xrightarrow{\widehat{\sigma}}s'$
%	in $\widehat{\N}$, with $ |\widehat{\sigma}|\leq|\sigma| $.
%	%\end{proposition}
%\end{restatable}
%
%\begin{proof}
%	By construction of $\widehat{\N}$, $\sigma$ is fireable in $\widehat{\N}$.
%	
%	
%	\noindent
%	First assume that we have an extremal thread $u$ which fires $ t\in T_{ab} $ creating a non final thread $ v $ that disappears by a matching cut transition $ (v,t_\tau)\in \sigma $ for $t_\tau\in T_\tau$.
%	One builds $\sigma'$ by (1) deleting from $\sigma $ the step $ (u,t) $, (2) deleting all the firings from $ Des_{\sigma}(v) $ in $\sigma$ and (3) replacing the step $ (v,t_\tau) $ by $(u,t^r)$. We claim that $s\xrightarrow{\sigma}s' $. Indeed
%	in $u$ the step $(u,t^r)$ has the same incidence in $u$
%	as the step  $(u,t)$ followed by $(v,t_\tau)$ (thus `anticipating' $(v,t_\tau)$ only add tokens in intermediate states)
%	and the other deleted firings are performed by threads in $Des_{\sigma}(v) $ which do not exist anymore.
%	Denote $\sigma^*$ the sequence obtained by iterating the process for all such cases.
%	
%	\noindent
%	Let us establish that we can transform  $\sigma^*$ into $\widehat{\sigma}$ fulfilling in the requirements for being \wellOrd,
%	by induction on $|V_s\cup V_{s'}|$, i.e. the number of extremal states.
%	If $ |V_s\cup V_{s'}|=0 $, $\sigma^*=\varepsilon$, hence  \wellOrd.
%	Assume that we have shown the proposition for any $\sigma^*$ with $|V_s\cup V_{s'}|< n$, and
%	that now we have $\sigma^*$ which fulfills $|V_s\cup V_{s'}|=n$.
%	We consider three cases according to a leaf thread $u$
%	(in $s$ or $s'$) with maximal depth:
%	\begin{enumerate}[nosep]
%		%
%		\item  $ u\in V_{s'} \cap V_s$.\,
%		Denote by $\sigma^*_u\subset \sigma^*$ the subsequence consisting of the firings
%		performed by $u$ in $\sigma^*$ and
%		$\sigma^*_r$ the subsequence of $\sigma^*$ obtained by removing $\sigma^*_u$.
%		Due to the first transformation,
%		$\sigma^*_u$ consists of elementary transitions.
%		Since $u$ is both an initial and final thread in $\sigma^*$,  $\sigma^*_u$ can be fired
%		at the end (or indifferently at the beginning) of $\sigma^*$.
%		Observe that $\sigma^*_r$ is a firing sequence from $s$ 
%		`without' $u$ to $s'$ `without' $u$.
%		So the induction applies: let $\widehat{\sigma}_r$ be the \wellOrd\ sequence
%		corresponding to $\sigma^*_r$. So $\widehat{\sigma}_r\sigma^*_u$ is the sequence
%		we are looking for.
%		%
%		\item  $u\in V_{s'} \setminus V_{s}$.\,
%		Let $(v,t) $ be the step which creates the thread $u$.
%		Denote by $\sigma^*_u\subset \sigma^*$ the subsequence consisting of  the firings
%		performed by $u$ in $\sigma^*$ and
%		$\sigma^*_r$ the subsequence of $\sigma^*$ obtained by removing $(v,t)$ and $\sigma^*_u$.
%		$\sigma^*_u$ consists of elementary transitions.
%		Since $u$ is a final thread in $\sigma^*$,  $\sigma^*_u$ can be fired
%		at the end of $\sigma^*$.
%		Observe that $\sigma^*_r$ is a firing sequence from $s$ to $s'$ 
%		`without' $u$ (say $s''$) where
%		$M_{s''}(v)=M_{s'}(v)+W^-(t)$.
%		By induction  there exists $\sigma^+_r$ a \wellOrd\ sequence
%		corresponding to $\sigma^*_r$ and
%		$\widehat{\sigma}_r$ be $\sigma^+_r$ with the firing $(v,t)$ inserted at the end of the  subsequence
%		of firings performed by $v$ in $\sigma^+_r$. Then $\widehat{\sigma}_r\sigma^*_u$ is the sequence
%		we are looking for.
%		%
%		%This sequence is still fireable from $ s' $ since $ (v,t) $ only decreases the marking of $ v $ and $ \sigma_u $ consist only of elementary transitions fired from $ u $. Since $\widehat{\sigma}_r$ has $ n-1 $ extremal threads we can use the induction hypothesis to get a \wellOrd\ sequence $ s\xrightarrow{\widehat{\sigma}'_r}s_r $.  Let $ v=v_i $ in the \wellOrd\ sequence. Since we did not fire $ (v_i,t) $ we have $ M_{s_r}(v_i)-W^-(t)=M_{s'}(v_i) $. Since the marking of $v_i$ changes only in $ \widehat{\sigma}_i\widehat{\sigma}_i^{ab} $, the sequence: $ \widehat{\sigma}'=  \widehat{\sigma}_r'\widehat{\sigma}_i\widehat{\sigma}_i^{ab}(v_i,t)\widehat{\sigma}_r''\widehat{\sigma}_u $ is \wellOrd\ and fireable from $ s $ to $ s' $.
%		%
%		\item $u\in V_s \setminus V_{s'}$.\,
%		Denote by $\sigma^*_u\subset \sigma^*$ the subsequence consisting of the firings
%		performed by $u$ in $\sigma^*$ and
%		$\sigma^*_r$ the subsequence of $\sigma^*$ 
%		obtained by removing $\sigma^*_u$.
%		\begin{itemize}[nosep]
%			%
%			\item If $\sigma^*_u$ does not end by a cut transition then
%			$\sigma^*_r$ is a firing sequence from $s$ `without' $u$ to $s'$.
%			Let $\widehat{\sigma}_r$ be the \wellOrd\ sequence
%			corresponding to $\sigma^*_r$. But $\widehat{\sigma}_r$ is also a sequence
%			from $s$ to $s'$.
%			%
%			\item  If $\sigma^*_u$ ends by a cut transition 
%			and $u$ is the root then
%			$\sigma^*_u$ is the sequence we are looking for.
%			%
%			\item If $\sigma^*_u$ ends by a cut step, $v$
%			is the parent of $u$ and $\Lambda(v,u)=t$ then
%			$\sigma^*_r$ is a firing sequence from $s$ `without' $u$ (say $s''$)
%			where $M_{s''}(v)=M_{s}(v)+W^-(t)$.
%			So the induction applies: let $\widehat{\sigma}_r$ be the \wellOrd\ sequence
%			corresponding to $\sigma^*_r$. So $\sigma^*_u\widehat{\sigma}_r$ is the sequence
%			we are looking for.
%			%
%		\end{itemize}
%		%
%	\end{enumerate}
%	Since we did not add any new step,   $ |\widehat{\sigma}|\leq |\sigma|$. 	
%\end{proof}
In order to recover from a sequence in $\widehat{\N}$ a sequence
in $\N$,  for every $ t\in T_{ret}$ one has to simulate the firings of a transition
$t^r$ by sequence $\sigma_t$. Therefore bounding the length of $\sigma_t$ is a critical issue. 
Recall that in~\cite{Rac78}, Rackoff showed that the coverability  problem for Petri nets
belongs to $\EXPSPACE$.
More precisely, he proved that if there exists a covering sequence,
then there exists a `short' one:
\begin{theorem}[Rackoff \cite{Rac78}]
	\label{thm:Rackoff covering path}Let
	$\N$  be a Petri net,  $m_{ini}$,
	$m_{tar}$ be markings and $\sigma$ be a firing sequence such that
	$m_{ini}\xrightarrow{\sigma}m\geq m_{tar}$.
	Then there exists a sequence $\sigma'$
	such that $m_{ini}\xrightarrow{\sigma'}m'\geq m_{tar}$ with
	$\left|\sigma'\right|\leq 2^{2^{cn\log n}}$
	for some constant $c$ and $n$ being the size of $(\N,m_{tar})$.
	
\end{theorem}
A surprising consequence of Rackoff's proof is that the length of the minimal coverability sequence does not depend on the initial marking of the net.


\begin{proposition}
	\label{prop:Length of an abstract transition in RPN}
	Let $\N$ be an RPN and $t\in T_{ret}$.
	Then the returning sequence $\sigma_t$
	fulfills $|\sigma_t|\leq 2^{\cdot2^{dn\log n}}$ for some constant $d$ and $n=size(\N)$.
\end{proposition}

\begin{proof}
	Let us enumerate
	$T_{ret}=\{t_1,\ldots,t_K\}$ in such a way that $i<j$ implies $|\sigma_{t_i}|\leq|\sigma_{t_j}|$.
	Observe first that the shortest returning sequences do not include
	firings of abstract transitions not followed by a matching cut transition
	since it could be omitted as it only deletes tokens in the thread.
	We argue by induction on $k\leq K$ that:
	\[
	|\sigma_{t_{k}}|<2^{k\cdot2^{cn\log n}} \qquad \mbox{where } c \mbox{ is the Rackoff constant}
	\]
	For $k=1$, we know that $\sigma_{t_{1}}$ has a minimal length over all
	returning sequences. Hence
	there are no cuts
	in $\sigma_{t_{1}}$ except the last one. Due to the above observation,
	$\sigma_{t_{1}}$ only includes firing of elementary transitions.
	Thus the Rackoff bound of Theorem~\ref{thm:Rackoff covering path} applies
	for a covering of some final marking.
	
	\noindent
	Assume that the result holds for all $i<k$.
	Due to the requirement on lengths,  $\sigma_{t_{k}}$
	only includes cuts from threads created by $t_{i}\in T_{ret}$ with $i<k$.
	Thus by Proposition~\ref{prop:omniciant}
	we get a sequence $\widehat{\sigma}_{t_{k}}\cdot(r,t_\tau)$ 
	in $\widehat{\N}$ (where $r$ is the root and $ t_\tau\in T_\tau $). The sequence
	$ \widehat{\sigma}_{t_{k}} $ consists of only elementary transitions
	and does not contain any transition  $t_i^r$ with $i\geq k$.
	The marking of $r$ reached by $ \widehat{\sigma}_{t_{k}} $ covers
	some final marking, hence	 by Theorem~\ref{thm:Rackoff covering path}
	there exists a covering sequence $\widehat{\sigma}_{t_{k}}'$ such that $|\widehat{\sigma}_{t_{k}}'|\leq2^{2^{cn\log n}}$.
	Since $\widehat{\sigma}_{t_{k}}$ does not contain firing of $t_i^r$ with $i\geq k$
	this also holds for $\widehat{\sigma}_{t_{k}}'$. Substituting any firing of $t_i^r$
	by 	$\sigma_{t_i}$, one gets a corresponding sequence $\sigma_{t_k}'$	in $\N$. Using the induction hypothesis, one gets that
	the length of $\sigma_{t_k}'$ fulfills:
	\[
	|\sigma_{t_k}'|\leq|\widehat{\sigma}_{t_{k}'}|2^{(k-1)\cdot2^{cn\log n}}\leq2^{2^{cn\log n}}\cdot 2^{(k-1)\cdot2^{cn\log n}}\leq2^{k\cdot2^{cn\log n}}
	\]
	From minimality of $\sigma_{t_{k}}$,
	one gets $|\sigma_{t_{k}}|\leq|\sigma_{t_k}'|\leq2^{k\cdot2^{cn\log n}}$
	which concludes the proof since
	\[
	\max_{t\in T_{ret}}\{ |\sigma_{t}|\}\leq2^{|T_{ret}|
		\cdot2^{cn\log n}}\leq2^{n2^{cn\log n}}\leq2^{2^{2cn\log n}}.
	\]
\end{proof}

Using the previous proposition, we can compute $T_{ret}$ in exponential space, by enumerating for all
abstract transitions, all firing sequences of sufficient length and checking whether they lead to the empty tree.


Below are immediate corollaries from the previous  propositions:
\begin{corollary}\label{col:bound_on_translation_of_N-hat_to_N}	
	Let $\N$ be a marked RPN. 
	Then for all $s\xrightarrow{\widehat{\sigma}}_{\widehat{\N}}s'$, there exists $s\xrightarrow{\sigma}_{\N}s'$ 
	such that $|\sigma|\leq 2^{\cdot2^{dn\log n}} |\widehat{\sigma}|$ for some constant $d$ and $n=size(\N)$.
\end{corollary}


\begin{corollary}\label{col:build_N_hat}
	Given an RPN $\N$ one can build $\widehat{\N}$ in exponential space. 
\end{corollary}


In order to mimic the behavior of a  specific thread in a firing sequence (which will be useful later on), 
we introduce the Petri net $\widehat{\N}_{el}$. The size of $\widehat{\N}_{el}$ is also linear w.r.t. the size of $\N$.

\begin{definition}\label{def:N_el}
	Let $\N$ be an RPN. Then the Petri net $\widehat{\N}_{el}=\left<P,\widehat{T}_{el},\widehat{W}^+_{el},\widehat{W}^-_{el}\right>$  is defined by:
	\begin{itemize}
		%
		\item $\widehat{T}_{el}=\widehat{T}\setminus T_\tau$;
		%
		\item For all $t\in \widehat{T}_{el}\setminus T_{ab}$,  $\widehat{W}^{-}_{el}(t)=\widehat{W}^{-}(t)$
		and  $\widehat{W}^{+}_{el}(t)=\widehat{W}^{+}(t)$;
		%
		\item For all $t\in T_{ab}$,  $\widehat{W}^{-}_{el}(t)=\widehat{W}^{-}(t)$ and  $\widehat{W}^+_{el}(t)=0$.
		
	\end{itemize}
Figure~\ref{fig:RPN_hat} has an example of an RPN $\N$ and its $\widehat{\N}_{el}$.
\end{definition}
As for  $\widehat{\N}$, one can build $\widehat{\N}_{el}$ in exponential space. 

\noindent{\bf Observation.} The main (straightforward) property of $\widehat{\N}_{el}$ is the following one.
Let $\sigma\in \widehat{T}_{el}^*$ with $n_t$ the number of occurrences of $t$ in $\sigma$. 
Then $m_0\xrightarrow{\sigma}_{\widehat{\N}_{el}} m$
if and only if $s[r,m_0]\xrightarrow{(r,\sigma)}_{\widehat{\N}} s$ with $V_s=\{r\}\cup \bigcup_{t\in T_{ab}} \{v_{t,1},\ldots,v_{t,n_t}\}$, $M_s(r)=m$
and for all $v_{t_i}$,  $r \xrightarrow{W^+(t)}_s v_{t_i}$  and $M_s(v_{t_i})=\Omega(t)$.




==> termination.tex <==
% !TEX root =main.tex
\section{Termination is \EXPSPACE-Complete}
\label{sec:termination}
In this section we tackle the termination problem for RPN.
Let $(\N,s_{0})$ be a marked RPN.
We denote the size of the input of the termination problem by $\eta$.
In~\cite{Rac78} Rackoff showed that the termination
problem for Petri net is solvable in exponential space:
\begin{theorem}[Rackoff\cite{Lipton76,Rac78}]
	\label{thm:Termination Bound For PN }The termination problem for Petri
	nets is $\EXPSPACE$-complete.
\end{theorem}
We aim to show that the termination
problem for RPN is $\EXPSPACE$-complete. $\EXPSPACE$-hardness follows
immediately from  $\EXPSPACE$-hardness of the termination problem for
Petri nets~\cite{Lipton76}.
By Proposition~\ref{col:rooted} we can assume that  $V_{s_0} = \{r\}$. Hence for the rest of the section, we will assume that $s_0 = s[r,m_0]$ for some marking $m_0$.

\noindent A main ingredient of the proof is the construction of an \emph{\at\ graph}
related to the firing of abstract transitions. 



\begin{definition}[\at\ graph]
	Let $(\N,s_0)$ be a marked RPN. Let
	$ G_{\N,s_{0}}=(V_{a},E_{a},M_{a}) $ be a labeled directed graph defined inductively as follows:\smallskip
	\begin{enumerate}
		%
		\item $r\in V_a$ and $M_{a}(r)=m_0$;
		%
		%		\item For any $t\in T_{ab}$, if there exists a fireable sequence $s[r,m_r] \xrightarrow{\sigma(r,t)}$, i.e. ending by firing $(r,t)$, then add $v_t$ to $ V_a$ and $(r,v_t)\in E_a$.
		%		%
		\item For any $v\in V_a$ and $t\in T_{ab}$, if there exists  $s[v,M_{a}(v)] \xrightarrow{\sigma(v,t)}$ then 
		
		$v_{t} \in V_a$, $(v,v_t)\in  E_a$ and $M_{a}(v) = \Omega(t)$.
	\end{enumerate}
	
\end{definition}
%\begin{definition}[\at\ graph]
%	Let $ \N $ be an RPN and $s$ be an initial state. Let
%	$ G_{\N,s_{0}}=(V_{a},E_{a},M_{a}) $ be a labelled directed graph defined by:\smallskip
%	
%\noindent	1. $V_{a}=\{ v_{t}\mid t\in T_{ab}\} \uplus \{r\}$;\\
%	2. $M_{a}:V_{a}\rightarrow\nat^{P}$ where $M_{a}(r)=m_r$ and for all $t$ in $T_{ab}$,
%	$M_{a}(v_t):=\Omega(t)$; \\
%	3. $E_{a}\subset V_{a}\times V_{a}$ such that for all $t \in T_{ab}$
%	and $v \in V_{a}$,
%	$(v,v_{t}) \in E_{a}$ if there exists a firing sequence
%	$\sigma$ from the state $s[r_v,M_{a}(v)]$ ending by a firing $(v,t)$. 
%\igor{\\(change the definition to include only reachable vertices?)}
%\end{definition}
Observe that an edge $(v,v_{t})$ means that  from state $s[v,M_a(v)]$, the
thread $v$ can fire $t$ in the future 
and by induction that $v_t\in V_a$ if and only if $t$ is fireable in the marked RPN.
Observe that the size of $ G_{\N,s_{0}}$ is linear w.r.t. the size of $(\N,s_0)$.
%Equivalently assertation~3 means that the edge $(v,v_t)$ belongs to $E_{a}$ if
%there exists a covering sequence
%$s[M_{a}(v)]\xrightarrow{\sigma} s\succeq s[W^-(t)]$.
%Thus building the \at\ graph amounts to solving
%a quadratic number of coverability problems.
%Using Theorem~\ref{thm:Coverabilty for RPN in EXPSPACE},
%one can build it in \EXPSPACE.
\begin{lemma}\label{lem:abstract graph in expspace}
	Let $(\N,s_{0})$ be a marked RPN. 
	Then one can build its abstract graph in exponential space.
\end{lemma}
\begin{proof}
	First note that $|V_a|\leq|T_{ab}|+1$. 
	Then for any vertex $v$ already in $V_a$ and any $t\in T_{ab}$ 
	checking whether  $s[v,M_{a}(v)] \xrightarrow{\sigma(v,t)}$ is fireable
	is equivalent to solving the covering problem 
	$M_{a}(v)\xrightarrow{\sigma} m\succeq W^-(t)$ in $\widehat{\N}_{el}$ (recall Definition~\ref{def:N_el})
	which can be done in exponential space due to Rackoff's coverability theorem for Petri nets.
\end{proof}
While we will not prove it, using a reduction from the Petri net coverability problem,
one can show that we cannot use less than an exponential space to build the abstract graph.

Let us illustrate the \at\ graph in
Figure~\ref{fig:at_graph} corresponding to the RPN of Figure~\ref{fig:rpn_example}.
Here the initial state is $s[r,p_{ini}]$. For clarity, we have renamed the abstract transitions
as follows:
$
t:={t_{beg}}$, $ta:={t_{a_2}}$, $tb:={t_{b_2}}.
$
For instance, the existence of the edge from $v_t$ to $v_{ta}$
is justified by the firing sequence $(v_t,t_{a_1})(v_t,ta)$.
\begin{figure}[h]
	\begin{center}
		%		(respectively $\Lambda_s, M_s$)
		\input{abst_tran_graph}
	\end{center}
	\caption{An abstract graph for the RPN in
		Figure~\ref{fig:rpn_example} }
	\label{fig:at_graph}
\end{figure}


Let $\sigma$ be an infinite firing sequence. We say that $\sigma$
is \emph{\lseq}\ if it visits a state $s$ whose depth is strictly greater
than $|T_{ab}|$. Otherwise, we say that $\sigma$ is \emph{\sseq}.
To solve the termination problem it suffices
to show whether the RPN has such an infinite sequence, either \sseq\
or \lseq.




The next lemma establishes that
\emph{lassos} of the \at\ graph
are witnesses of \lseq\ infinite sequences in an RPN:
\begin{restatable}{lemma}{unboundedpath}
	%\begin{lemma}
	\label{lem:Finidng unbounded path using at}
	Let $(\N,s_{0})$ be a marked RPN.
	Then there is a \lseq\ infinite sequence starting from $s_{0}$
	if and only if there is a cycle in $G_{\N,s_{0}}$.
	%\end{lemma}
\end{restatable}
\begin{proof}
	$\bullet$ Assume that $ \sigma $ is a \lseq\ sequence. Hence, it reaches
	a state  $\tilde{s}$ whose tree has a path $ \gamma $
	starting from the root, with $|\gamma|> |T_{ab}|$. Let us denote it by
	$\gamma=(v_{i})_{i=1}^{m}$.
	For all $ i\leq m $ denote by $ t_i $ the abstract transition that creates
	$ v_i $. Using $ \gamma$, one builds a path
	$ \gamma_{a}=v_{1}v_{2}\ldots v_{m} $ in $G_{\N,s_{0}}$ as follows. First
	$ v_{1}=r $ and $ m_r= M_{a}(r) $. Since along
	$ \sigma $ the
	thread $ r $ fires  $ t_1 $ to create $v_2$, there is an
	edge between $ r $ to $ v_{t_2} $ in $ G_{\N,s_{0}} $. For any
	$ 1< i\leq m $ the thread $ v_{i} $ is created with the marking
	$ \Omega(t_i)=M_{a}(v_{t_i}) $. Since $ v_{i+1} $ is a child of $ v_i $,
	somewhere on the sequence $ \sigma $ the thread $ v_i $ fires 
	$ t_{i+1} $. Therefore there is an edge from $ v_{t_{i}} $
	to $ v_{t_{i+1}} $ in $ G_{\N,s_{0}}$.
	The length of the path $ \gamma_a $ strictly greater then $ |T_{ab}|$,  and since $V_{a}\leq|T_{ab}|+1$ there is a cycle in $\gamma_a$.
	
	\noindent $\bullet$
	Conversely assume that there is a cycle in $G_{\N,s_{0}}$.
	Then there is an
	infinite path $\gamma_a=\{ v_{i}\} _{i=0}^{\infty}$
	in $G_{\N,s}$ starting from $r$, where for any $i\geq1$ denote by $t_{i}$ the abstract
	transition associated the vertex $v_i$. We now translate this infinite path
	to an \lseq\ sequence on $\N$ with initial state $s_{0}$. Note that
	$v_{0}=r$ and that $m_r=M_{a}(r)$. By definition of
	$E_{a}$ there is a sequence $s \xrightarrow{\sigma_{1}}s_0'$ where the
	abstract transition $ t_1 $ is fireable from $v_{0}$ in $ s_0' $. We get
	$ s\xrightarrow{\sigma_{1}}s_0'\xrightarrow{(v_0,t_1)}s_{2}$. Denote by
	$ v_1 $ the thread created by $t_1$. The threads marking has
	$M_{s_1}(v_1)=M_{a}(v_1)$, therefore one continues translating the path
	$ \gamma_a $ in the same way as the first edge. Since for any
	$ (v_i,v_{i+1}) $ in $ \gamma_{a} $ we create a new thread from
	$ v_i $ one gets an \lseq\ sequence. 
\end{proof}
We now show that for any \sseq\  $\sigma$ there
is a thread $v$ which fires infinitely many times in $\sigma$.

\begin{restatable}{lemma}{infinitelymanytimes}
	%\begin{lemma}
	\label{lem: thread repets infinitly many times}
	Let $(\N,s_0)$ be a marked RPN and $\sigma$ be a \sseq\
	sequence. Then there is a thread $v$ that fires infinitely many times
	in $\sigma$.
	%\end{lemma}
\end{restatable}
\begin{proof}
	If the root $r$ fires infinitely often then we are done.
	Otherwise, $r$ has finitely many children, and the firing subsequence of $\sigma$ of the subtree of (at least) one child, say $v$, must be infinite. 
	If $v$ fires infinitely often then we are done. 
	Otherwise, we proceed inductively up to $|T_{ab}|$ where some thread must fire infinitely often.
\end{proof}

%\begin{proof}
%	Assume for contradiction that there is no thread $v$ which fires infinitely
%	many times in $\sigma$. Let  $\sigma$ be:
%	\[
%	s_0\xrightarrow{(u_1,t_1)}s_1\xrightarrow{(u_2,t_2)}s_2\xrightarrow{(u_3,t_3)}\ldots
%	\]
%	Denote by $ V_0:=V_{s_0} $.
%	%Note that the minimal distance of any $v\in V_{0}$
%	%to the root in $ s_0 $ is $ 0 $.
%	Since $V_{0}$ is finite and  no
%	$ v\in V_0 $  fires infinitely many times along $\sigma$
%	there exists an index $m_{0}$ such that for any $i>m_{0}$,
%	$u_{i}\notin V_{0}$. Let us show how to build inductively a set $V_{k}$ and
%	an index $m_{k}$, with the following properties:
%	\begin{itemize}
%		%
%		\item For all $i>m_{k}$,  $u_{i}\notin \bigcup_{i=0}^k V_{k}$;
%		%
%		\item For all $v\in V_{k}$ the distance between $v$ and the root is at least $k$;
%		%
%		\item $V_{k}$ is finite.
%		%
%	\end{itemize}
%	Let $V_{k}=V_{s_{m_{k-1}}}\backslash\cup_{i=0}^{k-1}V_{i}$. By construction,
%	$V_{k}$ is finite. Moreover, any thread in $V_{k}$ has been created by a thread
%	$ u_i \in Des_{\sigma}(V_{k-1})$. Hence its distance from the root is at least of length $k$.
%%	is at least of distance $k$ from the root. 
%	 Finally, since no thread fires infinitely many times
%	on $\sigma$ there is an index $m_{k}$ such that for all $i>m_{k}$
%	$u_{i}\notin V_{k}$.
%	
%	\noindent
%	Let $ n=|T_{ab}|+|V_s|+1 $. The distance between $s_{m_{n}}$ and the root
%	is greater than $|T_{ab}|+|V_s|$ yielding a contradiction. 
%\end{proof}

We now show that given some state $s[r,m_0]$ one can check
in exponential space the existence
of a \sseq\ sequence in which $r$ fires infinitely many times.

\begin{restatable}{lemma}{sseqFromu}
	%	\begin{lemma}
	\label{lem:sseq from a given u}
	Let  $(\N,s_0)$ be a marked RPN. Then  one can check in exponential space,
	whether there exists an infinite sequence starting 
	with $r$ firing infinitely many times.
\end{restatable}
\begin{proof}
	We first show that there is a sequence  where $r$ fires infinitely many times 
	if and only if there is a infinite firing sequence in the marked Petri net $(\widehat{\N}_{el},m_0)$.
	
	\noindent
	$\bullet$ Assume there exists such $\sigma$ in $(\N,s[r,m_0])$. Then the sequence $\sigma$ is also fireable in $(\widehat{\N},s[r,m_0])$.
	In $\widehat{\N}$, one eliminates in $\sigma$ the cut transitions by increasing occurrence order as follows. Let $(v,t)$ be a cut transition
	and $(v',t')$ be the firing that creates $v$. Then one deletes all the firings performed by the descendants
	of $v$ and replaces $(v',t')$ by $(v',t'^r)$. Let $\sigma'$ be the sequence obtained after this transformation.
	In $\sigma'$, the root still fires infinitely often since no firing performed by the root has been deleted (but sometimes
	substituted by an elementary firing). Moreover, $\sigma'$ has no more cut transitions.
	Consider the still infinite firing sequence $(r,\sigma'')$ where in  $\sigma'$ all firings in other vertices than $r$ have been deleted.
	Observe now  that by definition, $\sigma''$ is also an infinite sequence of $\widehat{\N}_{el}$.
	
	\noindent
	$\bullet$  Conversely, assume there exists an infinite firing sequence $\sigma$ of $(\widehat{\N}_{el},m_0)$. Then
	$(r,\sigma)$  is  an infinite firing sequence of $(\widehat{\N},s[r,m_0])$ (with only root firings)
	entailing the existence of  an infinite firing sequence of $(\N,s[r,m_0])$. 
	
	\noindent
	By Theorem~\ref{thm:Termination Bound For PN }, one can check in exponential space
	whether there exists an infinite sequence of $(\widehat{\N}_{el},m_0)$.
\end{proof}

Summing up the results for \sseq\ and \lseq\ sequences we get:

\begin{theorem}
	\label{prop:Bounded path in EXPSPACE}
	The termination problem of RPN is \EXPSPACE-complete.
\end{theorem}

\begin{proof}
	The algorithm proceeds as follows.
	It builds in \EXPSPACE\ (by Lemma~\ref{lem:abstract graph in expspace}) the \at\ graph and
	checks  whether
	there is a \lseq\ infinite sequence
	using the characterization of Lemma~\ref{lem:Finidng unbounded path using at}.
	In the negative case, it looks for a \sseq\ infinite
	sequence. To this aim, it checks in exponential space for any reachable vertex $v$
	from $r$ in $G_{\N,s_{0}}$, whether
	there exists an infinite sequence starting from $s[v,M_{a}(v)]$
	with the root firing infinitely many times.
	The complexity follows from Lemma~\ref{lem:sseq from a given u}
	while the correctness
	follows from Lemma~\ref{lem: thread repets infinitly many times}.
\end{proof}


%\begin{proposition}\label{prop:reacabilty of s_u}
%	Let $(\N,s)$ be a marked RPN and $U\subseteq V_s$, closed by
%	the descendant relation. 
%	Then one can check in exponential space, whether there exists 
%	$\sigma = (v_1,t_1)\ldots(v_n,t_n)$ such that 
%	$s\xrightarrow{\sigma}s\backslash U$, and $v_i\in U$  for all $i\leq n$.
%\end{proposition}
%
%\begin{proof}
%	Let $R$ be the set of roots of $U$. 
%	Let $\rho\in R$ and define $s_\rho$ the state 
%	which is the subtree rooted at $\rho$ 
%%	 $V_{s_{\rho}} = Des_s(\rho) $ and $E_{s_{\rho}}$
%%	(respectively $\Lambda_{s_{\rho}}, M_{s_{\rho}}$) is equal to $E_s$ 
%%	restricted on $Des_s(\rho)$ (respectively $\Lambda_s, M_s$). 
%	The sequence $s\xrightarrow{\sigma}s\backslash U$ 
%	exists if and only if for all $\rho\in R$ 
%	there exists a sequence $s_\rho\xrightarrow{\sigma_\rho}\emptyset$. 
%	Therefore due to Theorem \ref{thm:cut problem}, 
%	this can be done in exponential space.	
%		
%\end{proof}
%
%%Combining Propositions~\ref{prop:reductiontoconstrained}
%%and~\ref{prop:Bounded path in EXPSPACE} one gets:
%We now prove that the termination problem is \EXPSPACE\ by reducing it in \EXPSPACE\
%to an exponential
%number of instances of the constrained termination problem with similar size:
%\begin{theorem}\label{thm:termination}
%The termination problem of RPN is \EXPSPACE-complete.
%\end{theorem}
%
%\begin{proof}
%	W.l.o.g. we assume that $\N$ has been enlarged to $\widehat{\N}$
%	since the termination problem remains unchanged
%	by this transformation.
%	Assume there is $\sigma$ an infinite firing sequence
%	and $U$ be the subset of initial threads that disappear
%	along $\sigma$. Observe that $U$ is closed by the descendent relation. 
%	Let $\sigma'$ be the shortest finite prefix of $\sigma$
%	such that all threads of $U$ have disappeared.
%	Using Proposition~\ref{prop: translating from RPN to sim},
%	$\sigma'$ can be assumed to be \wellOrd. Hence we can split it 
%	to two subsequences
%	$s\xrightarrow{\sigma_U}s\backslash U\xrightarrow{\sigma''}$, 
%	where the firings in $\sigma_U$ are done by threads in $U$. 
%	Therefore an infinite firing sequence starting from $s$ exists 
%	if and only if there
%	exists an infinite constrained sequence from some reachable 
%	$s\backslash U$. Thus for all $U\subseteq V$ closed by the descendent 
%	relations, one checks whether $s\backslash U$ is reachable from $s$ 
%	(in \EXPSPACE\ by Proposition \ref{prop:reacabilty of s_u}),
%	and in the positive case, solves the constrained termination problem
%	for $s\backslash U$(in \EXPSPACE\ 
%	by Proposition~\ref{prop:Bounded path in EXPSPACE}).
%\end{proof}

